Internal heating profiles for which downward conduction is impossible

We consider an internally heated fluid between parallel plates with fixed thermal fluxes. For a large class of heat sources that vary in the direction of gravity, we prove that $\langle\delta T \rangle_h \geq \sigma R^{-1/3} - \mu$, where $\langle\delta T \rangle_h$ is the average temperature difference between the bottom and top plates, $R$ is a `flux' Rayleigh number and the constants $\sigma,\mu >0$ depend on the geometric properties of the internal heating. This result implies that mean downward conduction (for which $\langle\delta T \rangle_h< 0$) is impossible for a range of Rayleigh numbers smaller than a critical value $R_0$. The bound demonstrates that $R_0$ depends on the heating distribution and can be made arbitrarily large by concentrating the heating near the bottom plate. However, for any given fixed heating profile of the class we consider, the corresponding value of $R_0$ is always finite. This points to a fundamental difference between internally heated convection and its limiting case of Rayleigh-B\'enard convection with fixed flux boundary conditions, for which $\langle\delta T \rangle_h$ is known to be positive for all $R$.

==> post-review/rv1.tex <==
\section{Introduction}
\label{sec:intro}


Convection driven by spatially varying heating is attracting attention as a generalisation of internally heated convection (IHC) due to its relevance in studying different regimes of heat transport by turbulence. Recent work demonstrates that varying the heating location can enhance heat transport in bounded domains \citep{kazemi2022,bouillaut2022, Lepot2018} and that bounds on the heat transport depend on the supply of potential energy due to variable heating \citep{Song2022}. 
Such studies of non-uniformly heated convection have implications for geophysical fluid dynamics, from mixing in lakes, where solar radiation acts as a spatially varying heat source, to convection in the Earth's mantle and liquid outer core driven by energy released irregularly by radioactive isotopes and secular cooling \citep{schubert2015treatise}. Furthermore, non-uniform heating is theoretically significant because it induces a much larger class of flows than those by boundary-forced examples such as Rayleigh-B\'enard convection (RBC). 


This work considers non-uniform IHC between parallel plates with fixed thermal fluxes. \revision{Specifically, we assume that the lower plate is a thermal insulator and that the upper plate is a poor conductor in comparison to the fluid's ability to transport heat \citep[see, for example,][]{Goluskin2015a}. The heat flux through the upper plate is therefore assumed fixed  and, to ensure that a statistically stationary state is realisable, is specified to match the total heat input due to internal heating (\cref{fig:config}\textit{(a)}). The Rayleigh number $R$ for this system, defined precisely in \S\ref{sec:setup}, quantifies the destabilising effect of internal heating relative to the stabilising effect of diffusion. An emergent physical property of the flow on which we will focus is the mean temperature difference, $\dT$, between the lower and upper plates (we use $\volav{\cdot}$ to represent an infinite time and volume average, with subscript $h$ denoting a horizontal average). }


\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \draw[black,thick] (-6,0) -- (-2,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (-6,1.8) -- (-2,1.8) node [anchor = west] {$z=1$};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(2.86,1.8) (3.02,1.62) (3.1,1.5)};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(3.1,0.3) (3.16,0.18) (3.34,0)};
    \draw [dashed ,colorbar10] (2.5,1.8) -- (3.7,0);
    \draw [colorbar10] (3.1,1.5) -- (3.1,0.3);
    \node at (1.25,-0.25) {$ \partial_z T = -1 $};
    \node at (1.25,2.025) {$ \partial_z T = -1 $};
    \node at (-4.75,0.9) { $H(z)$ };
    \draw[->] (-7,0) -- (-7,0.36) node [anchor=east]{$z$};
    \draw[->] (-7,0) -- (-6.6,0) node [anchor=north]{$x$};
    \draw[->] (-7,0) -- (-6.64,0.2) node [anchor=west]{$y$};
    \draw[black,thick] (0,0) -- (4,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (0,1.8) -- (4,1.8) node [anchor = west] {$z=1$};
    \node at (-4.75,-0.25) {$ \partial_z T = 0 $};
    \node at (-4.75,2.025) {$  \partial_z T = - 1 $};
    \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(-3.5,1.8) (-2.8,1.1) (-2.5,0)};
    \draw [colorbar10] plot [smooth,tension=1] coordinates {(-3.5,1.8) (-3.12,1.58) (-3,1.45)}; 
    \draw [colorbar10] (-3,1.45) -- (-3,0);
    \draw[->,colorbar10,thick] (2.5,0) -- (2.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (2.5,0) -- (2.9,0) node [anchor=north]{$T$};
   \draw[->,colorbar10,thick] (-3.5,0) -- (-3.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (-3.5,0) -- (-3.1,0) node [anchor=north]{$T$};
    \node at (-6.4,1.8) {\textit{(a)}};
    \node at (-0.4,1.8) {\textit{(b)}};
    \end{tikzpicture}
    \caption{\textit{(a)} Internally heated and \textit{(b)}  Rayleigh-B\'enard convection with fixed flux boundaries, where $H(z)$ is a positive non-uniform heating profile. In both panels, ({\color{colorbar10}\dashedrule}) denotes the conductive temperature profiles and ({\color{colorbar10}\solidrule}) the mean temperature profiles in the turbulent regime. In panel \textit{(a)}, the temperature profiles are for $H(z)=1$. }
    \label{fig:config}
\end{figure}

This paper communicates bounds on $\dT$ that depend on the Rayleigh number $R$ of the flow and the spatial distribution of the heat sources. More specifically, we prove that for any solution of the governing Boussinesq equations,
\begin{equation}
    \label{eq:main_res}
    \dT := \horav{T|_{z=0}} - \horav{T|_{z=1} } \geq \sigma R^{-\gamma}-\mu, 
\end{equation}
where $\sigma,\mu>0$ are constants depending only on the \revision{spatial distribution} of the internal heating, and $\gamma$ is a scaling rate. {\color{matlabred} A corollary of \eqref{eq:main_res} is that 
downward conduction, here defined as the emergent mean temperature of the upper plate being above that of the lower plate, i.e., $ \horav{T|_{z=1}} > \horav{T|_{z=0}}$, is impossible for $R\leq R_0= (\sigma/\mu)^{1/\gamma}$, where $R_0$ is a critical Rayleigh number that depends on the spatial distribution of the internal heating.} 


{\color{matlabred} To give context to this result, observe that a flow for which a rigorous characterisation of $\dT$ is known is fixed-flux RBC, shown schematically in \cref{fig:config}\textit{(b)}. In that case, symmetric heating and cooling rates are prescribed at the upper and lower boundaries (as opposed to internally), and the temperature drop satisfies the rigorous bound $\dT \geq cR^{-1/3}$ for a constant $c>0$ \citep{Otero2002}. The physical interpretation of this result is that the upper plate, through which heat leaves the domain, must, on average, remain colder than the lower one. Further, the difference in temperature between the plates cannot decrease at a rate faster than $R^{-1/3}$, where $R \rightarrow \infty$ corresponds to an increasingly turbulent and homogenised flow. Noting that $R$ is a flux-based Rayleigh number (rather than being defined in terms of an imposed temperature difference), the provable decay rate of the lower bound on $\dT$ agrees with the predictions of some phenomenological theories, namely the so-called ultimate regime \citep{kraichnan1962,spiegel1963generalization}. See \cite{  doering2020turning} and \cite{lohse2023} for recent reviews on the ultimate regime in RBC. }



{\color{matlabred}  There is a striking and crucial distinction between what can currently be proven about the behaviour of the temperature drop $\langle \delta T \rangle_h$ in IHC in comparison with fixed-flux RBC. In particular, while for fixed-flux RBC downward conduction can be ruled out for all Rayleigh numbers (i.e., that $\dT >0$ must hold for all $R$), it is not yet known whether there are any heating profiles $H(z)$ that lead to the equivalent property in IHC. For example, in the case where internal heating is applied uniformly ($H \equiv 1$), it was shown by \cite{Arslan2021a} that $\dT \geq 1.6552R^{-1/3}-0.03868$. This only rules out downward conduction up to the critical Rayleigh number  $R_0 = 78\,389 = 54.437 R_L$, where $R_L=1440$ denotes the Rayleigh number at which the flow becomes linearly unstable \citep{Goluskin2015a}. 

The bound \eqref{eq:main_res}, which is the main result of this paper, gives valuable additional information on the gap between the known behaviour of $\dT$ for IHC with an insulating bottom plate and fixed-flux RBC. Specifically, it allows us to understand how the gap depends on the spatial distribution $H(z)$ of the internally applied heating via the constants $\mu = \mu(H)$ and $\sigma = \sigma(H)$ in \eqref{eq:main_res}. The dependence of this gap on $H$ is interesting since it is not unreasonable to expect that downward conduction may be more likely to occur if heating is concentrated close to the upper plate, as in Figure \cref{fig:config2}~(a), rather than close to the lower plate, as in Figure \cref{fig:config2}~(b). The specific expressions for $\mu$ and $\sigma$ derived in this paper do not allow downward conduction to be ruled out (i.e. $R_0 <\infty$) for any {\em fixed} heating profile $H$. However, we show that it is possible to construct a sequence of heating profiles $H_r$, indexed by an integer $r$, in which heating is asymptotically concentrated towards the lower plate as $r \rightarrow \infty$, for which 
%
\[
R_0(H_r) = \left( \frac{\sigma(H_r)}{\mu(H_r)} \right)^{ \frac{1}{\gamma(H_r)}} \rightarrow \infty \quad \text{as} \quad   r\rightarrow \infty.
\]
%
In this sense, we can partially bridge the gap between what is known about $\dT$ for fixed-flux RBC and what appears, at least from the perspective of rigorous mathematical analysis, to be the much more intricate behaviour of internally heated convective flows.  


\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \fill [colorbar14] (-7,1.8) rectangle (-3.5,1.2);
    \fill [colorbar14] (-3,0) rectangle (0.5,0.6);
    \shade [top color = colorbar6, bottom color = colorbar13] (1,0.9) rectangle (4.5,0.45);
    \draw [colorbar13] (1,0.45) -- (4.5,0.45);
    \shade [top color = colorbar13, bottom color = colorbar6] (1,0.45) rectangle (4.5,0);
    \draw [colorbar6] (1,0.9) -- (4.5,0.9);
    \shade [top color = colorbar6, bottom color = colorbar1] (1,1.8) rectangle (4.5,1.35);
    \draw [colorbar1] (1,1.35) -- (4.5,1.35);
    \shade [top color = colorbar1, bottom color = colorbar6] (1,1.35) rectangle (4.5,0.9);
    \draw[black,line width=0.35mm] (-7,0) -- (-3.5,0) ;
    \draw[black,line width=0.35mm] (-7,1.8) -- (-3.5,1.8) ;
    \draw[black,line width=0.35mm] (-3,0) -- (0.5,0) ;
    \draw[black,line width=0.35mm] (-3,1.8) -- (0.5,1.8) ;
    \draw[black,line width=0.35mm] (1,0) -- (4.5,0) node [anchor=west] {$z=0$};
    \draw[black,line width=0.35mm] (1,1.8) -- (4.5,1.8) node [anchor = west] {$z=1$};
    \draw plot [smooth, tension = 1] coordinates {(-4.8,1.8) (-4.2,1.5) (-4,1.2)};
    \draw (-4,1.2) -- (-4,0);
    \draw plot [smooth, tension = 1] coordinates {(0,0) (-0.12,0.3) (-0.5,0.6)};
    \draw (-0.5,0.6) -- (-0.8,1.8);
    \draw plot [smooth, tension = 1] coordinates {(3.2,1.8) (3.8,0.8) (4,0)};
    \node at (-7.2,1.8) {\textit{(a)}};
    \node at (-3.2,1.8) {\textit{(b)}};
    \node at (0.8,1.8) {\textit{(c)}};
    \end{tikzpicture}
    \caption{ Examples of non-uniform heating profiles in a non-dimensionalised domain with illustrative sketches of the conductive temperature profiles (\solidrule) for fixed flux boundary conditions. In \textit{(a)}, the heating is localised near the upper boundary and in \textit{(b)} near the lower boundary while being zero elsewhere, shown with red ({\color{colorbar14}\solidrule}) and white spaces respectively. For \textit{(c)} the heating is sinusoidal with a maximum at $z=0.25$ ({\color{colorbar13}\solidrule}) and a minimum of zero at $z=0.75$ ({\color{colorbar1}\solidrule}).   }
    \label{fig:config2}
\end{figure}


In summary, this paper proves a Rayleigh-dependent lower bound on $\dT$ that depends on the geometric properties of the internally applied heating. As a corollary, for any heating profile, we can find an expression for the critical Rayleigh number $R_0$ below which downward conduction is impossible for any solution of the governing equations. To do this, we develop the mathematical approach of \cite{Arslan2021a} for flows driven by arbitrary (non-uniform) heating. The paper is structured as follows: \S\ref{sec:setup} describes the problem setup, in \S\ref{sec:Bounds} we prove the lower bound \eqref{eq:main_res}, \S\ref{sec:Imp_bound} highlights implications of the bound on the possibility of downward conduction in geophysical flows and in \S\ref{sec:conclusion} we conclude.}

\section{Setup}
\label{sec:setup}

We consider a layer of fluid between two horizontal plates separated by a distance $d$ and periodic in the horizontal ($x$ and $y$) directions with periods $L_x d$ and $L_y d$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Gravity acts in the negative vertical direction, and the fluid is heated internally at a position-dependent non-negative volumetric rate $\Tilde{H}\geq 0$. We assume that $\Tilde{H}$ is a non-negative integrable function on the domain that depends only on the vertical coordinate and satisfies   $\langle \tilde{H}\rangle>0$ strictly, and define a dimensionless heating as $H(z):=\tilde{H}/\langle \tilde{H}\rangle$. Note that $\langle H\rangle=\|H\|_{1}=1$ because $H(z)\geq 0$. Here and throughout the paper, $\lVert f \rVert_p$ is the standard $L^p$ norm of a function $f:[0,1]\rightarrow\mathbb{R}$.


To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2\langle \tilde{H}\rangle/\kappa \rho c_p$ as the temperature scale. The velocity of the fluid $\boldsymbol{u}(\boldsymbol{x},t)=(u(\boldsymbol{x},t),v(\boldsymbol{x},t),w(\boldsymbol{x},t))$ and temperature $T(\boldsymbol{x},t)$ in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ are then governed by the Boussinesq equations,
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
The non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa},
    \qquad\text{and}\qquad 
    R = \frac{g \alpha \langle \tilde{H}\rangle d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are no-slip for the velocity and fixed flux for the temperature:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:nu}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-1.
\end{gather}
\end{subequations} 
 A diagram of the system is shown in \cref{fig:config}\textit{(a)}.

It proves useful to define a function $\eta \in L^2(0,1)$ such that $\eta(z)$ measures the total (dimensionless) heat  added to those parts of the domain below a height $z$:
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z)\, \textrm{d}z.
\end{equation}
% Our assumptions on $H(z)$ imply that $0\leq \eta(z)\leq 1$. 
The value $\eta(1)=1$ corresponds to the total heat added to the domain and, therefore, to the negative heat flux applied at the top boundary in \eqref{bc:nu}.
We can obtain an identity for the mean vertical heat transport of the system by multiplying \eqref{eq:nondim_energy_nonUniform} by $z$ and taking an infinite-time and volume average. Use of \eqref{eq:eta_general} and a standard application of integration by parts with the boundary conditions \eqref{bc:u_non_u} \& \eqref{bc:nu} gives the identity
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \dT &= -\int^{1}_{0}(z-1)H\,\textrm{d}z=\int^{1}_{0}\eta(z)\,\textrm{d}z.
\end{align}
The left-hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical convective heat flux, $\wT$, and the mean conductive heat flux, $\dT$, and balances the potential energy added to the system. To see why, note that $-zH$ is the pointwise supply of (dimensionless) potential energy (the negative sign is there because potential energy is created by positive heating from below or negative heating from above). The middle term in \eqref{eq:energy_bal_nu} therefore accounts for the potential energy created by internal heating and cooling from the top boundary (alternatively, the shifted coordinate $z\mapsto z-1$, centred on the top boundary, can be seen as a means of removing the cooling at the top boundary from the calculation).

To remove the inhomogeneous boundary conditions on $T$, it is convenient to rewrite the temperature field in terms of perturbations $\theta$ from the conductive profile $T_c$,
\begin{equation}
    \label{eq:T}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition, $T'_c(z) = - \eta(z)$, where primes denote derivatives with respect to $z$. Then, \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ becomes
\begin{gather}
    \label{eq:theta_eq}
     \partial_t \theta + \boldsymbol{u} \cdot \bnabla \theta = \bnabla^2 \theta + w\, \eta(z) ,\\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{gather}

\section{Bounding heat transport}
\label{sec:Bounds}

To bound $\dT$ using methods that have been successfully applied to uniform IHC \citep{Arslan2021a}, we search for an upper bound on $\wT$ and use \eqref{eq:energy_bal_nu} to bound $\dT$. We will prove upper bounds on  $\mean{w\theta}$, which is equal to $\wT$ because the incompressibility of the velocity field and the boundary conditions \eqref{bc:u_non_u} imply that any function $f:[0,1]\rightarrow\mathbb{C}$ satisfies $\volav{w f} = \int^{1}_0 \horav{w} f(z) \textrm{d}z = 0$. The derivation in  \cref{sec:afm} is analogous to that in \cite{Arslan2021a}, so we only outline the main ideas in this paper.


\subsection{The auxiliary functional method}
\label{sec:afm}

Rigorous bounds on the mean quantities of turbulent flows can be found with the background method \citep{Doering1994, Doering1996,Constantin1995a}, which we formulate here in the more general framework of the auxiliary functional method \citep{Chernyshenko2014a,Fantuzzi2022}. We consider the quadratic auxiliary functional
\begin{equation}
    \label{eq:af}
    \mathcal{V}\{\boldsymbol{u},\theta\} =  \fint_\Omega  \frac{a}{2\,Pr\,R} |\boldsymbol{u}|^2 + \frac{b}{2}\left|\theta  - \frac{\phi(z)}{b}\right|^2 \textrm{d}\boldsymbol{x} ,
\end{equation}
where $a$ and $b$ are non-negative scalars and $\phi(z)$ a function, all to be optimised. As demonstrated by \cite{Chernyshenko2022}, the use of quadratic auxiliary functionals is equivalent to the background method, where $a$ and $b$ are referred to as balance parameters and $\phi(z)/b$ is the background temperature field 
{\color{matlabred} satisfying the boundary conditions on $\theta$ in \eqref{bc:theta_non_u}}. With a slight abuse of terminology, we refer to $\phi(z)$ as the background field. 

Given that $\mathcal{V}\{\boldsymbol{u},\theta\}$ remains bounded in time along solutions of \eqref{eq:continuit}, \eqref{eq:mom_eq} \& \eqref{eq:theta_eq} for any given initial $\boldsymbol{u}$ and $\theta$, the infinite-time average of the time derivative of $\mathcal{V}$ is zero. Using this property, we can write
\begin{equation}
    \label{eq:AFM_statemen}
    \mean{w\theta} = U - \left( U - \volav{w\theta} - \limsup_{\tau\rightarrow\infty} \frac{1}{\tau}\int^{\tau}_0\frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\} \textrm{d}t  \right),
\end{equation}
and deduce that $\mean{w \theta} \leq U$, if after rearranging, the functional in the brackets in \eqref{eq:AFM_statemen} is pointwise in time non-negative. 
Following computations analogous to \cite{Arslan2021a}, {\color{matlabred}the terms in the brackets of \eqref{eq:AFM_statemen} becomes
\begin{equation}
    \label{eq:s_f}
    \mathcal{S}\{\boldsymbol{u},\theta\}:=\fint_{\Omega} \frac{a}{R} |\bnabla \boldsymbol{u}|^2 + \beta |\bnabla \theta|^2 - (a+1+b\eta(z) - \phi'(z))w\theta - \phi'(z)\partial_z\theta + U \, \textrm{d}\boldsymbol{x}.
\end{equation}
The positivity of \eqref{eq:s_f} is demonstrated by first exploiting horizontal periodicity and using the Fourier series
\begin{equation}\label{e:Fourier}
    \begin{bmatrix}
    \theta(x,y,z)\\\boldsymbol{u}(x,y,z)
    \end{bmatrix}
    = \sum_{\boldsymbol{k}} 
    \begin{bmatrix}
    \hat{\theta}_{\boldsymbol{k}}(z)\\ \hat{\boldsymbol{u}}_{\boldsymbol{k}}(z)
    \end{bmatrix}
    \textrm{e}^{i(k_x x + k_y y)}\, ,
\end{equation}
where the sum is over suitable wavenumbers $\boldsymbol{k} = (k_x,k_y)$ with magnitude $\boldsymbol{k} = \sqrt{k_x^2+ k_y^2}$ and where the complex-valued Fourier amplitudes satisfy the complex conjugate relations $\hat{\boldsymbol{u}}_{-\boldsymbol{k}} =\hat{\boldsymbol{u}}^*_{\boldsymbol{k}} $ and $\hat{T}_{-\boldsymbol{k}} =\hat{T}^*_{\boldsymbol{k}} $. Then, $\mathcal{S}\{\boldsymbol{u},\theta\}$ can be lower bounded by 
\begin{equation}
    \mathcal{S}\{\boldsymbol{u},\theta\} \geq \mathcal{S}_0\{\hat{\theta}_{0}\} + \sum_{k} \mathcal{S}_{\boldsymbol{k}}\{\hat{w}_0, \hat{\theta}_0\},
    \label{eq:s_f_f}
\end{equation}
where
\begin{equation}
    \mathcal{S}_0\{\hat{\theta}_0\} = U+ \int^{1}_0 b |\hat{\theta}'_0|^2 - \phi'\hat{\theta}'_0 \textrm{d}z,
    \label{eq:S0}
\end{equation}
and
\begin{multline}
    \label{eq:sk_non_uni}
     \mathcal{S}_{\boldsymbol{k}}\{\hat{w}_{\boldsymbol{k}},\hat{\theta}_{\boldsymbol{k}}\}= \frac{a}{R\,k^2} \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2^2 + \frac{2a}{R} \lVert \hat{w}'_{\boldsymbol{k}} \rVert_2^2 + \frac{ak^2}{R}\lVert \hat{w}_{\boldsymbol{k}} \rVert_2^2 + b \lVert \hat{\theta}'_{\boldsymbol{k}}\rVert_2^2  + b k^2\lVert \hat{\theta}_{\boldsymbol{k}} \rVert_2^2  \\ - \int^{1}_0 \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{\hat{w}_{\boldsymbol{k}} \hat{\theta}^*_{\boldsymbol{k}} \}  \textrm{d}z \geq 0.
\end{multline}
%
Standard arguments \citep{Arslan2021,Arslan2021a} imply that one can assume that $\hat{w}_{\boldsymbol{k}}$ and $\hat{\theta}_{\boldsymbol{k}}$ to be real-valued functions. 

Ensuring that $\mathcal{S}_{\boldsymbol{k}} \geq 0$ for any functions $\hat{w}_{\boldsymbol{k}}(z), \hat{\theta}_{\boldsymbol{k}}(z)$ satisfying the boundary conditions 
%
\begin{subequations} 
\begin{gather}
    \label{bc:w_k}
    \hat{w}_{\boldsymbol{k}}(0) = \hat{w}_{\boldsymbol{k}}(1)= \hat{w}_{\boldsymbol{k}}'(0)= \hat{w}_{\boldsymbol{k}}'(1)=0,\\
    \label{bc:T_k}
     \hat{\theta}_{\boldsymbol{k}}'(0) =  \hat{\theta}_{\boldsymbol{k}}'(1) =0,
\end{gather}
\end{subequations}
%
is commonly referred to as a {\em spectral constraint} at wavenumber $\boldsymbol{k}$. The right-hand side of \eqref{eq:s_f_f} is non-negative if the spectral constraint is satisfied for each wavenumber $\boldsymbol{k} \in \mathbb{N}_{0}$. This, in turn, implies the desired property that $\mathcal{S}(\boldsymbol{u},\theta) \geq 0$ for any solution to the governing equations. It then follows from \eqref{eq:AFM_statemen} that $\langle wT \rangle \leq U$ for any solution of the governing equations, where $U$ is the scalar appearing in the equation \eqref{eq:S0} for the spectral constraint at wavenumber $\boldsymbol{k}=0$.

The simple structure of the spectral constraint at wavenumber $\boldsymbol{k}=0$ can give useful information on the upper bound $U$ that can be proven using the auxiliary function method. In particular, if $a,b,\phi(z)$ can be chosen so that the spectral constraints $ \mathcal{S}_{\boldsymbol{k}}\{\hat{w}_{\boldsymbol{k}},\hat{\theta}_{\boldsymbol{k}}\}  \geq 0$ holds for all non-zero wavenumbers, then it is possible to prove a bound and the numerical value of the best provable bound $U$ can be found by minimising \eqref{eq:S0} over functions $\hat{\theta}_{\boldsymbol{0}}$ that satisfy the boundary conditions \eqref{bc:T_k} at $\boldsymbol{k}=0$. This gives a best provable bound (after fixing $\phi(z),a$ and $b$) of 
}
\begin{equation}
    \label{eq:U_bound}
    U = \int^{1}_{0}\frac{\phi'(z)^2}{4b}\textrm{d}z.
\end{equation}
{\color{matlabred} Although the parameter $a$ does not appear in \eqref{eq:U_bound}, there is an implicit interplay between $a$ and $\phi(z)$ since, given \eqref{eq:sk_non_uni}, both must be chosen appropriately if the spectral constraint at non-zero wavenumbers is to be satisfied. This is clarified in \S \ref{sec:spectral}.

Finding a good bound within the auxiliary function method then corresponds to identifying $a,b$ and $\phi(z)$, which satisfy the spectral constraints for positive wavenumbers while keeping the value of $U$ given by \eqref{eq:U_bound} as small as possible. }



\subsection{Enforcing the spectral constraint for non-zero wavenumbers}
\label{sec:spectral}

{\color{matlabred} Recall that the cumulative heating function $\eta(z) \in L^2(0,1)$ is given by \eqref{eq:eta_general} and that $\eta(z)$ is an increasing function satisfying $\eta(0)=0$ and $\eta(1)=1$. The aim now is to find parameters $a,b, \phi(z)$ such that the spectral constraints $\mathcal{S}_{\boldsymbol{k}}\{\hat{w}_{\boldsymbol{k}},\hat{\theta}_{\boldsymbol{k}}\} \geq 0$ hold for every non-zero wavenumber $\boldsymbol{k}$. To this end,} we choose the background field as
    \begin{equation}
	 \phi'(z) = \frac{(a+1)}{\lVert \eta \rVert_2}
        \begin{dcases}
            0, &  0\leq z \leq \delta, \\
            \eta(z) + \lVert \eta \rVert_2,  &  \delta \leq z \leq 1-\delta,\\
            0,& 1-\delta \leq z \leq 1,
        \end{dcases}
    \label{eq:phi_prime}
    \end{equation}
    where $\delta \leq \frac12$ is the width of the boundary layers of $\phi'(z)$. We also set
\begin{equation}
    \label{eq:b_relation}
    b = \frac{a+1}{\lVert \eta \rVert_2}.
\end{equation}

{\color{matlabred} 
The motivation for these parameter choices is as follows. The background field $\phi(z)$ is chosen such that in the `bulk region' $\delta \leq z \leq 1-\delta$, the term $(a+1+b\eta(z) - \phi'(z))$ appearing in the final, sign-indefinite, integral of \eqref{eq:sk_non_uni} is identically equal to zero. Consequently, to verify the spectral constraint $ \mathcal{S}_{\boldsymbol{k}}\{\hat{w}_{\boldsymbol{k}},\hat{\theta}_{\boldsymbol{k}}\} \geq 0$ we only need to estimate the final integral term in \eqref{eq:sk_non_uni} for integrals over only the `boundary layers' $0 \leq z \leq \delta$ and $1-\delta \leq z \leq 1$. As we show below this can be achieved by using standard functional estimates that exploit the boundary conditions \eqref{bc:w_k} and \eqref{bc:T_k}. 

In the boundary layers,  for simplicity, $\phi'(z)$ is chosen to be zero to satisfy the assumed boundary conditions on $\phi(z)$ and give no detrimental contribution to the bound $U$ in \eqref{eq:U_bound}. Once these choices have been made, the key parameter is the boundary layer width $\delta$, and there is a natural tension in that a large value of $\delta$ improves (reduces) the bound $U$ but makes verification of the spectral constraint increasingly difficult (see \eqref{eq:sk_cond_ineq}). 

Finally, the motivation for the choice of $b$ comes from the fact that for the case of uniform heating (where  $\eta(z)=z$ and $\| \eta \|_2 = 1/\sqrt{3}$) previous work \citep{Arslan2021a} reveals that as $R$ increases $a$ decreases to zero whereas $b\rightarrow\sqrt{3}$. The choice \eqref{eq:b_relation} respects this relation and maintains algebraic simplicity in the following derivations. } 


We begin by formulating a simpler sufficient condition for the spectral constraint \eqref{eq:sk_non_uni} to hold. First, we drop the positive terms in $\hat{w}_{\boldsymbol{k}}'(z)$, $\hat{w}_{\boldsymbol{k}}(z)$ and $\hat{\theta}'_{\boldsymbol{k}}(z)$. Then, we plug in our choices \eqref{eq:phi_prime} for $\phi'(z)$ and \eqref{eq:b_relation} for $b$, and use the inequality $\eta(z)\leq 1$ to conclude that \eqref{eq:sk_non_uni} holds if 
\begin{equation}
    \label{eq:sk-cond_2}
    \frac{a}{R k^2} \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2^2 - \frac{a+1}{\lVert \eta \rVert_2} (1+\lVert \eta \rVert_2)  \int_{(0,\delta)\cup(1-\delta,1)} |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \geq 0.
\end{equation}
Note that the boundary layers $(0,\delta)$ and $(1-\delta,1)$ are disjoint because $\delta\leq \tfrac12$ by assumption.

Next, given the boundary conditions on $w_{\boldsymbol{k}}(z)$ from \eqref{bc:w_k}, the use of the fundamental theorem of calculus and the Cauchy-Schwarz inequality gives
\begin{equation}
\label{eq:w_estimate}
     \hat{w}_{\boldsymbol{k}}(z) = \int^{z}_0 \int^{\xi}_0 \hat{w}_{\boldsymbol{k}}''(\sigma) \textrm{d}\sigma \textrm{d}\xi \leq \int^{z}_0 \sqrt{\xi} \, \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_{2} \,\textrm{d}\xi  = \frac23 z^\frac32\, \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2.
\end{equation}
Using \eqref{eq:w_estimate} and the Cauchy-Schwarz inequality, we can estimate
\begin{align}
     \int_0^\delta | \hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \leq  \int_0^\delta |\hat{w}_{\boldsymbol{k}}| |\hat{\theta}_{\boldsymbol{k}}| \textrm{d}z
     \leq \frac23 \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2\int_0^\delta
     z^{\frac32} \, |\hat{\theta}_{\boldsymbol{k}}| \textrm{d}z 
     &\leq \frac23 \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2 \lVert \hat{\theta}_{\boldsymbol{k}} \rVert_2\left( \int^{\delta}_0 z^3 \textrm{d}z \right)^{\frac12} \nonumber \\
     &=\frac{\delta^2}{3}  \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2 \lVert \hat{\theta}_{\boldsymbol{k}} \rVert_2 . 
 \end{align}
 The same estimate applies to $\int_{1-\delta}^1 |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z$, so we conclude that \cref{eq:sk-cond_2} holds if
\begin{equation}
    \frac{a}{R k^2} \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2^2 - \frac{2(a+1)}{3 \lVert \eta \rVert_2} (1+\lVert \eta \rVert_2 ) \delta^2  \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2\lVert \hat{\theta}_{\boldsymbol{k}} \rVert_2    \geq 0.
\end{equation}
The left-hand side of this inequality is a homogeneous quadratic form in $\lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2$ and $\lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2$ and it is non-negative if it has a nonpositive discriminant. Therefore, the spectral constraint is satisfied if
\begin{equation}
    \label{eq:sk_cond_ineq}
    \delta^4 \leq \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) (1+\lVert \eta \rVert_2)^2 R }.
\end{equation}

\subsection{Estimating the bound}
\label{sec:eval_b}

Next, we estimate the bound $U$ in \eqref{eq:U_bound} given our ans\"{a}tze \eqref{eq:b_relation} and \eqref{eq:phi_prime}. Making use of the fact that $\eta(z)\geq 0$ gives, after rearranging,  
\begin{align}
    U &=
    \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z
    \nonumber \\
    &= \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1}_{0}\left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z 
    - \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int_{(0,\delta) \cup (1-\delta,1)} \left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z
    \nonumber \\
    &\leq 
   \frac12 (a+1)  \left( \lVert \eta \rVert_2 + \lVert \eta \rVert_1 -  \lVert \eta \rVert_2 \delta \right).
     \label{eq:U_form_sub}
\end{align}
By definition, $a$ is real and positive, which means that $(a+1)^m\geq1$ for all $m>0$. Therefore,
taking $\delta$ as large as possible in \eqref{eq:sk_cond_ineq} and substituting into \eqref{eq:U_form_sub} gives,
\begin{align}
    U &\leq   \frac12 (a+1)  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1) 
    - \frac{\sqrt{3}}{2} \frac{\lVert\eta\rVert_2^{5/4}}{(1+\lVert\eta\rVert_2)^{1/2}}(a+1)^{3/4} a^{1/4} R^{-1/4}  \nonumber\\
    &\leq   \frac12 (a+1)  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1) 
    - \frac{\sqrt{3}}{2} \frac{\lVert\eta\rVert_2^{5/4}}{(1+\lVert\eta\rVert_2)^{1/2}} a^{1/4} R^{-1/4} .
    \label{eq:U_delt_sub}
\end{align}
We now minimise the last expression in \eqref{eq:U_delt_sub} over $a$ to obtain the best possible estimate on $U$. The optimal choice of $a$ is
\begin{equation}
    a^* =  \frac{a_0 \lVert \eta \rVert_2^{5/3}}{ (\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{4/3} (1+\lVert \eta \rVert_2 )^{2/3}} R^{-1/3},
\end{equation}
where $a_0 = (\frac{9}{256})^{1/3}$. Finally, substituting for $a$ in \eqref{eq:U_delt_sub}, rearranging, and since  $\mean{w\theta} \leq U$, we get
\begin{equation}
    \mean{w \theta} \leq  \frac12  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1)  -  \frac{a_1 \lVert \eta \rVert_2^{5/3}}{(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{1/3}(1+\lVert \eta \rVert_2)^{2/3} } R^{-1/3},
\end{equation}
where $a_1 = \frac{3\sqrt{3}}{8} a_0^{1/4} $.
Then, by \eqref{eq:energy_bal_nu}, 
\begin{equation}
    \label{eq:dT_bound_simple}
    \dT \geq   -\underbrace{\frac12  ( \lVert \eta \rVert_2 - \lVert \eta \rVert_1)}_{\mu}  +  \underbrace{\frac{a_1 \lVert \eta \rVert_2^{5/3}}{(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{1/3}(1+\lVert \eta \rVert_2)^{2/3} }}_{\sigma} R^{-1/3},
\end{equation}
completing the proof of \eqref{eq:main_res} {\color{matlabred} for the $\eta$-dependent values of $\mu$ and $\sigma$ indicated in \eqref{eq:dT_bound_simple}. 

Finally, we must also check that requirement that the choice of $\delta$ in the above argument via \eqref{eq:sk_cond_ineq} satisfies the constraint $\delta\leq \frac12$ to ensure that the two boundary layers do not interact.  This gives a minimum Rayleigh number $R=R_m$ above which the final bound \eqref{eq:dT_bound_simple} holds. With $\delta$ defined by \eqref{eq:sk_cond_ineq}, it follows that 
\begin{equation}
    R_m = \frac{18 \lVert \eta \rVert_2^{2} }{(\lVert \eta \rVert_1 + \lVert \eta \rVert_2)(1+ \lVert \eta \rVert_2)^2}.
\end{equation}

In practice, this does not place a strong restriction on our results. For example, consider the case of uniform heating where $H(z)=1$. Here, one has $\eta(z)=z$ and obtains from  \eqref{eq:dT_bound_simple} the lower bound $\dT \geq -0.03868 + 0.1850 R^{-1/3}$, valid for all $R\geq R_m =2.2384$ which is far below the critical Rayleigh number for linear instability of $R=1440$. The bound matches the scaling and asymptote of \cite{Arslan2021a}. The difference in the constant multiplying the $O(R^{-1/3})$ term is due to the choice taken in \cite{Arslan2021a} of a $\phi'(z)$ with linear (rather than constant) boundary layers. To obtain as simple a bound as possible in\eqref{eq:dT_bound_simple}, the constant multiplying the $R$ scaling was not optimised in this work.}


\section{Implications of the bound}
\label{sec:Imp_bound}
{\color{matlabred} Inequality \eqref{eq:dT_bound_simple} states that $\dT < 0$ (i.e downward conduction) is impossible for Rayleigh numbers $R$ satisfying  
%
\begin{equation}
    R_m \leq R \leq R_0 := \frac{8a_1^3 \lVert \eta \rVert_2^5 }{(1+\lVert \eta \rVert_2)^2(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)(\lVert \eta \rVert_2 - \lVert \eta \rVert_1)^3}\, .
    \label{eq:Rc_g}
\end{equation}%
The above expression for $R_0$ is obtained simply by setting the right-hand-side of \eqref{eq:dT_bound_simple} to zero. The magnitude of $R_0$ is plotted as a function of $\lVert \eta \rVert_1$ and $\lVert \eta \rVert_2$ in \cref{fig:main_res}. The domain of the function shown in \cref{fig:main_res} respects the fact that 
%
\begin{equation} \label{eq:eta_ineqs}
\|\eta\|_1 \leq \|\eta\|_2 \leq \sqrt{ \|\eta\|_1} \, ,
\end{equation}
%
for any increasing function $\eta(z)$ satisfying $\eta(0)=0$ and $\eta(1)=1$. The lower bound follows from the Cauchy-Schwarz inequality, while the upper bound is a simple consequence of $\eta(z) \leq 1$ for any $0 \leq z \leq 1$. 

An important implication of these inequalities is that $\mu = -\frac12 (\|\eta\|_2 - \|\eta\|_1)$ is strictly negative unless $\|\eta\|_2 = \|\eta\|_1$. When  $\mu$ is strictly negative, the corresponding value of $R_0$ is finite, meaning that there is a maximum Rayleigh number (indicated in \cref{fig:main_res}) up to which downward conduction can be ruled out. Given this observation, it is natural to ask whether there are fixed heating profiles for which $\|\eta\|_2=\|\eta\|_1$, then one could provably eliminate the possibility of downward conduction for arbitrarily large Rayleigh numbers. Interestingly, given the restrictions that $\eta(0)=0$ and $\eta(1)=1$, this is only possible in the limiting case that $H(z)$ is a single Dirac measure of unit heating at the lower boundary $z=0$. 
}

% AW: I don't get the point of this "two Dirac" thing. Have deleted this. 
%
% {\color{matlabred}The set of valid functions $\eta(z)$ can be further restricted}. 
%According to \eqref{eq:dT_bound_simple}, only for heating profiles for which $\|\eta\|_{1}=\|\eta\|_{2}$ is it possible to guarantee that $\dT>0$ for all $R$. However, noting that $\eta(z)$ increases monotonically with respect to $z$, $\eta(0)=0$ and $\eta(1)=1$ then,
%\begin{equation}
%    \lVert \eta \rVert_2^2 = \lVert \eta^2 \rVert_1 < \lVert \eta \rVert_1. 
%    \label{eq:eta_L2_bounds}
%\end{equation}
%Within the class of heating profiles, we have considered, \eqref{eq:eta_L2_bounds} gives an upper bound on $\lVert \eta \rVert_2$ and rules out the possibility that there is a heating profile for which $\dT>0\ \forall R$. Taking $H$ as a distribution rather than a function, then $\|\eta\|_{1}=\|\eta\|_{2}$ would correspond to the set of distributions consisting of two (not necessarily equal) finite amounts of heat, represented as Dirac measures at $z=0$ and $z=1$. 

\begin{figure}
    \centering
    \hspace{-1cm}
    \includegraphics[scale=1]{fig/myVectorFile.eps}
     \begin{tikzpicture}[overlay]
        \node at (-12,8.4) {\textit{(a)}};
       \node at (-4.5,6.7) {\textit{(b)}};
        \node at (-12,2.7) {\textit{(c)}};
        \node at (-8.8,2.7) {\textit{(d)}};
       \node at (-5.9,2.7) {\textit{(e)}};
       \node at (-3,2.7) {\textit{(f)}};
    \end{tikzpicture}
    \caption{\textit{(a)} Contour plot of $R_0$ as given in \eqref{eq:Rc_g} with the inset \textit{(b)} highlighting a region ($[0.925,1]\times[0.95,1]$) where $\lVert \eta\rVert_1 \sim \lVert \eta \rVert_2$. In panel \textit{(a)} the green cross (\mycross{matlabgreen}) highlights uniform heating, drawn in \textit{(c)}, the blue cross (\mycross{matlabblue}) highlights heating near the lower boundary drawn in \textit{(d)}, the yellow cross (\mycross{matlabyellow}) highlights heating near the upper boundary \textit{(e)} and the black cross (\mycross{black}) highlights sinusoidal heating, panel \textit{(f)}. }
    \label{fig:main_res}
\end{figure}


% AW: I'm not sure I agree that || \eta ||_1= || \eta ||_2 unless the dirac is at z=0. Deleted this. 
%
%A further restriction on the possible values of $\|\eta\|_{1}$ and $\|\eta\|_{2}$ comes from the Cauchy-Schwarz inequality $\|\eta\|_{1}\leq\|\eta\|_{2}$, which would be saturated by distributions consisting of a single Dirac measure of unit heat at some height $z\in[0,1]$. For the differentiable $\eta$ considered in this work, the inequality is strict,
%\begin{equation}
%    \lVert \eta \rVert_1 < \lVert \eta \rVert_2.
%    \label{eq:eta_L1_bounds}
%\end{equation}
%The open set of functions satisfying \eqref{eq:eta_L2_bounds} and \eqref{eq:eta_L1_bounds} is illustrated in figure \ref{fig:main_res}\textit{(a)}.



The inequality in \eqref{eq:dT_bound_simple} applies to all heating profiles that can be specified as a function of $z$ and integrated to unity. Figure \ref{fig:main_res} \textit{(a)}  is a contour plot of the critical $R_0$ over the open region satisfying the inequalities \eqref{eq:eta_ineqs}. Examples of non-uniform heating profiles from \cref{fig:config2} appear in \cref{fig:main_res} for cases in which the heating is \textit{(d)} near the bottom boundary, \textit{(e)} near the upper boundary and \textit{(f)} sinusoidal, with the corresponding value of $R_0$ highlighted with crosses in \cref{fig:main_res} \textit{(a)}. {\color{matlabred} The profiles \textit{(c)}-\textit{(f)} and their corresponding $R_0$ can be compared to physical examples of IHC, but before doing so, we note that the precise values of $R_0$ computed in \cref{fig:main_res} are not as important as the relative magnitudes of $R_0$.  


The bounds we obtain can help justify physical observations. 
In the case of mantle convection, it is difficult to accurately determine the distribution of the radioactive heating sources is unknown, and the Rayleigh number (but is believed to be of the order $10^6$ to $10^8$ \citep{schubert2015treatise}). However, a higher concentration of the heat in the upper mantle, in comparison to a uniform distribution, will give rise to smaller $R_0$ and a smaller magnitude of $\dT$ that would align with the observation of the slower-than-expected cooling rate of the Earth interior \citep{JAUPART2015223}. Alternatively, convection in the Sun resembles heating similar to \textit{(d)}, of distributed heating near the lower regions of the convective zone. Heating concentrated at the bottom of the domain, as seen in \cref{fig:main_res}, results in a value of $R_0$ much larger than the case of uniform heating. Moreover, for estimated Rayleigh numbers of $10^{22}$ \citep{schumacher2020}, downwards conduction can be ruled out for heating concentrated sufficiently closely to the lower boundary.


Finally, we demonstrate an application of the bounds obtained in this work. Instead of starting with a fixed $H(z)$ and asking for the corresponding $R_0$, we can instead take a given Rayleigh number, motivated by a geophysical or astrophysical flow, and for a family of $H(z)$ (\cref{fig:main_res} \textit{(d)} to \textit{(f)} are different one-parameter families of heating profiles) asses which heating profiles in that family guarantee that downwards conduction is ruled out. For example, taking \cref{fig:main_res}\textit{(c)} where heating is uniform in a region $(0,\epsilon)$ where $\epsilon\leq 1$, by our result in \eqref{eq:Rc_g} we can obtain a value for $R_0$ as $\epsilon$ decreases, as plotted in \cref{fig:Hbottom}\textit{(b)}. Then, for example, taking a Rayleigh number of $10^{22}$, our bound \eqref{eq:dT_bound_simple} indicates that downward conduction is impossible when the heating profile is such that $\epsilon < 1.366 \times 10^{-7}$ \cref{fig:Hbottom}\textit{(b)}. For the Sun, where the convective zone is estimated to be of the order of $0.713 R_{\odot}$ (where $R_{\odot}$ is the solar radius)\citep{miesch2005}, this corresponds to heating in a region of 6.8cm. Remark that $10^{22}$ is an estimated Rayleigh number that arises from including boundary and internal heating in the definition of $R$. For a well-chosen $R$, \eqref{eq:dT_bound_simple} has direct implications on physical flows, especially if one can establish the optimal constants in the $R$ scaling of \eqref{eq:dT_bound_simple}.
This exercise highlights the use of bounds to assess cases of internally heated convection in nature where downward conduction is ruled out.
}

\begin{figure}
    \centering
    \includegraphics{fig/H_b1.eps}
    \begin{tikzpicture}[overlay]
        \node at (-12.5,4.4) {\textit{(a)}};
       \node at (-6.2,4.4) {\textit{(b)}};
    \end{tikzpicture}
    \caption{ {\color{matlabred} Panel \textit{(a)} plots heating profiles $H(z)$, with mean one, where the heating is uniform in a region $(0,\epsilon)$ near the lower boundary  and zero elsewhere. In panel \textit{(a)} eight cases are plotted of $\epsilon \in [0.05,0.5]$, where $\epsilon = 0.05$ is in yellow ({\color{colorbar2}\solidrule}) and $\epsilon=0.5$ in black ({\color{black}\solidrule}) . Panel \textit{(b)} plots $\epsilon$ against $R_0$, the value below which downwards conduction is ruled out. The vertical dashed line (\dashedrule) corresponds to $\epsilon = 1.366 \times 10^{-7}$ intersecting the red line at $R_0=10^{22}$. For a given Rayleigh number (i.e. $10^{22}$) \textit{(b)} can be used to find the value of $\epsilon$ for heating profiles in \textit{(a)} below which downwards conduction is impossible. }}
    \label{fig:Hbottom}
\end{figure}


\section{Conclusion}
\label{sec:conclusion}

We have obtained lower bounds on the mean vertical conductive heat transport, $\dT$, for non-uniform internally heated convection between parallel plates with fixed flux thermal boundary conditions. The bounds are expressed in terms of a Rayleigh number and the mean vertical heat flux $\eta(z)$, corresponding to the prescribed internal heating $H(z)$ integrated upwards from the bottom boundary to a height $z$. In particular, we proved with the auxiliary functional method that $\dT \geq -\mu + \sigma R^{-1/3}$ in \eqref{eq:dT_bound_simple}, where $\mu, \sigma>0$. We were, therefore, able to obtain an explicit Rayleigh number $R_0$, in terms of $\eta(z)$, below which it is possible to guarantee that $\dT\geq 0$. The results are consistent with those obtained from the particular case of uniform internal heating ($\eta=z$) \citep{Arslan2021a}. As an addendum, while this paper only considers no-slip boundary conditions, by the arguments in \cite{Fantuzzi2018}, the same result of \eqref{eq:dT_bound_simple}, albeit with a different value of $a_1$, is obtained for stress-free boundary conditions. 


Only in the limit of heat being concentrated entirely at the bottom boundary is it possible to guarantee that $\dT \geq 0$ for all $R$ ($\mu=0$ in the previous paragraph). However, in a mathematical sense, such heating profiles are distributions rather than functions of $z$, lying beyond the scope of the internal heating profiles considered in this work and constitute the closure, of the open set of pairs $(\|\eta\|_{1}, \|\eta\|_{2})$ that determine $\mu$ and $\sigma$ (shown in figure \ref{fig:main_res}). In this regard, there is an intriguing connection with Rayleigh-B\'{e}nard convection, for which $\dT \geq 0$ for all $R$ \citep{Otero2002}.


While the auxiliary functional method provides a rigorous bound on $\dT$, it does not guarantee the existence of flows that saturate the bound or provide insight into the predominant physical processes responsible for extremising $\dT$. In other words, the question of whether there are solutions to the Boussinesq equations that produce negative mean vertical conductive heat transport ($\dT<0$) when $R>R_0$ remains an open and interesting problem to investigate in the future. A possible avenue for exploring this question is the method of optimal wall-to-wall transport \citep[][]{Tobasco2017}, which would yield a velocity field that minimises $\dT$ subject to a prescribed set of constraints, along with upper bounds on $\dT$. 

Finally, caution should be applied in interpreting the Rayleigh number used to study non-uniform IHC. Our Rayleigh number follows convention by defining temperature and length scales using the volume-averaged internal heating and domain height, respectively. However, in cases with heating concentrated towards the top of the domain, the physical interpretation of the Rayleigh number as quantifying the size of destabilising forces relative to the stabilising effects of diffusion is questionable. Although the choice of Rayleigh number is somewhat superficial, an appropriate choice might shed light on the dependence of the bounds on $R$ in terms of the underlying physics. Heating and cooling that is applied non-uniformly over the horizontal as well as vertical directions \citep[][]{Song2022} poses further challenges in this regard, and an opportunity to extend the results reported
in this work.




==> v1.tex <==
% \section{Introduction}
% \label{sec:intro}

% Fluids across a wide range of scales, transport heat by both conduction and convection. Thermal convection in particular occurs when  temperature gradients are of  sufficient size to induce instability in an otherwise motionless fluid. As the fluid is forced into motion by larger gradients, eventually, the convection becomes turbulent. Turbulent convection can on the one hand be driven purely by boundary heating, known as Rayleigh--B\'enard (RB) convection or by internal heating. 
% Whether it is convection in the interior of planets and the Earth's Mantle \citep{bercovici2011mantle,MantleConvectioninTerrestrialPlanets,schubert2001mantle} or in high opacity atmospheres like that of Venus \citep{tritton1975internally,schubert_etal,moroz1981atmosphere}, an understanding of internally heated (IH) convection is key to understanding geophysical fluid dynamics.        

% The main question in both IH an RB convection is the variation of the vertical heat transport by conduction and convection as the heating strength, determined by the non-dimensional Rayleigh number ($Ra$ for RB and $R$ for IH convection), is increased. See \cite{Goluskin2016book} for a review of both. While both types of convection have been studied with computational and experiments, inferences on the mean vertical convective and conductive heat transport are limited by the range of parameters that can be spanned in computation. Instead, it is of greater interest to know the scaling of the mean vertical convective and conductive heat transport $\mean{wT}$ and  $\mean{\delta T}$ for all $R$. Here $\mean{\cdot}$ denotes the infinite time and volume average of the quantity of interest. While heuristic scaling arguments exist for both RB \citep{GroSjfm2000a,stevens2013} and IH \citep{Wang2020,creyssels_2021} convection, we require verification of the proposed scaling arguments. This can be achieved through a rigorous investigation of the underlying equations, without recourse to unproven assumptions.     


% One quantity of relevance for both types of convection is the Nusselt number $Nu$, a non-dimensional number that quantifies the enhancement of vertical heat transport due to convection. For RB convection heuristic arguments suggest two probable scaling behaviours for $Nu$ with respect to $Ra$ \citep{doering2020turning}. Based off the idea that thermal boundary layers are the limiting factor of heat transport \cite{Malkus1954} and \cite{priestley1954vertical} independently first proposed that $Nu \sim Ra^{1/3}$, known as the classical scaling regime. This scaling has since been observed in experiments and simulations \citep{iyer2020classical, bailon2010,vieweg2021,Johnston2009,silano2010}. On the other hand another if instead heat transport is limited by the free-fall velocity in the bulk of the fluid then \cite{spiegel1963generalization} demonstrated that $Nu \sim Ra^{1/2}$. This ultimate scaling regime has since been proven rigorously to be an upper bound on $Nu$ \citep{Doering1996,Otero2002,Kerswell2001}. In IH convection the situation is different. No single clear Nusselt can be defined for all IH convection problems and instead the enhancement of the heat transport due to convection can be evaluated with different quantities based on the thermal boundary conditions prescribed \citep{Goluskin2016book}. In the case of isothermal boundaries held at the same temperature, with uniform internal heating, heuristic arguments suggest two possible scaling laws for the convective heat transport of $\mean{wT} \sim \frac12 - R^{-1/4} $ or $\mean{wT} \sim \frac12 - R^{-1/3}$, corresponding to the classical or ultimate regime respectively \citep{Arslan2021}. A number of scaling arguments have also been proposed for alternative response parameters \citep{creyssels_2021,Wang2020}.       

% Rigorous upper and lower bounds have been proven for uniform IH convection on $\mean{T}$ and $\mean{wT}$, by use of the \textit{background field method} \citep{Doering1994,Doering1996,constantin1995dissipative}. The method can be seen as a particular case of a broader framework for bounding time-averages referred to as the \textit{auxiliary functional method } \citep{Chernyshenko2022}. The method is known to yield sharp bounds for sufficiently well-posed ordinary and partial differential equations \citep{Tobasco2018,Rosa2020}.   
% With the auxiliary functional method a variational principle is utilised to formulate a convex optimisation problem over the parameters in a quadratic functional $\mathcal{V}$ of the velocity $\boldsymbol{u}$ and temperature $T$ \citep{Chernyshenko2014a,Goluskin2019}. This method has seen successful application to a wide range of fluid flows, see \cite{Fantuzzi2022} for an extensive review. Often, the results are proven by utilising additional information from the governing equations in the form of minimum/maximum principles. Indeed for RB convection additional information can be used to prove the classical scaling regime given that Prandtl number, $Pr$ is larger than $Ra^{1/3}$ \citep{choffrut2016upper,Seis2015}, where $Pr$ is the non-dimensional ratio of the viscous and thermal diffusivities.  
% Indeed, for uniform IH convection use of a minimum principle was critical to obtaining any bounds on $\mean{wT}$ that scaled with $R$ \citep{Arslan2021,kumar2021ihc,Arslan2023}.      


% The majority of previous studies either consider RB convection or uniform IH convection. In recent years, interest in non-uniform internally heated/cooled (NIHC) convection has provided insight into both models of thermal convection \citep{kazemi2022,Miquel2019,Bouillaut2019,Tobasco2022,Song2022}. Varying the region of heating, and even allowing for cooling, allows for an investigation of different regimes of heat transport due to turbulence. In fact, simulations and experiments \citep{Lepot2018,kazemi2022} demonstrate that heat transport can be enhanced if the heating is modified from near the lower boundary to being
% distributed within the bulk of the domain. Having a non-uniform heat source could be arranged (and viewed) as interpolating between boundary driven Rayleigh-B\'enard and internally heated convection. However, the exact nature of such an interpolation of the underlying PDEs remains unclear. In this paper we utilise a non-uniform heating/cooling profile to investigate IH convection when the upper and lower boundaries are poor thermal conductors. 



% In uniform IH convection between poorly conducting boundaries $\mean{T}$ has been studied in \cite{Goluskin2015a} and $\mean{wT}$ (and by extension $\mean{\delta T}$) in \cite{Arslan2021a}. When the lower boundary is taken to be a thermal insulator, the removal of the stably stratified boundary layer removes much of the difficulty associated with convection driven by internal heating. Additionally, combining this with a heating profile that varies in the vertical direction allows for the means to directly interpolate between the original convective systems. In particular \cite{Arslan2021a} demonstrated lower bounds on $\mean{\delta T}$, that implied conductive heat transport from the top to the bottom could not be ruled for arbitrarily large $R$. The key question of this work is to ask if the downwards conductive heat flux can be minimised, and in fact demonstrably zero, with internal heating/cooling that is non-uniform.



% \begin{figure}
%     \centering
%     \begin{tikzpicture}[every node/.style={scale=0.95}]
%     \draw[black,thick] (-6,0) -- (-2,0) node [anchor=west] {$z=0$};
%     \draw[black,thick] (-6,1.8) -- (-2,1.8) node [anchor = west] {$z=1$};
%     % \draw[<->,black,dashed] (-5.7,0.15) -- (-5.7,1.85) node at (-5.9,1){$d$};
%     % \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(2.5,1.8) (3.5,0.9) (3.8,0)};
%     % \draw [colorbar10] plot [smooth, tension =1] coordinates {(2.5,1.8) (2.9,1.5) (3.1,1.27)};
%     % \draw [colorbar10] (3.1,1.27) -- (3.1,0);
%     \node at (1.25,-0.25) {$ \partial_z T = 0 $};
%     \node at (1.25,2.025) {$ \partial_z T = 0 $};
%     % \node at (-4.75,0.9) { IH };
%     \draw[->,colorbar10] (-3.5,0) -- (-3.5,0.45) node [anchor = east]{$z$};
%     \draw[->,colorbar10] (-3.5,0) -- (-3,0) node [anchor=north]{$H$};
%     \draw[->] (-6.8,0) -- (-6.8,0.36) node [anchor=east]{$z$};
%     \draw[->] (-6.8,0) -- (-6.4,0) node [anchor=north]{$x$};
%     \draw[->] (-6.8,0) -- (-6.5,0.18) node [anchor=west]{$y$};
%     \draw[black,thick] (0,0) -- (4,0) node [anchor=west] {$z=0$};
%     \draw[black,thick] (0,1.8) -- (4,1.8) node [anchor = west] {$z=1$};
%     % \draw[<->,black,dashed] (0.3,0.15) -- (0.3,1.85) node at (0.1,1){$d$};
%     \node at (-4.75,-0.25) {$ \partial T = 0 $};
%     \node at (-4.75,2.025) {$  \partial T = -1 $};
%     % \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(-3.5,1.8) (-2,0.9) (-3.5,0)};
%     % \draw [colorbar10] plot [smooth,tension=1] coordinates {(-3.5,1.8) (-3.05,1.73) (-2.9,1.67)};
%     % \draw [colorbar10] (-2.9,1.67) -- (-2.9,0.315);
%     % \draw [colorbar10] plot [smooth, tension =1] coordinates {(-2.9,0.315) (-3.05,0.18) (-3.5,0)};
%     \draw [dotted,colorbar10] (-3.5,0) -- (-3.5,1.8) ;
%     \draw[->,colorbar10] (3,0) -- (3,0.45) node [anchor = east]{$z$};
%     \draw [dotted,colorbar10] (3,0) -- (3,1.8) ;
%     \draw[->,colorbar10] (3,0) -- (3.5,0) node [anchor=north]{$H$};
%     % \node at (1.25,0.9) {\textrm{IH}};
%     \node at (-6.4,1.8) {\textit{(a)}};
%     \node at (-0.4,1.8) {\textit{(b)}};
%     \end{tikzpicture}
%     \caption{placeholder.}
%     \label{fig:config}
% \end{figure}


\section{Setup}
\label{sec:setup}

We consider a layer of fluid bounded between two horizontal plates separated by a distance $d$ heated non-uniformly internally. The dimensional heating is given by $\Tilde{H}=H_0 H(z)$ where $H_0$ is the volumetric heating rate while $H(z)$ is a $z$-dependent function representing the heating or cooling. For simplicity the layer is periodic in the horizontal ($x$ and $y$) directions with periods $L_x$ and $L_y$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$.     

To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2H_0/\kappa \rho c_p$ as the temperature scale. The motion of the fluid in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ is then governed by the Boussinesq equations
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
Notice that if we wanted to increase the generality of the argument we could consider non-uniform heating which varies in all three spatial directions $H(\boldsymbol{x})$. The non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa}, \quad R = \frac{g \alpha H_0 d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}

It will be convenient to introduce the function,
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z) \textrm{d}z,
\end{equation}
which is a measure of the potential energy in the system.
In this section we take the boundary conditions to be no-slip and fixed flux,
\begin{subequations}
\label{bc:non_uni}
\begin{align}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:T_f}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-\eta(1).
\end{align}
\end{subequations} 
For a statistically stationary state to be achieved we could make the following two choices for the temperature boundary condition at the top: (i) mean one heating/cooling in the domain $\eta(1)=1$ (ii) mean zero heating/cooling in the domain $\eta(1)=0$.
% \begin{itemize}
%     \item[1.] mean one heating/cooling in the domain, $\eta(1) = 1$. 
%     \item[2.] mean zero heating/cooling in the domain, $\eta(1) = 0$.
% \end{itemize}

We can evaluate the energy balance of the system by taking $\mean{z\cdot \eqref{eq:nondim_energy_nonUniform}}$, by making use of \eqref{eq:eta_general},  \eqref{bc:T_f} and integrating by parts to obtain
\begin{align}   
\label{eq:energy_bal_nu}
    \mean{wT} + \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}} &= \volav{\eta(z)}.
    % - \overline{\horav{\partial_z T|_{z=1}}} - \volav{z\, H(z)}\nonumber \\ &= \volav{\eta(z)} - \eta(1) - \overline{\horav{\partial_z T|_{z=1}}} \nonumber\\ & = \volav{\eta(z)} .
\end{align}
The left hand side of \eqref{eq:energy_bal_nu} is the sum of the mean heat flux due to convection, $\mean{wT}$ and conduction $\mean{\delta T} = \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}}  $ . 
If the internal heating were to be uniform, ie $\eta=z$, then the problem reduces to that presented in \cite{Arslan2021a} where $\mean{wT} + \mean{\delta T} = \frac12$. 

In the case where $\eta(1)=1$ the boundary conditions are inhomogeneous and so it will be convenient to rewrite the temperature field in terms of perturbations and the conductive profile,
\begin{equation}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
% It follows that the mean vertical convective heat transport holds the relation, $\mean{wT} = \mean{w\theta}$. 
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition it is apparent that
\begin{equation}
    T'_c = - \eta(z).
\end{equation}
Writing \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ gives
\begin{eqnarray}
     \partial_t \theta + \boldsymbol{u} \cdot \nabla \theta = \Delta \theta + w\, \eta(z) ,
\end{eqnarray}
where $\theta$ has boundary conditions
\begin{equation}
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{equation}

The Nusselt number can be defined in terms of the ratio of overall heat transport to mean conductive heat transport. In terms of $\eta(z)$, for non-uniform heating this becomes
\begin{equation}
    \label{eq:Nu_non_u}
    Nu = \frac{\mean{\delta T }  + \mean{wT}}{ \mean{\delta T } } = \frac{\volav{\eta(z)}}{\volav{ \eta(z)} \, - \mean{wT}} \, .
\end{equation}


\section{Linear and energy stability}
\label{sec:stability}

% Since the static state $T_c = \int -\eta(z)\textrm{d}z + C$, where $C$ can be arbitrarily chosen. One can take $C=\frac12$ without loss of generality. 

The linear and nonlinear stability of the flow can be determined as has already been demonstrated for the case of $\eta=z$ and $H=1$ in \cite{Goluskin2015a}. Due to the thermal boundary conditions the problem is unstable for all $k$, thus an asymptotic analysis can be carried out to analytically determine the $R$ for linear and nonlinear stability. The expressions for the linear and nonlinear stability for non-uniform heating profiles are 
\begin{equation}
\tag{\theequation\textit{a,b}}
     R_L = \frac{1}{\int^{1}_0 \eta(z) P(z) \textrm{d}z }, \qquad
    R_E = \frac{2}{\int^{1}_0 (\frac{1}{\gamma} + \eta(z)) Q(z) \textrm{d}z}, \label{eq:stab_lim}
\end{equation}
where $P(z)$ and $Q(z)$ are polynomials that satisfy the vertical velocity boundary conditions and where $P''''(z)=1$ and $Q'''' = \frac12 (1+\gamma z)$. For reference later the polynomials are
\begin{equation}
    P(z) = \frac{1}{24} (z^4 - 2z^3 + z^2), \quad  
    Q(z) = \frac{1}{240} (\gamma z^5 + 5z^4 -(3\gamma +10)z^3 + (2\gamma+5)z^2).
\end{equation}
$\gamma$ is a balance parameter, equivalent to $b$ in \eqref{eq:V_func}.

% that appears in the functional
% \begin{equation}
%     E_\gamma \left\{\boldsymbol{u},\theta \right\} = \frac12 \volav{\frac{1}{Pr\,R}|\boldsymbol{u}|^2 + \gamma \theta^2}
% \end{equation}
% which is the functional used within the classical energy method to determine energy stability. The polynomial $P$ is 
% \begin{equation}
% P(z) = 
% % \begin{dcases}
% \frac{1}{24} (z^4 - 2z^3 + z^2), \\
%     % \frac{1}{24}(z^4 - 2z^3 + z), & \textrm{free-slip}.
% % \end{dcases}
% \end{equation}
% while for $Q$ we have
% \begin{equation}
% Q(z) = 
% % \begin{dcases}
% \frac{1}{240} (\gamma z^5 + 5z^4 -(3\gamma +10)z^3 + (2\gamma+5)z^2).
%     % \frac{1}{240}(\gamma z^5 + 5z^4 -(\tfrac{10}{3}\gamma +10)z^3 + (\tfrac73  \gamma+5)z^2), & \textrm{free-slip}.
% % \end{dcases}
% \end{equation}
% 
\section{Bounds on heat transport}
\label{sec:nonuni_bounds}

The main aim of this work is to demonstrate bounds on the heat transport for non-uniform heating profiles. This is achieved by an application of auxiliary functional method to prove an upper bound on $\mean{wT}$ and by extension $\mean{\delta T}$ through \eqref{eq:energy_bal_nu}. When taking quadratic auxiliary functions this methodology is known to be equivalent to the background field method \cite{Chernyshenko2022}. The quadratic auxiliary functional used is 
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},T\} = \volav{ \frac{a}{2 Pr \,R}|\boldsymbol{u}|^2 + \frac{b}{2} |\theta|^2 - \phi \theta }.
    \label{eq:V_func}
\end{equation}
where $a$ and $b$ are non-negative numbers referred to as balance parameters, while $\phi(z)$ is the background temperature field satisfying the same boundary conditions as $\theta$. Following the auxiliary functional methodology initially outlined in \cite{Arslan2021a} a minimization problem can be constructed for the upper bound $U$ on $\mean{wT}=\mean{w\theta}$. For brevity we omit the derivation here.
Using the fact that \eqref{eq:V_func} is bounded along solutions of the governing equations, the infinite time average of the time derivative of \eqref{eq:V_func} is zero. 
% Then it follows that
% \begin{eqnarray}
%     \mean{w\theta} &=& \overline{ \volav{w\theta} + \mathcal{L}\mathcal{V} } = U - \overline{U- \volav{w\theta} - \mathcal{L}\mathcal{V} } = U - \mathcal{S},
% \end{eqnarray}
% where $\mathcal{L}\mathcal{V}$ is the Lie derivative of \eqref{eq:V_func} over the governing equations \eqref{eq:gov_eqs}.
Then the upper bound $\mean{w\theta}\leq U$ is given provided
\begin{equation}
    \mathcal{S} := \volav{ \frac{a}{R} |\nabla \boldsymbol{u}|^2 + b |\nabla \theta|^2 - \left(a + 1 + b \eta(z)  - \phi' \right)w \theta - \phi'(z) \theta' + U } \geq 0
    \label{e:sc_nonuni}
\end{equation}
for all $\boldsymbol{u}$ and $\theta$ subject to the boundary conditions \eqref{bc:u_non_u} and \eqref{bc:theta_non_u} and incompressibility.
Exploiting horizontal periodicity we carry out a Fourier decomposition of fields $\boldsymbol{u}$ and $\theta$ and following an argument analogous to that used in \cite{Arslan2021a} obtain that  
\begin{equation}
    \label{eq:U_bound}
    U = \volav{ \frac{\phi'(z)^2}{4b} },
\end{equation}
while requiring that for all $\boldsymbol{k} \neq 0$, 
\begin{equation}
    \label{eq:sk_non_uni}
     \mathcal{S}_{\boldsymbol{k}} := \volav{  \frac{a|w''_{\boldsymbol{k}}(z)|^2}{R\,k^2}  + b |\theta'_{\boldsymbol{k}}(z)|^2 -  \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} (z)\theta^*_{\boldsymbol{k}}(z) \}  } \geq 0 .
\end{equation}

% can estimate $\mathcal{S}$ from below as 
% \begin{equation}
%     \mathcal{S} \geq \mathcal{S}_0 + \sum_{\boldsymbol{k}} \mathcal{S}_{\boldsymbol{k}}
% \end{equation}
% where
% \begin{align}
%     \label{eq:s0_non_uni}
%      \mathcal{S}_0 &:= \volav{ b |\theta'|^2 - \phi'(z) \theta' + U } ,  \\
%      \label{eq:sk_non_uni}
%      \mathcal{S}_{\boldsymbol{k}} &:= \Big\langle \frac{ a }{R} \Big( \frac{|w''_{\boldsymbol{k}}|^2}{k^2} + 2|w'_{\boldsymbol{k}}|^2 + k^2 |w_{\boldsymbol{k}}|^2 \Big) + b |\theta'_{\boldsymbol{k}}|^2 + b k^2 |\theta_{\boldsymbol{k}}|^2  \nonumber\\
%     & \hspace{3cm} -  \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} \theta^*_{\boldsymbol{k}} \}  \Big\rangle  \quad \forall \boldsymbol{k} \neq 0.
% \end{align}
% The condition $\mathcal{S}\geq0$ can be shown to hold if both $\mathcal{S}_0$ and $\mathcal{S}_{\boldsymbol{k}}$ are independently non-negative.
% % are sufficient for \eqref{e:sc_nonuni} to hold for all $\boldsymbol{u}$ and $\theta$.
% As shown in \cite{Arslan2021a} the non-negativity of \eqref{eq:s0_non_uni} is ensured by taking
% \begin{equation}
%     \label{eq:U_bound}
%     U = \volav{ \frac{\phi'(z)^2}{4b} }.
% \end{equation}

\subsection{Uniform upper bound}
With the non-uniform heating given by $H(z)$, we first investigate the uniform in $R$ and $Pr$ upper bound on $\mean{w\theta}$, which we denote $U_0$.  

Making the choices, $a =0$ and $\phi'(z) = 1+ b \eta(z)$ guarantees that $\mathcal{S}_{\boldsymbol{k}} \geq 0 $ for all $\boldsymbol{k}\neq 0$. Then the choice of background profile substituted into \eqref{eq:U_bound} gives 
\begin{equation}
    U_0 = \volav{ \frac{(1+b\eta(z))^2}{4b} } = \frac{1}{4b} + \volav{  \frac{\eta(z)}{2} + \frac{b \eta^2(z)}{4} } ,
\end{equation}
which is optimised with the choice
\begin{equation}
    b = \frac{1}{  \lVert \eta \rVert_2 },
\end{equation}
such that
\begin{equation}
    \label{eq:U0_uni_upper_non}
    U_0 = \frac{1}{2} \lVert \eta \rVert_2 + \frac{1}{2} \volav{ \eta(z) }.
\end{equation}
Given \eqref{eq:energy_bal_nu}, the uniform upper bound implies that 
\begin{equation}
    \label{eq:delt_T_uni}
    \mean{\delta T} \geq \sigma := \frac12 \volav{\eta(z)} - \frac12 \lVert \eta \rVert_2.
\end{equation}
The aim is to seek $\eta(z)$ that demonstrates $\mean{\delta T} \geq 0$. The uniform upper bound on $\mean{w\theta}$ in \eqref{eq:U0_uni_upper_non} can also be substituted into the definition of $Nu$ in \eqref{eq:Nu_non_u} which gives
\begin{equation}
    \label{eq:Nu_non_uni}
    Nu \leq \frac{\volav{\eta(z)}}{\tfrac12\volav{\eta(z)} - \tfrac12 \lVert \eta \rVert_2} = \frac{\volav{\eta(z)} }{\sigma}.
\end{equation}
As $R$ increases the heat transport due to convection over conduction increases. In the asymptotic limit of $R=\infty$ where $U=U_0$, the expectation is that $Nu=\infty$, which can only be occur if $\sigma=0$. 
% For convenience we define 
% \begin{equation}
%     \label{eq:Nu_cond}
%     \sigma: =  \tfrac12\volav{\eta(z)} - \tfrac12 \lVert \eta \rVert_2 .
% \end{equation}
The implication of which is that $\mean{\delta T} \geq 0$. In uniform internal heating where $\eta(z)=z$ it follows that $\sigma = \frac12 - \frac{1}{\sqrt{3}}  < 0 $ and $\mean{\delta T} = \frac12 \left(\frac12 - \frac{1}{\sqrt{3}} \right)<0$.

Further to the condition of $\sigma = 0$ With a non-trivial selection of $\phi'(z)$ an expression on $U$ can be obtained in terms of $\eta(z)$ which yields $R$-dependent conditions after   $\mathcal{S}_{\boldsymbol{k}}\geq0$ is satisfied.
We next present a choice of background profile, building on \cite{Arslan2021a}, to obtain an $R$ dependent bound.


\section{Choice of background profile}
\label{sec:tau_field}

The $R$ scaling for any bound is given by constructing a $\phi'(z)$ with nonzero boundary layers. In analogy to the $H(z)=1$ case \citep{Arslan2021a}, we choose
\begin{equation}
    \label{eq:b_rel}
    b = \frac{ a +1}{ \lVert \eta \rVert_2 },
\end{equation}
and the background profile is taken to be,  
\begin{equation}
	 \phi'= (a+1)
        \begin{dcases}
            \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta}, &  0\leq z \leq \delta, \\
           1 + \frac{ \eta(z)}{ \lVert \eta \rVert_2 },  &  \delta \leq z \leq 1-\delta,\\
            \left(1+ \frac{\eta(1-\delta)}{ \lVert \eta \rVert_2 }\right)\frac{(1-z)}{\delta},& 1-\delta \leq z \leq 1.
        \end{dcases}
        \label{eq:phi_prime}
\end{equation}
The value in the bulk of $\phi'$ is necessitated by the sign-indefinite term of the condition $\mathcal{S}_{\boldsymbol{k}}\geq0$ in \eqref{eq:sk_non_uni}. The behaviour in the boundary layers is chosen such that the profile is continuous at $\delta$ and $1-\delta$ given that $\phi'(0)=\phi'(1)=0$. 

Due to the no-slip boundary condition \eqref{bc:u_non_u} and incompressibility, at both boundaries $\hat{w}_{\boldsymbol{k}}=  \hat{w}_{\boldsymbol{k}}' = 0$. Then by use of the fundamental theorem of calculus and the Cauchy-Schwarz inequality we have that
\begin{equation}
    \hat{w}_{\boldsymbol{k}} \leq \frac23 z^{\frac32} \lVert \hat{ w}''_{\boldsymbol{k}}\rVert_2 . 
    \label{eq:w_est}
\end{equation}
The $\hat{w}_{\boldsymbol{k}}\hat{T}_{\boldsymbol{k}}$ term in \eqref{eq:sk_non_uni} can be estimated after substitution for $\phi'(z)$ in \eqref{eq:phi_prime}, $b$ in \eqref{eq:b_rel}, $\hat{w}_{\boldsymbol{k}}$ in \eqref{eq:w_est} and after use of the Cauchy-Schwarz inequality to obtain
\begin{align}
    \int^{\delta}_0 &(a+1+ b \eta(z) - \phi'(z)) |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \nonumber\\ &\leq\int^{\delta}_0 \frac23 ( a+1)\left[1 + \frac{\eta(z)}{  \lVert \eta \rVert_2 } -  \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta} \right] z^{\frac32} \hat{\theta}_{\boldsymbol{k}} \textrm{d}z \lVert \hat{w}''_{\boldsymbol{k}}\rVert_2  \nonumber  \\
    &\leq \frac23(a+1)  \underbrace{\left(\int^{\delta}_0 \left[1 + \frac{\eta}{ \lVert \eta \rVert_2 } -  \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta} \right]^2 z^3 \textrm{d}z  \right)^{\frac12}}_{\Psi_0}  \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2 \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2.
    \label{eq:sign_indefinite_psi}
\end{align}
The same calculation in $[1-\delta,1]$ gives the same estimate with $\Psi_1$, where $\eta(\delta)$ is replaced by $\eta(1-\delta)$ and $z$ with $1-z$.
The integrals $\Psi_0$ and $\Psi_0$ once evaluated for a particular profile $H(z)$ gives a $\delta=\delta(R)$ to satisfy the condition $\mathcal{S}_{\boldsymbol{k}}\geq 0$. Substituting \eqref{eq:sign_indefinite_psi} into \eqref{eq:sk_non_uni} gives
\begin{equation}
    \label{eq:sk_nonu}
    \mathcal{S}_{\boldsymbol{k}} \geq \frac{a}{R k^2} \lVert \hat{w}''_{\boldsymbol{k}}\rVert_2^2 + b k^2 \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2^2 - \frac23 ( a+1)( \Psi_0 + \Psi_1 ) \lVert \hat{w}''_{\boldsymbol{k}}\rVert_2 \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2 .
\end{equation} 
The homogeneous quadratic form is non-negative given it has a nonpositive discriminant, which holds when
\begin{equation}
    \label{eq:psi_sc}
      \Psi_0 + \Psi_1 \leq  \sqrt{\frac{ 9 a }{R(a+1) \lVert \eta \rVert_2 } } ~ .
\end{equation}

% The condition \eqref{eq:psi_sc} may appear odd, due to the fact that the heating distribution $\eta(z)$ appears both on the left and right-hand side. However, as will be demonstrated for $H(z)$ in , and in fact for all $\eta(z) \in L^2(\Omega)$, then up to constants $\Psi_i \lesssim \delta^2$ for $i\in\{1,2\}$. This was the case for $H(z)=1$ as demonstrated in \cite{Arslan2021a}.


Finally, consider the upper bound $U$. Substituting  $b$ from \eqref{eq:b_rel} and $\phi'(z)$ from \eqref{eq:phi_prime} into $U$ given by \eqref{eq:U_bound} gives that
\begin{align}
    U =&~ \frac{\delta(a+1)}{12 \lVert \eta \rVert_2}   \left[ \left( \lVert \eta \rVert_2 + \eta(\delta)\right)^2 + \left( \lVert \eta \rVert_2 + \eta(1-\delta) \right)^2 \right] + \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z\, .
    \label{eq:U_form_sub}
\end{align}
In the expression \eqref{eq:U_form_sub}, the first term is positive and order $\delta$. For a bound of the form
$U \leq U_0(\eta) - c(\eta)R^{-\frac13}$, both the uniform upper bound ($U_0$) and negative $\delta$ contribution would have to come from the second term in \eqref{eq:U_form_sub}. 

\section{Non-uniform heating and cooling profiles}
\label{sec:non_uni_egs}

For the case of $\eta(1)=0$ we examine a test profiles and calculate $\sigma$ to see if the condition $\sigma = 0$ can be satisfied. The uniform upper bound for each heating profile can be found by calculating $U_0$ given by \eqref{eq:U0_uni_upper_non}. 
% Initially we propose a non-uniform heating profile with mean one internal heating i.e. $\eta(1)=1$. Following this we take a brief look at a profile with net zero heating and cooling i.e. $\eta(1)=0$. 

% \subsection{Mean one heating/cooling : \texorpdfstring{$\eta(1)=1$}{test 1}}
% \label{eq:mean_one_profile}
% \subsubsection{Polynomial heating}

% We start with the case of mean one heating within the domain.#
% As such the boundary condition at $z=1$ from \eqref{bc:non_uni} is unit outwards heat flux.
The family of heating profiles we consider are smooth profiles parameterised by $n\in \mathbb{R}_+ $ such that  
  \begin{equation}    
        \label{eq:heating_smooth}
        H(n,z) = (n+1)(1-z)^{n} \quad \forall n \geq 0.
\end{equation}
The corresponding $\eta(z)$ can be found using \eqref{eq:eta_general} which gives
\begin{equation}
    \label{eq:eta_1}
    \eta(n,z) = 1 - (1-z)^{n+1}.
\end{equation}
\begin{figure}
\hspace{-1cm}
    \centering
    \includegraphics[scale=0.8]{fig/non_uni1.eps}
    \begin{tikzpicture}[overlay]
        \node at (-11,6) {\textit{(a)}};
        \node at (-11,3) {\textit{(b)}};
    \end{tikzpicture}
    \caption[Plots of smooth mean one heating profiles]{\textit{(a)} Plots of the heating profiles $H(z)$ given by \eqref{eq:heating_smooth} and \textit{(b)} plots of the heating distributions $\eta(z)$ given in \eqref{eq:eta_1} for $n\in[1,100]$ ({\color{mygrey}\solidrule}) with $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar6}\solidrule}) and $n=2$ ({\color{colorbar15}\solidrule}) highlighted.}
    \label{Fig:smooth_non_uni}
\end{figure}
In \cref{Fig:smooth_non_uni}  we plot example profiles of $H(z)$ and $\eta(z)$, where the cases of $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar6}\solidrule}) and $n=2$ ({\color{colorbar15}\solidrule}), higher $n$ are plotted in grey up to $n=100$. As $n$ increases the heating profile is a polynomial of increasing order with the heating becoming more localised to the lower boundary. At $n=\infty$ the heating profile becomes a Dirac delta distribution at $z=0$. Whereas for $n=0$ the heating is profile is that of uniform internal heating. Evaluating first the integral and L2 norm of $\eta$ gives
\begin{equation}
    \tag{\theequation{\textit{a,b}}}
     \volav{\eta} = \frac{n+1}{n+2}\, , \qquad
    \lVert \eta \rVert_2 = \sqrt{\frac{2 (n + 1)^2}{(n + 2)(2n + 3)}}\, . \label{eq:eta_int_1}
\end{equation}
Then $\sigma$ in \eqref{eq:delt_T_uni} becomes
\begin{equation}
     \sigma =  \frac{n+1}{2(n+2)} -  \frac{\sqrt{2}}{2}  \frac{n + 1}{\sqrt{ (n + 2)(2n + 3)} } ,
     \label{eq:sig_1}
\end{equation}
% and for reference later
% \begin{subequations}
% \begin{align}
%     \volav{\eta} &= \frac{n+1}{n+2}\, , \label{eq:eta_int_1}\\
%     \lVert \eta \rVert_2 &= \sqrt{\frac{2n^2 + 4n + 2}{(n + 2)(2n + 3)}}\, . \label{eq:eta_2norm_1}
% \end{align}
% \end{subequations}
Therefore, only when $n=\infty$ and the heating profile is a Dirac delta is the condition $\sigma=0$ satisfied. Stated in other words for the mean conductive heat flux to always be positive the heating is taken to be a Dirac delta distribution. The energy injected into the system is given exactly by $\volav{\eta}$ and as $n$ goes from 0 to $\infty$, $\volav{\eta}$ goes from $\frac12$ to 1.

% We can also illustrate that the bound would be of the form $\mean{wT}\leq U_0 - cR^{-1/3}$ where the constant $c$ is independent of the 

Next we determine the necessary condition for $\mathcal{S}_{\boldsymbol{k}}\geq 0 $ by evaluating $\Psi_0$ and $\Psi_1$ in \eqref{eq:sign_indefinite_psi}.
Given \eqref{eq:eta_1} and \eqref{eq:eta_int_1} then $\eta(z) \leq 1$ $\forall n$, and $-(\eta(\delta)/\lVert \eta \rVert_2 ) \leq 0 $ such that 
\begin{eqnarray}
    \Psi_0 \leq  \left( \int^{\delta}_0 \left[1 + \frac{1}{\lVert \eta \rVert_2}  \right]^2 z^3 \textrm{d}z \right)^{1/2} = \frac{\delta^2}{2} \left(1 + \frac{1}{\lVert \eta \rVert_2 }\right) .
\end{eqnarray}
These estimates fix $\Psi_0=\Psi_1$ such that the condition for the positivity of $\mathcal{S}_{\boldsymbol{k}}$ becomes
\begin{equation}
    \label{eq:delta_cond}
    \delta  \leq \left( \frac{81 a \lVert \eta \rVert_2}{R( a+1) \left(1 + \lVert \eta \rVert_2  \right)^2 } \right)^{1/4} \, .
\end{equation}
Next we look at the upper bound $U$ as given by \eqref{eq:U_form_sub} on the mean convective heat transport. We first state that for all $\delta < 1$ we can make the estimate that
\begin{align}
    (1-\delta)^{n+2} &= 1 - (n+2)\delta + \sum^{n+2}_{2}  \begin{pmatrix} n+2 \\ 2 \end{pmatrix} (-\delta)^{k} 
    \geq 1 - (n+2)\delta.
    \label{eq:est_bound}
\end{align}
Then assuming that $\eta(\delta)= 1 - (1-\delta)^{n+1}\leq 1$, $\eta(1-\delta) = 1 - \delta^{n+1}\leq 1$ and $(1-\delta)^{2n+3} - \delta^{2n+3} \leq 1$ for all $n$, after substituting \eqref{eq:eta_1} into \eqref{eq:U_form_sub} and using \eqref{eq:est_bound} we obtain
\begin{align}
    U \leq&~ \frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2   + \frac{a+1}{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\lVert \eta \rVert_2 + 1 - (1-z)^{n+1} \right)^2 \textrm{d}z \nonumber \\ 
    = &\frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2  + \frac{a+1}{4\lVert \eta \rVert_2}\Big((1+ \lVert \eta \rVert_2)^2(1-2\delta)  + \frac{2(1+\lVert \eta \rVert_2) }{(n+2)} (\delta^{n+2} - (1-\delta)^{n+2})  \nonumber \\
    & \hspace{5cm} - \frac{\delta^{2n+3} - (1-\delta)^{2n+3}}{2n+3}  \Big) \nonumber
    \\
    \leq&~ \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2} + \frac{1}{2n+3} \right)  \nonumber
    \\ & \hspace{5cm} -\frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - 1 -\frac{3\delta^{n+1}}{n+2}  \right)\delta  .
\end{align}
Finally, estimating the higher order term as $\delta^{n+1}  \leq m (n+2)$,
gives that
\begin{align}
    U \leq& ~  \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right)  -   \frac{ \delta(a+1)(1+ \lVert \eta \rVert_2)(   2 \lVert \eta \rVert_2 - 1 -3m  )}{6\lVert \eta \rVert_2}  .
\end{align}
For a bound of the form $U\leq f_0(n) - f_1(n)R^{-\beta}$, we require $  2 \lVert \eta \rVert_2 - 1 -3m \geq0$. The easiest way to see the range of valid of $m$ is in considering the two limits. At $n=0$ we require $m\leq \frac{-3+2\sqrt{3}}{9}$, while for $n\rightarrow\infty$ the condition is that $m\leq \frac16$. Given that $\lVert \eta \rVert_2$ monotonically increases for all $n$ we can make the choice $m =  \frac{1}{21}$, such that the bound which follows holds provided $ \delta^{n+1} \leq      \tfrac{1}{21}(n+2) $.
Finally the bound can be written as 
\begin{align}
    U \leq&~  \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right) -  \delta \, \frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - \frac87 \right) .
\end{align}
We determined $\delta$ in \eqref{eq:delta_cond}. If we take $\delta$ as large as possible and substitute back into $U$, realising that since $a>0$ then $a+1\geq1$ such that
\begin{align}
    U \leq& \underbrace{ \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right)}_{U_0}  - \underbrace{
    \frac{  (1+ \lVert \eta \rVert_2)^{1/2}}{2 \, \lVert \eta \rVert_2^{3/4}} \left(   2 \lVert \eta \rVert_2 - \frac87 \right)}_{U_1}\frac{a^{1/4}}{R^{1/4}} .
    \label{eq:U_final_forms}
\end{align}
Minimising \eqref{eq:U_final_forms} with respect to $a$ by solving $\partial_a U =0$ gives
\begin{equation}
    a = \left(\frac{U_1}{4 U_0} \right)^{4/3}    R^{-1/3},
\end{equation}
such that
\begin{align}
\tag{\theequation{\textit{a,b}}}
    \mean{wT} \leq U_0 - \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{1/3} R^{-1/3} , \qquad \mean{\delta T} \geq \frac{n+1}{n+2} -  U_0 + \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{1/3} R^{-1/3}\, .
 \end{align}
% and
% \begin{align}
%     \mean{\delta T} \geq& ~\frac{n+1}{n+2} -  U_0 + \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{\frac13} R^{-\frac13}\, .
% \end{align}
The bound on $\mean{\delta T}$ can be rearranged and simplified with \eqref{eq:eta_int_1} to obtain
\begin{align}
    \label{eq:delt_T_main_result}
    \mean{\delta T} \geq& ~ \sigma  +  \frac{ 3 }{16\lVert \eta \rVert_2} \left(\frac{2(1+\lVert \eta\rVert_2)^2(2\lVert \eta \rVert_2 - \tfrac87)^4}{\frac{n+1}{n+2} + \lVert \eta \rVert_2  } \right)^{1/3}
   R^{-1/3}\, .
\end{align}
Observe that if $n=0$, we have the results of \cite{Arslan2021a}
\begin{equation}
\tag{\theequation{\textit{a,b,c}}}
    \mean{wT} \leq \frac{3+2\sqrt{3}}{12} - c R^{-1/3} , \quad  \mean{\delta T} \geq \frac{3-2\sqrt{3}}{12} +   cR^{-1/3}\, ,\quad      Nu \leq \left(\frac{3-2\sqrt{3}}{6} + c R^{-1/3}\right)^{-1}.
\end{equation}
where instead $c\approx 0.0015$.
As a note the prefactor in the bound is smaller than that demonstrated in \cite{Arslan2021a}. A difference between the two choices is that while in the previous case the $\delta$ range was chosen for simplicity, here the restriction on $m$, restricts the $\delta$ to have to be below $\frac{-6+4\sqrt{3}}{9}$ as the bound is to accomodate all profiles $H$ defined by \eqref{eq:heating_smooth}. Crucially note that for some $R>R_n$ inverse conduction occurs where $\mean{\delta T} < 0$.
However for $n\rightarrow \infty$,
\begin{equation}
    U \leq 1 - c R^{-1/3},  \quad   \mean{\delta T} \geq c R^{-1/3},  \quad   Nu \leq c^{-1} R^{1/3},
\end{equation}
where $c \approx 0.2423$.
The main result on the intermediate behaviour of $\mean{\delta T}$ as $n$ varies. We find from \eqref{eq:delt_T_main_result} that $\mean{\delta T} \geq -f(n) + g R^{-1/3}$ where $f(n)\sim \frac{1}{n}$ and $g \sim \mathcal{O}(10^{-1})$. As such for a given heating profile $H(z)$ parameterised by $n$ in \eqref{eq:heating_smooth}, the value of the $R$ above which $\mean{\delta T}\leq 0$, $R_c$, for sufficiently large $n$ scales as $R_c \sim n^3$. 
 

The linear and nonlinear stability limits of the flow for this class of non-uniform heating profile is given by \eqref{eq:stab_lim}, substituting \eqref{eq:eta_1} for $\eta$ and evaluating the integral gives
\begin{subequations}
\begin{align}
        R_L = \frac{720}{ 1 - 60\frac{n^2+5n+6}{(n+6)(n+5)(n+4)(n+3)(n+2)} },  \\ R_E = \frac{5760}{\frac{1}{\gamma}(1+\gamma)(2 + \gamma ) - 24 \frac{60\gamma + (n+7)(60 + (n+6)(\gamma-5 + 2n\gamma+5n)))}{(n+7)(n+6)(n+5)(n+4)(n+3)(n+2)}}.
\end{align}
\end{subequations}
It is easy to confirm then for $n=0$ then $R_L=1440$, while for $n\rightarrow\infty$ then $R_L\rightarrow720$. As is well established these values are in fact $R$ above which uniform internally heated and fixed flux Rayleigh--B\'enard convection are linearly unstable \cite{Goluskin2016book}. 

If one optimises for $\gamma$ we obtain an expression for the energy stability in terms of $n$, where for $n=0$ the optimal $\gamma^*=\sqrt{35} /3$ and $R_E = 2880(6\sqrt{35} - 35)\approx 1429.86$. In the case of Rayliegh--B\'enard convection $R_E=R_L$ is known a priori, this is not the case for non-uniform internally heated convection where there always exists a $R_E < R_L$ where a flow may be unstable to energy perturbations but remain linearly stable.


\begin{figure}
% \hspace{-1cm}
    \centering
    \includegraphics[scale=1]{fig/DT_1.eps}
        \begin{tikzpicture}[overlay]
        \node at (-6,7.7) {\textit{(a)}};
        \node at (-6,3.8) {\textit{(b)}};
        \node at (0.1,3.8)
        {\textit{(c)}} ;
    \end{tikzpicture}
    \caption[Lower bounds on dT]{ \textit{(a)} Plots of the lower bounds on $\mean{\delta T}$, with
    heating profiles $H(z)$ given by \eqref{eq:heating_smooth} for $n\in[0,100]$ ({\color{mygrey}\solidrule}) with $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar6}\solidrule}), $n=2$ ({\color{colorbar15}\solidrule}) and $n=\infty$ ({\solidrule}) highlighted. \textit{(b)} Plots of the critical $R_c$ at which the lower bound on $\mean{\delta T}$ becomes equal to zero for given $n$ and \textit{(c)} plots of $\sigma$ as given in \eqref{eq:sig_1} against $n$ for the heating profiles of \eqref{eq:heating_smooth}. }
    \label{fig:bound_dT_1}
\end{figure}


%%%%%%%%%%%% subsection removed doesnt add to discussion
% \subsubsection{Exponential heating }

% Another family of mean one heating profiles, as opposed to polynomial $H(z)$ are exponential $H(z)$ parameterised by $\ell \in \mathbb{R}_+$. 

% The heating profile choice is 
%   \begin{equation}    
%         \label{eq:heating_smooth_exp}
%         H(\ell,z) = \frac{\textrm{e}^{-\frac{z}{\ell}}}{\ell(1-\textrm{e}^{-\frac{1}{\ell}})}.
% \end{equation}
% The corresponding $\eta(z)$ can be found using \eqref{eq:eta_general}, from which we obtain
% \begin{equation}
%     \label{eq:eta_1_exp}
%     \eta(n,z) = \frac{1 - \textrm{e}^{-\frac{z}{\ell}}}{1-\textrm{e}^{-\frac{1}{\ell}}}.
% \end{equation}

% \begin{figure}
% \hspace{-1cm}
%     \centering
%     \includegraphics[scale=0.8]{fig/non_unie.eps}
%     \begin{tikzpicture}[overlay]
%         \node at (-11,6) {\textit{(a)}};
%         \node at (-11,3) {\textit{(b)}};
%     \end{tikzpicture}
%     \caption[Plots of smooth mean one heating profiles]{\textit{(a)} Plots of the heating profiles $H(z)$ given by \eqref{eq:heating_smooth_exp} and \textit{(b)} plots of the heating distributions $\eta(z)$ given in \eqref{eq:eta_1_exp} for $\ell$ ({\color{mygrey}\solidrule}) with $\ell=10^{-2}$ ({\color{colorbar1}\solidrule}), $\ell=10^{-1}$ ({\color{colorbar6}\solidrule}) and $\ell=1$ ({\color{colorbar15}\solidrule}) highlighted.}
%     \label{fig:smooth_non_uni_exp}
% \end{figure}

% In \cref{fig:smooth_non_uni}  we plot example profiles of $H(z)$ and $\eta(z)$, where the cases of $\ell=10^{-2}$ ({\color{colorbar1}\solidrule}), $\ell=10^{-1}$ ({\color{colorbar6}\solidrule}) and $\ell=1$ ({\color{colorbar15}\solidrule}), are highlighted. As $\ell$ decreases the heating profile is an of increasing order with the heating becoming further localised to the lower boundary. At $\ell=0$ the heating profile becomes a Dirac delta distribution at zero. Whereas for $\ell=\infty$ the heating is profile is that of uniform internal heating. Evaluating $\sigma$ as defined in \eqref{eq:Nu_cond} gives
% \begin{equation}
%      \sigma =  \frac{1-\ell(1-\textrm{e}^{-\frac{1}{\ell}})- \sqrt{1-2\ell(1-\textrm{e}^{-\frac{1}{\ell}}) + \tfrac12 \ell (1-\textrm{e}^{-\frac{2}{\ell}})} }{2(1-\textrm{e}^{-\frac{1}{\ell}})} 
%      \label{eq:sig_1_e}
% \end{equation}
% and for reference later
% \begin{subequations}
% \begin{align}
%     \volav{\eta} &= \frac{1-\ell(1-\textrm{e}^{-\frac{1}{\ell}})}{1-\textrm{e}^{-\frac{1}{\ell}}}\, , \label{eq:eta_int_1_e}\\
%     \lVert \eta \rVert_2 &= \frac{\sqrt{1-2\ell(1-\textrm{e}^{-\frac{1}{\ell}}) + \tfrac12 \ell (1-\textrm{e}^{-\frac{2}{\ell}})}}{1-\textrm{e}^{-\frac{1}{\ell}}} \, . \label{eq:eta_2norm_1_e}
% \end{align}
% \end{subequations}
% Therefore, only when $\ell=0$ and the heating profile is a Dirac delta is the condition $\sigma=0$ satisfied, as before.

% % We can also illustrate that the bound would be of the form $\mean{wT}\leq U_0 - cR^{-1/3}$ where the constant $c$ is independent of the $R$ and $Pr$. Estimating the integral since $\eta(z) \leq 1$ $\forall n$, and $-(\eta(\delta)/\lVert \eta \rVert_2 ) \leq 0 $ then
% % \begin{eqnarray}
% %     \Psi_0 \leq  \left( \int^{\delta}_0 \left[1 + \frac{1}{\lVert \eta \rVert_2}  \right]^2 z^3 \textrm{d}z \right)^{\frac12} = \frac{\delta^2}{2} \left(1 + \frac{1}{\lVert \eta \rVert_2 }\right) .
% % \end{eqnarray}
% % % For brevity we retain the integral of $\Psi$ as
% % % \begin{equation}
% % %     \Psi \leq \frac{\delta^4}{4} \left(1 + \frac{1}{\lVert \eta \rVert_2 }\right)^2 .
% % % \end{equation}
% % The condition for the positivity of $\mathcal{S}_{\boldsymbol{k}}$ becomes
% % \begin{equation}
% %     \label{eq:delta_cond}
% %     \delta  \leq \left( \frac{9 a \lVert \eta \rVert_2}{R( a+1) \left(1 + \lVert \eta \rVert_2  \right)^2 } \right)^{\frac14} \, .
% % \end{equation}
% % The bound on the mean convective heat transport can be simplified by given the fact that $\eta(\delta)= 1 - (1-\delta)^{n+1}\leq 1$ and $\eta(1-\delta) = 1 - \delta^{n+1}\leq 1$ this gives
% % \begin{align}
% %     U \leq&~ \frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2   + \frac{a+1}{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\lVert \eta \rVert_2 + 1 - (1-z)^{n+1} \right)^2 \textrm{d}z \nonumber \\ 
% %     % =& ~ \frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2   + \frac{a+1}{4 \lVert \eta \rVert_2 } \Big(  \left(1 + \lVert \eta \rVert_2 \right)^2 (1-2\delta) + \frac{2\left(1 + \lVert \eta \rVert_2 \right)}{n+2}   (\delta^{n+2} - (1-\delta)^{n+2}) \nonumber 
% %     % \\ &~ - \frac{1}{2n+3}   (\delta^{2n+3}-(1-\delta)^{2n+3})  \Big) \nonumber 
% %     % \\
% %     \leq& ~ \frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2   + \frac{a+1}{4 \lVert \eta \rVert_2 } \Big(  \left(1 + \lVert \eta \rVert_2 \right)^2 (1-2\delta) + \frac{2\left(1 + \lVert \eta \rVert_2 \right)}{n+2}  (\delta^{n+2} - (1-\delta)^{n+2}) \nonumber\\&~ + \frac{1}{2n+3}   \Big) .
% % \end{align}
% % The $(1-\delta)^{n+2}$ term due to its sign needs to be estimated, while retaining an order 1 contribution. We can Taylor expand the term about zero and estimate appropriately 
% % \begin{align}
% %     (1-\delta)^{n+2} &= 1 - (n+2)\delta + \frac12 (n+2)(n+1)\delta^2 - \frac16 (n+2)(n+1)n \delta^3 +  ..., \nonumber\\
% %     &= 1- (n+2)\delta  + \frac12(n+2)(n+1)\delta\left( \delta - \frac13 n \delta^2 + ... \right)\nonumber \\
% %     &\geq 1 - (n+2)\delta.
% % \end{align}
% % Use of the previous estimate gives 
% % \begin{align}
% %     U \leq& ~ ~ \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2}{n+2} (1+\lVert \eta \rVert_2) + \frac{1}{2n+3} \right) \nonumber
% %     \\ &-  \frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - 1   \right)\delta  + \frac{(a+1)(1+\lVert \eta \rVert_2)}{2(n+2)\lVert \eta \rVert_2} \delta^{n+2}.
% % \end{align}
% % % For the non-uniform heating profile of $\eta = 1 - (1-z)^{n+1}$,
% % % \begin{equation}
% % %     \lVert \eta \rVert_2 = \sqrt{\frac{2(n+1)^2}{(n+2)(2n+3)}}~~.
% % % \end{equation}
% % Finally, estimating the final term of order $\delta^{n+2}$ as  
% % \begin{equation}
% %     \frac{(a+1)(1+\lVert \eta \rVert_2)}{2(n+2)\lVert \eta \rVert_2} \delta^{n+2} \leq m \delta    \frac{(a+1)(1+\lVert \eta \rVert_2)}{\lVert \eta \rVert_2} ,
% % \end{equation}
% % which holds for $\delta \leq 4m$ and gives that
% % \begin{align}
% %     U \leq& ~  \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right)  -   \frac{ \delta(a+1)(1+ \lVert \eta \rVert_2)(   2 \lVert \eta \rVert_2 - 1 -6m  )}{6\lVert \eta \rVert_2}  .
% % \end{align}
% % Then clearly for a bound of the form $U\leq U_0(n) - f(n)R^{-\beta}$, we require $  2 \lVert \eta \rVert_2 - 1 -6m \geq0$. Considering the extremes, at $n=0$ this equates to $m\leq \frac{-3+2\sqrt{3}}{18}$, while for $n\rightarrow\infty$ the condition is that $m\leq \frac16$. We make the choice $m = \frac{1}{40}$, sch that the following results hold for $\delta\leq \frac{1}{10}$.

% % Finally the bound is 
% % \begin{align}
% %     U \leq&~  \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right) -  \delta \, \frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - \frac{23}{20}  \right) .
% % \end{align}
% % Taking $\delta$ from \eqref{eq:delta_cond} as an equality and substituting gives that
% % \begin{align}
% %     U \leq& ~\frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right) - 
% %     \frac{ \sqrt{3}\, a^{\frac14}  (1+ \lVert \eta \rVert_2)^{\frac12}}{6 R^{\frac14}\, \lVert \eta \rVert_2^{\frac34}} \left(   2 \lVert \eta \rVert_2 - \frac{23}{20}  \right) .
% % \end{align}
% % Minimising with respect to $a$ by solving $\partial_a U =0$, gives
% % \begin{equation}
% %     a = \underbrace{\left( \frac{ \sqrt{3} \lVert \eta \rVert_2^{\frac14}  \, (1+ \lVert \eta \rVert_2)^{\frac12} \left(   2 \lVert \eta \rVert_2 - \frac{23}{20}  \right)  }{ 6\left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2}{n+2} (1+\lVert \eta \rVert_2) + \frac{1}{2n+3} \right) } \right)^{\frac43}}_{a_0}
% %     R^{-\frac13},
% % \end{equation}
% % such that
% % \begin{align}
% %     U \leq& ~\frac{1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2} + \frac{1}{2n+3} \right) \nonumber \\ &- 
% %    \left[\frac{ \sqrt{3}\,  a_0^{\frac14}  (1+ \lVert \eta \rVert_2)^{\frac12}}{ \lVert \eta \rVert_2^{\frac34}} \left(   2 \lVert \eta \rVert_2 - \frac{23}{20}  \right) - \frac{   (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} }{4 a_0^{-1} \lVert \eta \rVert_2 } \right] R^{-\frac13}\, .
% %  \end{align}
% % and
% % \begin{align}
% %     \mean{\delta T} \geq& ~\frac{n+1}{n+2} -  \frac{1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2} + \frac{1}{2n+3} \right) \nonumber \\ &+ 
% %    \left[\frac{ \sqrt{3}\,  a_0^{\frac14}  (1+ \lVert \eta \rVert_2)^{\frac12}}{ \lVert \eta \rVert_2^{\frac34}} \left(   2 \lVert \eta \rVert_2 - \frac{23}{20}  \right) - \frac{   (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} }{4 a_0^{-1} \lVert \eta \rVert_2 } \right] R^{-\frac13}\, .
% % \end{align}
% % Given $\lVert \eta \rVert_2$ as given by \eqref{eq:eta_2norm_1}, this can be simplified and rewritten as 
% % \begin{align}
% %     \mean{\delta T} \geq& ~ \frac{n+1}{2(n+2)} - \frac{\lVert \eta \rVert_2}{2}  + 
% %    \left[\frac{ \sqrt{3}\,  a_0^{\frac14}  (1+ \lVert \eta \rVert_2)^{\frac12}}{ \lVert \eta \rVert_2^{\frac34}} \left(   2 \lVert \eta \rVert_2 - \frac{23}{20}  \right) - \frac{a_0}{2}\left(\frac{n+1}{n+2} + \lVert \eta \rVert_2 \right) \right] R^{-\frac13}\, .
% % \end{align}

% % We observe that if $n=0$,
% % \begin{equation}
% %     U \leq \frac{3+2\sqrt{3}}{12} - c R^{-1/3}
% % \end{equation}
% % where $c\approx 0.0003$ so that
% % \begin{equation}
% %     Nu \leq \left(\frac{3-2\sqrt{3}}{6} + c R^{-1/3}\right)^{-1},
% % \end{equation}
% % and 
% % \begin{align}
% %     \mean{\delta T} \geq& \frac{3-2\sqrt{3}}{12} +   cR^{-1/3}\, .
% % \end{align}
% % As a note the prefactor in the bound is smaller than that demonstrated in \cite{Arslan2021a} for the $n=0$ heating profile. This difference occurs due to the choice $\delta\leq \frac{1}{10}$, while in the uniform heating case the choice was $\delta\leq \frac13$. A difference between the two choices is that while in the previous case the $\delta$ range was chosen for simplicity, here the restriction on $m$, restricts the $\delta$ to have to be below $\frac{-6+4\sqrt{3}}{9}$.   
% % However for $n\rightarrow \infty$,
% % \begin{equation}
% %     U \leq 1 - c R^{-1/3}
% % \end{equation}
% % where $c \approx 0.183$ such that
% % \begin{equation}
% %     Nu \leq c^{-1} R^{1/3},
% % \end{equation}
% % and 
% % \begin{equation}
% %     \mean{\delta T} \geq c R^{-1/3}
% % \end{equation}
% % Of greater interest is the behaviour of $\mean{\delta T}$ with $n$. In fact, we find that $\mean{\delta T} \geq -p(n) + c(n) R^{-1/3}$ where $p(n)\sim \frac{1}{n}$ and $c(n) \sim constant$. As such for a given heating profile $H(z)$ parameterised by $n$, the value of the Rayleigh number above which $\mean{\delta T}\leq 0$, $R_n$, for sufficiently large $n$ scales as $R_n \sim n^3$. 
 

% % Finally the linear stability limit of the flow for this class of non-uniform heating profile is given by
% % \begin{equation}
% %     R_L = \frac{720(1-\textrm{e}^{-\frac{1}{\ell}})}{ 1 + 60\ell^3\textrm{e}^{-\frac{1}{\ell}}(1+6\ell+12\ell^2) - 60\ell^3(1-6\ell+12\ell^2) }.
% % \end{equation}
% % It is easy to confirm then for $n=0$, the linear stability limit is at $R_L=1440$, while for $n\rightarrow\infty$, $R_L\rightarrow720$, which is the linear stability limit for Rayleigh--B\'enard convection with fixed flux thermal boundary conditions.
% % While for the energy stability
% % \begin{equation}
% %     R_E = \frac{5760(1-\textrm{e}^{-\frac{1}{\ell}})}{ (1-\textrm{e}^{-\frac{1}{\ell}})(1 + \frac{2}{\gamma} )+\tfrac{31}{6}  + \tfrac{\gamma}{12}- 6\gamma\ell^3\textrm{e}^{-\frac{1}{\ell}}- 10\ell^3(1-\textrm{e}^{-\frac{1}{\ell}}) +60\ell^4(1+\textrm{e}^{-\frac{1}{\ell}}) + 2\gamma \ell^4(9+21\textrm{e}^{-\frac{1}{\ell}}) - 120\ell^5(1-(1+\gamma)\textrm{e}^{-\frac{1}{\ell}}) - 120\gamma \ell^6(1-\textrm{e}^{-\frac{1}{\ell}})}.
% % \end{equation}
% % Which can be optimised for $\gamma$ to obtain a relation for the energy stability limit in terms of $n$. 

% % % \begin{figure}
% % % % \hspace{-1cm}
% % %     \centering
% % %     \includegraphics[scale=1]{fig/DT_1.eps}
% % %         \begin{tikzpicture}[overlay]
% % %         \node at (-6,7.7) {\textit{(a)}};
% % %         \node at (-6,3.8) {\textit{(b)}};
% % %         \node at (0.1,3.8)
% % %         {\textit{(c)}} ;
% % %     \end{tikzpicture}
% % %     \caption[Lower bounds on dT]{ \textit{(a)} Plots of the lower bounds on $\mean{\delta T}$, with
% % %     heating profiles $H(z)$ given by \eqref{eq:heating_smooth} for $n\in[0,100]$ ({\color{mygrey}\solidrule}) with $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar6}\solidrule}), $n=2$ ({\color{colorbar15}\solidrule}) and $n=\infty$ ({\solidrule}) highlighted. \textit{(b)} Plots of the critical $R_c$ at which the lower bound on $\mean{\delta T}$ becomes equal to zero for given $n$ and \textit{(c)} plots of $\sigma$ as given in \eqref{eq:sig_1} against $n$ for the heating profiles of \eqref{eq:heating_smooth}. }
% % %     \label{fig:bound_dT_1}
% % % \end{figure}






\subsection{Mean zero heating/cooling: \texorpdfstring{$\eta(1)=0$}{test 1} }
\label{eq:mean_zero_profile}
\subsubsection{Polynomial heating and cooling }
\begin{figure}
    \centering
    \includegraphics[scale=0.8]{fig/non_uni3.eps}
     \begin{tikzpicture}[overlay]
        \node at (-11,6) {\textit{(a)}};
        \node at (-11,3) {\textit{(b)}};
    \end{tikzpicture}
    \caption[Plots of smooth net zero heating and cooling profiles]{\textit{(a)} Plots of smooth heating and cooling profiles $H(z) $ given by  \eqref{eq:H_hc} and \textit{(b)} plots of the heating distribution $\eta(z)$ given by \eqref{eq:eta_3} for odd $n\in[1 , 101]$ ({\color{mygrey}\solidrule}) with $n=1$ ({\color{colorbar1}\solidrule}), $n=3$ ({\color{colorbar6}\solidrule}) and $n=5$ ({\color{colorbar15}\solidrule}) highlighted.} 
    \label{fig:piecewise_non_uni3}
\end{figure}

The final non-uniform heating profile considering is one where there is net zero heating/cooling in the domain due to the choice $\eta(1)=0$. For $n \in 2\mathbb{N}-1$ we consider the following profile
\begin{equation}
    \label{eq:H_hc}
    H(n,z) = (1-2z)^n.
\end{equation}
The corresponding $\eta(z)$ to \eqref{eq:H_hc} is given by
\begin{equation}
    \label{eq:eta_3}
      \eta(n,z) = \frac{1 - (1-2z)^{n+1}}{2(n+1)},
\end{equation}
from which evaluating $\sigma$ in \eqref{eq:Nu_cond} gives
\begin{equation}
    \label{eq:sig_3}
    \sigma = \frac{1}{4(n+2)} - \frac{1}{2\sqrt{2(n+2)(2n+3)}}.
\end{equation}

As would be expected from physical arguments in this case the limiting behaviour of $\sigma$ and $\volav{\eta}$ can be said to be the opposite to that of \eqref{eq:heating_smooth}. Taking $n = \infty$ in \eqref{eq:sig_3} gives  $\sigma = 0$ however then $\volav{\eta} \rightarrow 0 $. In this scenario the upper bound on $\mean{wT}$ is somewhat more difficult to interpret. Since for $n$ increasing, $U_0$ as given in \eqref{eq:U0_uni_upper_non} goes to zero. For a fluid that is contained in an insulating box with no net heating or cooling, the mean vertical convective heat transport may not be the best diagnostic quantity to further understand the turbulence.  

Investigating further we start with the two integrals of $\eta$
\begin{subequations}
\begin{align}
    \volav{\eta} =& \frac{1}{2(n+2)} \\
    \lVert \eta \rVert_2 =& \sqrt{\frac{1}{2(n+2)(2n+3)}}.
    \end{align}
\end{subequations}
First we determine $\delta$ from evaluating $\Psi$, which by use of the fact that $\eta(z)\leq 1$ for all $z\in[0,1]$, then 
\begin{equation}
    \Psi \leq \left(\int^{\delta}_{0} \left[ 1 + \frac{1}{\lVert \eta \rVert_2} \right]^2 z^{3} \textrm{d}z\right)^{\frac12} = \frac{\delta^2}{2 \lVert \eta \rVert_2} (1+ \lVert \eta \rVert_2)
    \label{eq:delta_mean_zero}
\end{equation}
so that then
\begin{equation}
    \delta \leq  \left(\frac{9 a \lVert \eta \rVert_2}{R (a + 1)(1+ \lVert \eta \rVert_2)^2} \right)^{\frac14}.
    \label{eq:delta_condition}
\end{equation}
Turning to the bound on the convective heat transport, with $\eta$ given by \eqref{eq:eta_3} and since for odd $n$, $(-1)^{n+1} = 1$, while  $(-1)^{n+2}=-1$ and $(-1)^{2n+3}=-1$, evaluating the integral and estimating from above we have that
\begin{align}
    U &= \frac{\delta(a+1)}{24 \lVert \eta \rVert_2(n+1)^2} \left(1 + 2\lVert \eta \rVert_2(n+1) - (1-2\delta)^{n+1} \right)^2  \nonumber \\ 
    &\qquad + \frac{a + 1}{16   \lVert \eta \rVert_2 (n+1)^2 } \int^{1-\delta}_{\delta} \left( 1+ 2\lVert \eta \rVert_2(n+1) - (1-2z)^{n+1} \right)^2 \textrm{d}z \nonumber \\
    &\leq \frac{\delta(a+1)}{24 \lVert \eta \rVert_2(n+1)^2} \left(1 + 2\lVert \eta \rVert_2(n+1) \right)^2  + \frac{a + 1}{16 \lVert \eta \rVert_2(n+1)^2} \Bigg( \left(1 + 2\lVert \eta \rVert_2 (n+1)\right)^2(1-2\delta)  \nonumber \\ 
    & \qquad -    (1+  2\lVert \eta \rVert_2(n+1))\frac{2(1-2\delta)^{n+2}}{n+2} +  \frac{(1-2\delta)^{2n+3}}{2n+3} \Bigg).
\end{align}
Using that $1-2\delta\leq 1$ gives
% \begin{align}
%     U &\leq \frac{\delta (a + 1) }{6 \lVert \eta \rVert_2}  \left(1 + \lVert \eta \rVert_2 \right)^2 + \frac{a + 1}{16 \lVert \eta \rVert_2 (n+1)^2} \Bigg(\left(1 + 2\lVert \eta \rVert_2 (n+1)\right)^2(1-2\delta) \nonumber \\ & \hspace{4cm} -   (1+  2\lVert \eta \rVert_2(n+1))\frac{2(1-2\delta)^{n+2}}{n+2} +  \frac{1}{2n+3} \Bigg).
% \end{align}
% We can Taylor expand one of the terms in the parenthesis and estimate appropriately as
% \begin{align}
%     (1-2\delta)^{n+2} &= \sum^{n+2}_{k=0}  \begin{pmatrix} n+2 \\ k \end{pmatrix} (-2\delta)^{k} \geq 1 - \ell (n+2)  \delta ,
%     \label{eq:lower_2}
% \end{align}
% where $\ell$ is non-negative and for the lower bounds to hold it is required that $\ell\geq 2-\delta(n+1)$ which for $\delta \leq \frac14$ implies that we require $\ell \geq \frac14(7-n)$. Then substituting the lower bound in \eqref{eq:lower_2} into $U$ which gives
\begin{align}
    U &\leq  \frac{ a + 1}{16 (n+1)^2 \lVert \eta \rVert_2} \Big(\left(1 + 2(n+1)\lVert \eta \rVert_2 \right)^2 +  \frac{1}{2n+3} \Big) - \delta \, \frac{ (a + 1)  \left(1 + 2(n+1)\lVert \eta \rVert_2 \right)^2}{ 12 (n+1)^2 \lVert \eta \rVert_2} .
\end{align}
As in \cref{eq:mean_one_profile} the upper bound on $U$ looks similar for the polynomial profiles of $H$ considered, in addition to $\delta$ being given by the same equation as demonstrated by \eqref{eq:delta_mean_zero}, such that after substitution we obtain that
\begin{align}
    U &\leq \underbrace{\frac{ 1}{16 (n+1)^2 \lVert \eta \rVert_2} \Bigg(\left(1 + 2(n+1)\lVert \eta \rVert_2 \right)^2 +  \frac{1}{2n+3} \Bigg)}_{U_0}  (a+1) \nonumber \\ 
    & \qquad\qquad - \underbrace{\frac{\sqrt{3}}{12} \frac{(1+2(n+1)\lVert \eta \rVert_2)^{2}}{(n+1)^2\lVert \eta \rVert_2^{\frac34}}(1+\lVert \eta \rVert_2)^{\frac12} }_{U_1} \frac{a^{\frac14}}{R^{\frac14}}. 
\end{align}
% then with the choice $\ell=\frac23$, which holds for $n\geq \frac53$. This excludes $n=1$ from our upper bound of 
% \begin{equation}
%    U \leq \frac{a + 1}{4 \lVert \eta \rVert_2} \left(\left(1 + \lVert \eta \rVert_2 \right)^2 -   \frac{2(1+  \lVert \eta \rVert_2)}{n+2} +  \frac{1}{2n+3} \right) - \frac13 \delta (a + 1) \left(1 + \lVert \eta \rVert_2 \right).
% \end{equation}
\begin{figure}
% \hspace{-1cm}
    \centering
    \includegraphics[scale=1]{fig/DT_2.eps}
        \begin{tikzpicture}[overlay]
        \node at (-6,7.7) {\textit{(a)}};
        \node at (-6,3.8) {\textit{(b)}};
        \node at (0.1,3.8)
        {\textit{(c)}} ;
    \end{tikzpicture}
    \caption[Lower bounds on dT]{ \textit{(a)} Plots of the lower bounds on $\mean{\delta T}$, with
    heating profiles $H(z)$ given by \eqref{eq:H_hc} for odd $n\in[0,51]$ ({\color{mygrey}\solidrule}) with $n=1$ ({\color{colorbar1}\solidrule}), $n=3$ ({\color{colorbar6}\solidrule}) and $n=5$ ({\color{colorbar15}\solidrule})highlighted. \textit{(b)} Plots of the critical $R_c$ at which the lower bound on $\mean{\delta T}$ becomes equal to zero for given $n$ and \textit{(c)} plots of $\sigma$ as given in \eqref{eq:sig_3} against $n$ for the heating profiles of \eqref{eq:H_hc}. }
    \label{fig:bound_dT_2}
\end{figure}
% For this bound on $\mean{wT}$ to approach a constant from below, it is necessary that $2 + 2\lVert \eta \rVert_2 - 3 \ell > 0$. 
It then remains to minimise for $a$ by solving $\partial_a U =0$ to obtain that
\begin{equation}
    a = \left( \frac{U_1}{4 U_0} \right)^{\frac43} R^{-1/3}.
\end{equation}
Substituting into $U$ gives
\begin{align}
   U \leq  U_0 - \frac34 \left( \frac{U_1^4}{4 U_0} \right)^{\frac13} R^{-1/3} . 
\end{align}
Using \eqref{eq:energy_bal_nu} and after some simplification we have the lower bound
\begin{align}
    \mean{\delta T} \geq& ~ \frac{n}{4(n+1)(n+2)} - \frac{\sqrt{2}((n+2)^2 + (n+1)^2)}{8(n+1)^2\sqrt{(n+2)(2n+3)}} + \frac34 \left( \frac{U_1^4}{4 U_0} \right)^{\frac13}   R^{-1/3} . 
\end{align}


The linear stability limit can be calculated and is given by
\begin{equation}
    R_L = \frac{1440(n+1)}{1 - 15\, \frac{n^3 + 13n^2 + 56n + 81}{(n+2)(n+3)(n+4)(n+6)}}.
    \label{eq:Lin_stab_2}
\end{equation}
The implication of \eqref{eq:Lin_stab_2} is that for $n=\infty$, the system is stable to linear perturbations. However the linear and energy stability limits of internally heated convection are not equal such that subcritical convection is possible. 





\subsubsection{Exponential heating and cooling}

Considering the non-uniform heating and cooling profiles of \cite{bouillaut2022} yields the same results. In the work of \cite{bouillaut2022} the profiles considered are 
\begin{equation}
    H(z,\ell) = \frac{\textrm{e}^{-\frac{z}{\ell}}}{\ell} + \textrm{e}^{-\frac{1}{\ell}} - 1.
    \label{eq:h_exp}
\end{equation}
The corresponding $\eta$ is
\begin{equation}
    \eta(z,\ell) = z( \textrm{e}^{-\frac{1}{\ell}} - 1 ) - \textrm{e}^{-\frac{z}{\ell}} + 1.
    \label{eq:eta_exp}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[scale=0.9]{fig/non_uni_e.eps}
     \begin{tikzpicture}[overlay]
        \node at (-12,6.8) {\textit{(a)}};
        \node at (-12,3.2) {\textit{(b)}};
    \end{tikzpicture}
    \caption[Plots of smooth net zero heating and cooling profiles 2]{\textit{(a)} Plots of smooth heating and cooling profiles $H(z) $ given by  \eqref{eq:h_exp} and \textit{(b)} plots of the heating distribution $\eta(z)$ given by \eqref{eq:eta_exp} for $\ell\in[10^{-3} , 10]$ ({\color{mygrey}\solidrule}) with $\ell=0.01$ ({\color{colorbar1}\solidrule}), $\ell=0.1$ ({\color{colorbar6}\solidrule}) and $\ell=1$ ({\color{colorbar15}\solidrule}) highlighted.} 
    \label{fig:piecewise_non_unie}
\end{figure}

The integrals for this heating profile are
\begin{subequations}
\begin{align}
    \int^{1}_0 \eta~ \textrm{d}z &= \tfrac12 ( \textrm{e}^{-\frac{1}{\ell}} + 1 ) + \ell ( \textrm{e}^{-\frac{1}{\ell}} - 1 ), \\
    \lVert \eta \rVert_2^2 & = (\tfrac13 + 2\ell^2)(\textrm{e}^{-\frac{1}{\ell}} - 1)^2 + \textrm{e}^{-\frac{1}{\ell}} + \tfrac32 \ell (\textrm{e}^{-\frac{2}{\ell}} - 1)  . 
\end{align}
\end{subequations}
Then the $\sigma$ representing the uniform upper lower bound is given as 
\begin{equation}
    \label{eq:sig_exp}
    \sigma = \frac14 ( \textrm{e}^{-\frac{1}{\ell}} + 1 ) + \frac12 \ell ( \textrm{e}^{-\frac{1}{\ell}} - 1 ) - \frac12 \left( (\tfrac13 + 2\ell^2)(\textrm{e}^{-\frac{1}{\ell}} - 1)^2 + \textrm{e}^{-\frac{1}{\ell}} + \frac32 \ell \textrm{e}^{-\frac{2}{\ell}} - \frac32 \ell \right)^{\frac12} .
\end{equation}
Following the same method as outlined above, and specifically by evaluating  \eqref{eq:U_form_sub} the upper bound $U$ given that $\eta(\delta) \leq 1$ and $\eta(1-\delta) \leq 1$ on the first instance becomes
\begin{eqnarray}
    U &\leq& \frac{\delta(a+1)(1+ \lVert \eta \rVert_2 )^2}{6 \lVert \eta \rVert_2}  + \frac{a+1}{4 \lVert \eta \rVert_2} \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z)  \right)^2 \textrm{d}z \nonumber \\
    &=& \frac{\delta (a+1)(1+ \lVert \eta \rVert_2 )^2}{6 \lVert \eta \rVert_2} + \frac{a+1}{4 \lVert \eta \rVert_2} \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + 1 + z(\textrm{e}^{-\frac{1}{\ell}}-1) - \textrm{e}^{-\frac{z}{\ell}}  \right)^2 \textrm{d}z \nonumber \\
    &=& \frac{\delta (a+1)(1+ \lVert \eta \rVert_2 )^2}{6 \lVert \eta \rVert_2}  + \frac{a+1}{4 \lVert \eta \rVert_2} \Bigg( (1+\lVert \eta \rVert_2)^2(1-2\delta) + (1+ \lVert\eta \rVert_2)(\textrm{e}^{-\frac{1}{\ell}}-1)(1-2\delta)  \nonumber \\
    && + \frac13(\textrm{e}^{-\frac{1}{\ell}} -1)^2( (1-\delta)^3 - \delta^3) - 2\ell (1+ \lVert \eta \rVert_2 )(\textrm{e}^{-\frac{\delta}{\ell}} - \textrm{e}^{- \frac{1-\delta}{\ell}}  ) \nonumber \\
    && + \ell (\textrm{e}^{- \frac{2\delta}{\ell}} - \textrm{e}^{-2 \frac{1-\delta}{\ell}}) - 2\ell (\textrm{e}^{-\frac{1}{\ell}}-1)( 2\textrm{e}^{-\frac{\delta}{\ell}} - (2-\delta)\textrm{e}^{-\frac{1-\delta}{\ell}} ) \Bigg) .
\end{eqnarray}
We make the following estimates
\begin{equation}
    -\textrm{e}^{-\frac{1-\delta}{\ell}} \leq -\textrm{e}^{-1/\ell}, \qquad \textrm{e}^{-\delta/\ell} \leq 1, \qquad \textrm{e}^{- \frac{1-\delta}{\ell}} \leq \textrm{e}^{-\delta/\ell}.
\end{equation}
and 
\begin{equation}
    (1-\delta)^3-\delta^3 \leq 1- 2\delta\, , 
\end{equation}
such that
\begin{align}
    U \leq &~~ \frac{(a+1)}{4 \lVert \eta \rVert_2} \underbrace{\left( (1+\lVert \eta \rVert_2)^2 + (1+ \lVert \eta \rVert_2)(\textrm{e}^{-\frac{1}{\ell}}-1) + \tfrac13(\textrm{e}^{-\frac{1}{\ell}}-1)^2 + \ell(1 -\textrm{e}^{-\frac{2}{\ell}})  \right)}_{U_1} \nonumber \\ 
    &- \frac{\delta (a+1)}{6\lVert \eta \rVert_2} \underbrace{\left( 2(1+\lVert \eta \rVert_2)^2 + 3(1+\lVert \eta \rVert_2)(\textrm{e}^{-\frac{1}{\ell}} - 1) +(\textrm{e}^{-\frac{1}{\ell}}-1)(\textrm{e}^{-\frac{1}{\ell}}(1+3\ell)-1)  \right)}_{U_2} \, . \label{eq:U_bound_3}
\end{align}
The spectral constraint of $\mathcal{S}_{\boldsymbol{k}} \geq 0$ gives the condition \eqref{eq:delta_cond} for $\delta$. Taking \eqref{eq:delta_cond} as an equality for $\delta$ substituting into \eqref{eq:U_bound_3}, estimating from above given that $a\geq 0$ such that $(a+1)^{\frac34}\geq 1$, then optimising for $a$ we find
\begin{equation}
    a = \underbrace{\left[ \frac{\sqrt{3} \lVert \eta \rVert_2^{\frac14} U_2 }{6(1+\lVert \eta \rVert_2)^{\frac12} U_1 } \right]^{\frac43}}_{a_0} R^{-\frac13},
\end{equation}
such that then 
\begin{align}
    U \leq ~~ \frac{U_1 }{4 \lVert \eta \rVert_2} -  \left[\frac{\sqrt{3} a_0^{\frac14} U_2}{6\lVert \eta \rVert_2^{\frac34}(1+\lVert \eta \rVert_2)^{\frac12}} - \frac{a_0 U_1}{4 \lVert \eta \rVert_2} \right] R^{-\frac13} \, . \label{eq:U_bound_3a}
\end{align}
The lower bound on the mean conductive heat transport is
\begin{equation}
    \mean{\delta T} \geq \volav{\eta} - \frac{U_1 }{4 \lVert \eta \rVert_2} + \left[\frac{\sqrt{3} a_0^{\frac14} U_2}{6\lVert \eta \rVert_2^{\frac34}(1+\lVert \eta \rVert_2)^{\frac12}} - \frac{a_0 U_1}{4 \lVert \eta \rVert_2} \right] R^{-\frac13} .
\end{equation}
\begin{figure}
% \hspace{-1cm}
    \centering
    \includegraphics[scale=1]{fig/DT_3.eps}
        \begin{tikzpicture}[overlay]
        \node at (-6,7.7) {\textit{(a)}};
        \node at (-6,3.8) {\textit{(b)}};
        \node at (0.1,3.8)
        {\textit{(c)}} ;
    \end{tikzpicture}
    \caption[Lower bounds on dT]{ \textit{(a)} Plots of the lower bounds on $\mean{\delta T}$, with
    heating profiles $H(z)$ given by \eqref{eq:h_exp} for $\ell\in[10^{-2},10^2]$ ({\color{mygrey}\solidrule}) with $\ell=10^{-2}$ ({\color{colorbar1}\solidrule}) and $\ell=10^{-1}$ ({\color{colorbar6}\solidrule}) highlighted. \textit{(b)} Plots of the critical $R_c$ at which the lower bound on $\mean{\delta T}$ becomes equal to zero for given $\ell$ and \textit{(c)} plots of $\sigma$ as given in \eqref{eq:sig_exp} against $\ell$ for the heating profiles of \eqref{eq:h_exp}. }
    \label{fig:bound_dT_3}
\end{figure}

Finally the linear stability limit can be calculated by substituting \eqref{eq:eta_exp} into \eqref{eq:stab_lim} we find that
\begin{equation}
    R_L = \frac{1440}{(\textrm{e}^{-\frac{1}{\ell}} + 1)(1 + 720 \ell^4) + 120\ell^3(\textrm{e}^{-\frac{1}{\ell}} - 1)(1+12\ell^2)},
\end{equation}
where in the limit of $\ell \rightarrow 0$ we find that $R_L \rightarrow 1440$ while in the limit $\ell \rightarrow \infty$ it transpires that $R_L \rightarrow 0$.  

\section{Discussion}





==> v2.tex <==
\section{Introduction}
\label{sec:intro}

Across a wide range of scales, fluids transport heat by both conduction and convection. Thermal convection in particular occurs when temperature gradients are of sufficient size to induce instability in an otherwise motionless fluid. As the size of the gradients increase, eventually, the convection becomes turbulent. Turbulent convection can on the one hand be driven purely by boundary heating, as in Rayleigh--B\'enard convection, or by internal heating. 
From the interior of planets and the Earth's Mantle \citep{MantleConvectioninTerrestrialPlanets} to planetary atmospheres \citep{tritton1975internally} the resultant dynamics are driven by internal sources or sinks of heat.  

The large scale dynamics of internally heated convection (IHC) can be understood through a select number of quantities. These are the mean temperature $\mean{T}$, the vertical heat transport by conduction $\dT$, and the mean vertical convective heat flux $\wT$. Here and throughout the paper, angled brackets denote a volume average, the subscript $h$ indicates averaging only over the horizontal directions, and overbars indicate averaging over infinite time. Of particular interest is the variation of these mean quantities as the rate of heating, quantified by the Rayleigh number $R$, increases. $R$ is the nondimensional ratio of the destabilising effects of heating to the stabilising effect of diffusion. In simulations and experiments, studies are limited by the range of Rayleigh numbers that can be spanned. Instead, one can seek scaling laws valid for all $R$, by solving suitably constructed optimisation problems for the relevant quantity. While scaling laws can be sought with a number of different approaches, of particular interest are rigorous bounds, which do not rely on any unproven assumptions.  

Rigorous scaling laws for $\wT$ and $\mean{T}$ in IHC with spatially uniform heating have been derived  under a range of boundary conditions  using the \emph{background method} \citep{Lu2004,Whitehead2011,Whitehead2012,Goluskin2012,Arslan2021a, Arslan2021,Arslan2023,kumar2021ihc}. The method, popularized by \cite{Doering1994,Doering1996} and \cite{Constantin1995a}, produces upper bounds on mean quantities that are quadratic in the flow variables through the solution of a convex optimization problem.
In comparison to previous applications of the background field method for IHC 
in this paper we prove scaling laws for $\wT$ when the internal heating is taken to be non-uniform and fixed flux boundary conditions hold. However, the resultant bounds demonstrated in \cite{Arslan2021a} on $\dT$ could not rule out inverse conduction, ie $\dT < 0$, for $R>78400$. This paper aims to investigate if such unphysical behaviour can be ruled out by use of non-uniform heating profiles by proving $R$-dependent bounds on the quantities of interest. As will be demonstrated the $R$ value above which inverse conduction occurs can be increased by localising the heat to the lower boundary.    


Non-uniform IHC has also been studied in alternative geometries and with insulating boundaries \citep{Miquel2019,Tobasco2022,Song2022}. 
In these contexts rigorous bounds have been demonstrated for $\mean{T}$ and the Nusselt number $Nu$, quantifying the total over the mean conductive heat transport vertically. This paper focuses on a fluid confined to a planar geometry where the non-uniform heating has mean one and is only a function of $z$.    

 




\section{Setup}
\label{sec:setup}

We consider a layer of fluid heated internally with kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Bounded between two horizontal plates separated by a distance $d$, the layer is periodic in the horizontal ($x$ and $y$) directions with periods $L_x$ and $L_y$.
The dimensional heating is $\Tilde{H}=H_0 H(z)$ where $H_0$ is the volumetric heating rate while $H(z)$ is an arbitrary function.

To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2H_0/\kappa \rho c_p$ as the temperature scale \citep{roberts1967convection}. The motion of the fluid in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ is then governed by the Boussinesq equations
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
Notice that if we wanted to increase the generality of the argument we could consider non-uniform heating which varies in all three spatial directions $H(\boldsymbol{x})$. The usual non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa}
    \qquad\text{and}\qquad 
    R = \frac{g \alpha H_0 d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are taken to be no-slip for the velocity vector $\boldsymbol{u}$, and fixed flux for the temperature:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:T_f}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-\eta(1),
\end{gather}
\end{subequations} 
where we introduce the total potential energy of the system as,
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z) \textrm{d}z.
\end{equation}
A statistically stationary state can be achieved when $\eta(1)=1$, corresponding to mean one heating/cooling in the domain \citep{Goluskin2016book,Arslan2021a}. Alternatively, one could take $\eta(1)=0$ (mean zero heating/cooling).


We can evaluate the energy balance of the system by taking $\mean{z\cdot \eqref{eq:nondim_energy_nonUniform}}$, and using \eqref{eq:eta_general},  \eqref{bc:T_f} and integrating by parts to obtain
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}} &= \volav{\eta(z)}.
\end{align}
The left hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical heat flux due to convection, $\wT$, and the mean heat flux due to conduction, $\dT = \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}}$.
Like by taking $\mean{z^2\cdot \eqref{eq:nondim_energy_nonUniform}}$
A uniform in $R$ and $Pr$ bound on $\mean{T}$ can be demonstrated. Once more integrating by parts with the boundary conditions and given that $\mean{zwT}\geq0 $ we have that 
\begin{equation}
    \label{eq:T_uniform}
    \mean{T} \leq \volav{z \eta(z)}.
\end{equation}
If the internal heating were to be uniform, then $\eta=z$ and the problem reduces to that presented in \cite{Arslan2021a} where $\wT + \dT = \frac12$ and $\mean{T} \leq \frac13$. 

The Nusselt number defined in terms of $\eta(z)$, for non-uniform heating becomes
\begin{equation}
    \label{eq:Nu_non_u}
    Nu = \frac{\dT  + \wT}{ \dT } = \frac{\volav{\eta(z)}}{\volav{ \eta(z)} \, - \mean{wT}} \, .
\end{equation}



The value of $R$ at which the flow becomes linearly and nonlinearly unstable can be determined analytically for this flow.
The expressions follow from the discussion in \cite{Goluskin2015a} and are
\begin{equation}
\tag{\theequation\textit{a,b}}
     R_L = \frac{1}{\int^{1}_0 \eta(z) P(z) \textrm{d}z }, \qquad
    R_E = \frac{2}{\int^{1}_0 (\frac{1}{\gamma} + \eta(z)) Q(z) \textrm{d}z}, \label{eq:stab_lim}
\end{equation}
where $P(z)$ and $Q(z)$ are polynomials dependent on the vertical velocity boundary conditions 
\citep[][\emph{Appendix A}]{Goluskin2015a} and $\gamma$ is a balance parameter, equivalent to $b$ in \eqref{eq:V_func}. 


Finally, to remove the inhomogeneous boundary conditions on $T$ it is convenient to rewrite the temperature field in terms of perturbations from the conductive profile,
\begin{equation}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition it follows that $T'_c = - \eta(z)$. Then, writing \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ gives
\begin{subequations}
\begin{align}
     \partial_t \theta + \boldsymbol{u} \cdot \nabla \theta = \Delta \theta + w\, \eta(z) , \\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{align}
\end{subequations}


\section{Bounds on heat transport}
\label{sec:nonuni_bounds}

The main aim of this work is to demonstrate $R$ dependent bounds on the heat transport for non-uniform heating profiles. This is achieved by an application of auxiliary functional method \citep{Chernyshenko2014a,Chernyshenko2022,Fantuzzi2022} to prove an upper bounds on $\wT$ and by extension a lower bound on $\dT$ given \eqref{eq:energy_bal_nu}. When using quadratic auxiliary functions this approach is equivalent to the background field method. The quadratic auxiliary functional used is 
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},T\} = \volav{ \frac{a}{2 Pr \,R}|\boldsymbol{u}|^2 + \frac{b}{2} |\theta|^2 - \phi \theta },
    \label{eq:V_func}
\end{equation}
where $a$ and $b$ are non-negative numbers referred to as balance parameters, while $\phi(z)$ is the background temperature field satisfying the same boundary conditions as $\theta$. Following exactly the approach outlined in \cite{Arslan2021a} a minimization problem can be constructed for the upper bound $U$ on $\wT=\mean{w\theta}$. For brevity we omit the derivation here as the steps are identical.
Then we can bound the mean convective heat transport $\mean{w\theta}\leq U$, where
\begin{equation}
    \label{eq:U_bound}
    U = \volav{ \frac{\phi'(z)^2}{4b} },
\end{equation}
while requiring that for all $\boldsymbol{k} \neq 0$, 
\begin{equation}
    \label{eq:sk_non_uni}
     \mathcal{S}_{\boldsymbol{k}} := \volav{  \frac{a|w''_{\boldsymbol{k}}(z)|^2}{R\,k^2}  + b |\theta'_{\boldsymbol{k}}(z)|^2 -  \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} (z)\theta^*_{\boldsymbol{k}}(z) \}  } \geq 0 .
\end{equation}


\subsection{Uniform upper bound}
We first investigate the uniform in $R$ and $Pr$ upper bound on $\mean{w\theta}$, which we denote $U_0$.  Making the choices, $a =0$ and $\phi'(z) = 1+ b \eta(z)$ guarantees that $\mathcal{S}_{\boldsymbol{k}} \geq 0 $ for all $\boldsymbol{k}\neq 0$ in \eqref{eq:sk_non_uni}. Then the choice of background profile substituted into \eqref{eq:U_bound} gives 
\begin{equation}
    U_0 = \volav{ \frac{(1+b\eta(z))^2}{4b} } = \frac{1}{4b} + \volav{  \frac{\eta(z)}{2} + \frac{b \eta^2(z)}{4} } \, ,
\end{equation}
which is optimised with the choice $b = 1/ \lVert \eta \rVert_2 $
such that
\begin{equation}
    \label{eq:U0_uni_upper_non}
    U_0 = \frac{1}{2} \lVert \eta \rVert_2 + \frac{1}{2} \volav{ \eta(z) } \, .
\end{equation}
Given \eqref{eq:energy_bal_nu}, the uniform upper bound implies that 
\begin{equation}
    \label{eq:delt_T_uni}
    \mean{\delta T} \geq \sigma := \frac12 \volav{\eta(z)} - \frac12 \lVert \eta \rVert_2.
\end{equation}
The aim is to seek $\eta(z)$ that demonstrates $\mean{\delta T} \geq 0$. The uniform upper bound on $\mean{w\theta}$ in \eqref{eq:U0_uni_upper_non} can also be substituted into the definition of $Nu$ in \eqref{eq:Nu_non_u} which gives $Nu  \leq \volav{\eta(z)} / \sigma $.
As $R$ increases, the heat transport due to convection over conduction increases. In the asymptotic limit of $R=\infty$ where $U=U_0$,  $Nu=\infty$, can only occur if $\sigma=0$ since $\eta$ is bounded.
Implying directly that $\dT \geq 0$. For reference, in uniform internal heating where $H=1$ it follows that $\sigma = \frac12 - \frac{1}{\sqrt{3}}  < 0 $ and $\dT = \frac12 \left(\frac12 - \frac{1}{\sqrt{3}} \right)<0$.
We now next present a choice of background profile, building on \cite{Arslan2021a}, to obtain an $R$ dependent bound.


\section{Choice of background profile}
\label{sec:tau_field}

The $R$ scaling for any bound is given by constructing a $\phi'(z)$ with nonzero boundary layers. In analogy to the $H(z)=1$ case \citep{Arslan2021a}, we choose
\begin{equation}
    \label{eq:b_rel}
    b = \frac{ a +1}{ \lVert \eta \rVert_2 },
\end{equation}
and the background profile is taken to be  
\begin{equation}
	 \phi'= (a+1)
        \begin{dcases}
            \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta}, &  0\leq z \leq \delta, \\
           1 + \frac{ \eta(z)}{ \lVert \eta \rVert_2 },  &  \delta \leq z \leq 1-\delta,\\
            \left(1+ \frac{\eta(1-\delta)}{ \lVert \eta \rVert_2 }\right)\frac{(1-z)}{\delta},& 1-\delta \leq z \leq 1.
        \end{dcases}
        \label{eq:phi_prime}
\end{equation}

Due to the no-slip boundary condition \eqref{bc:u_non_u} and incompressibility, we have that $\hat{w}_{\boldsymbol{k}}(z)|_{z=\{0,1\} } =  \hat{w}_{\boldsymbol{k}}'(z)|_{z=\{0,1\} } = 0$. Then by use of the fundamental theorem of calculus and the Cauchy--Schwarz inequality we have that
\begin{equation}
    \hat{w}_{\boldsymbol{k}} \leq \frac23 z^{\frac32} \lVert \hat{ w}''_{\boldsymbol{k}}\rVert_2 . 
    \label{eq:w_est}
\end{equation}
Evaluating the sign-indefinite integral in \eqref{eq:sk_non_uni} for $\phi'(z)$ from \eqref{eq:phi_prime}, $b$ from \eqref{eq:b_rel}, $\hat{w}_{\boldsymbol{k}}$ from \eqref{eq:w_est} and using the Cauchy-Schwarz inequality gives in $[0,\delta]$
\begin{align}
    \int^{\delta}_0 &(a+1+ b \eta(z) - \phi'(z)) |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \nonumber\\ &\leq\int^{\delta}_0 \frac23 ( a+1)\left[1 + \frac{\eta(z)}{  \lVert \eta \rVert_2 } -  \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta} \right] z^{\frac32} \hat{\theta}_{\boldsymbol{k}} \textrm{d}z \lVert \hat{w}''_{\boldsymbol{k}}\rVert_2  \nonumber  \\
    &\leq \frac23(a+1)  \underbrace{\left(\int^{\delta}_0 \left[1 + \frac{\eta}{ \lVert \eta \rVert_2 } -  \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta} \right]^2 z^3 \textrm{d}z  \right)^{\frac12}}_{\Psi}  \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2 \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2.
    \label{eq:sign_indefinite_psi}
\end{align}
The same estimate holds for $[1-\delta,1]$.
The integrals $\Psi$ once evaluated for a particular profile $H(z)$ gives a necessary condition for $\delta$ to satisfy such that $\mathcal{S}_{\boldsymbol{k}}\geq 0$. Substituting \eqref{eq:sign_indefinite_psi} into \eqref{eq:sk_non_uni} gives
\begin{equation}
    \label{eq:sk_nonu}
    \mathcal{S}_{\boldsymbol{k}} \geq \frac{a}{R k^2} \lVert \hat{w}''_{\boldsymbol{k}}\rVert_2^2 + b k^2 \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2^2 - \frac43 ( a+1)\Psi \lVert \hat{w}''_{\boldsymbol{k}}\rVert_2 \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2 .
\end{equation} 
The homogeneous quadratic form is non-negative given it has a nonpositive discriminant, which holds when
\begin{equation}
    \label{eq:psi_sc}
      \Psi \leq \frac12 \sqrt{\frac{ 9 a }{R(a+1) \lVert \eta \rVert_2 } } ~ .
\end{equation}



Given $\phi'(z)$ from \eqref{eq:phi_prime} we now have  $U$, after substituting $b$ from \eqref{eq:b_rel} into \eqref{eq:U_bound} to get
\begin{align}
    U =&~ \frac{\delta(a+1)}{12 \lVert \eta \rVert_2}   \left[ \left( \lVert \eta \rVert_2 + \eta(\delta)\right)^2 + \left( \lVert \eta \rVert_2 + \eta(1-\delta) \right)^2 \right] + \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z\, .
    \label{eq:U_form_sub}
\end{align}

We next consider only $\eta(1)=1$ and take test profiles to calculate $\sigma$ and the uniform upper bound $U_0$ given by \eqref{eq:U0_uni_upper_non}. Then we demonstrate $R$ dependent bounds on $\mean{\delta T}$ and determine the value of $R$ above which inverse conduction cannot be ruled out.
 

\section{Non-uniform heating profiles}
\label{sec:non_uni_egs}


The family of heating profiles we consider are smooth profiles parameterised by $n\in \mathbb{R}_+ $ such that  
  \begin{equation}    
        \label{eq:heating_smooth}
        H(n,z) = (n+1)(1-z)^{n} \quad \forall n \geq 0.
\end{equation}
The corresponding $\eta(z)$ can be found using \eqref{eq:eta_general} and gives
\begin{equation}
    \label{eq:eta_1}
    \eta(n,z) = 1 - (1-z)^{n+1}.
\end{equation}
\begin{figure}
\hspace{-1cm}
    \centering
    \includegraphics[scale=0.9]{fig/non_uni1.eps}
    \begin{tikzpicture}[overlay]
        \node at (-11,3.5) {\textit{(a)}};
        \node at (-4.7,3.5) {\textit{(b)}};
    \end{tikzpicture}
    \caption{\textit{(a)} Plots of the heating profiles $H(z)$ given by \eqref{eq:heating_smooth} and \textit{(b)} plots of the heating distributions $\eta(z)$ given in \eqref{eq:eta_1} for $n\in[1,100]$ ({\color{mygrey}\solidrule}) with $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar6}\solidrule}) and $n=2$ ({\color{colorbar15}\solidrule}) highlighted.}
    \label{Fig:smooth_non_uni}
\end{figure}

In \cref{Fig:smooth_non_uni}  we plot example profiles of $H(z)$ and $\eta(z)$.
As $n$ increases the heating profile is a polynomial of increasing order with the heating becoming more localised to the lower boundary. At $n=\infty$ the heating profile becomes a Dirac delta distribution at $z=0$, whereas for $n=0$ the heating is profile is that of uniform internal heating. Evaluating first the integrals of $\eta$ gives
\begin{equation}
    \tag{\theequation{\textit{a,b}}}
     \volav{\eta} = \frac{n+1}{n+2}\, , \qquad
    \lVert \eta \rVert_2 = \sqrt{\frac{2 (n + 1)^2}{(n + 2)(2n + 3)}}\, . \label{eq:eta_int_1}
\end{equation}
Then $\sigma$ in \eqref{eq:delt_T_uni} is
\begin{equation}
     \sigma =  \frac{n+1}{2(n+2)} -  \frac{\sqrt{2}}{2}  \frac{n + 1}{\sqrt{ (n + 2)(2n + 3)} } \, .
     \label{eq:sig_1}
\end{equation}
Therefore, only when $n=\infty$ and the heating profile is a Dirac delta is the condition $\sigma=0$ satisfied. Stated in other words for the mean conductive heat flux, $\dT$, to be positive for all $R$ the heating is localised at the lower boundary exactly. The problem, in this case becomes equivalent, in some sense, to fixed flux Rayleigh-B\'enard convection \citep{Otero2002}. In fact the linear stability values can be shown to match. 
Given \eqref{eq:stab_lim}, substituting \eqref{eq:eta_1} for $\eta$ and evaluating the integral gives
\begin{subequations}
\begin{align}
        R_L = \frac{720}{ 1 - 60\frac{n^2+5n+6}{(n+6)(n+5)(n+4)(n+3)(n+2)} },  \\ R_E = \frac{5760}{\frac{1}{\gamma}(1+\gamma)(2 + \gamma ) - 24 \frac{60\gamma + (n+7)(60 + (n+6)(\gamma-5 + 2n\gamma+5n)))}{(n+7)(n+6)(n+5)(n+4)(n+3)(n+2)}}.
\end{align}
\end{subequations}
It is easy to confirm then for $n=0$ then $R_L=1440$, while for $n\rightarrow\infty$ then $R_L\rightarrow720$. Which are exactly the values of $R$ above which uniform internally heated and fixed flux Rayleigh--B\'enard convection respectively are linearly unstable \citep{Goluskin2016book}. If one optimises for 
$\gamma$ we obtain an expression for the energy stability in terms of $n$, where for $n=0$ the optimal $\gamma^*=\sqrt{35} /3$ and $R_E = 2880(6\sqrt{35} - 35)\approx 1429.86 < R_L$. In the case of Rayliegh--B\'enard convection $R_E=R_L$.


Next we determine the condition for which $\mathcal{S}_{\boldsymbol{k}}\geq 0 $ by evaluating $\Psi$ in \eqref{eq:sign_indefinite_psi}.
Given \eqref{eq:eta_1} and \eqref{eq:eta_int_1} then $\eta(z) \leq 1$ $\forall n$, and $-(\eta(\delta)/\lVert \eta \rVert_2 ) \leq 0 $ such that 
\begin{eqnarray}
    \Psi \leq  \left( \int^{\delta}_0 \left[1 + \frac{1}{\lVert \eta \rVert_2}  \right]^2 z^3 \textrm{d}z \right)^{1/2} = \frac{\delta^2}{2} \left(1 + \frac{1}{\lVert \eta \rVert_2 }\right) .
\end{eqnarray}
The condition for the positivity of $\mathcal{S}_{\boldsymbol{k}}$ becomes
\begin{equation}
    \label{eq:delta_cond}
    \delta  \leq \left( \frac{81 a \lVert \eta \rVert_2}{R( a+1) \left(1 + \lVert \eta \rVert_2  \right)^2 } \right)^{1/4} \, .
\end{equation}
Next we evaluate $U$ as given by \eqref{eq:U_form_sub} with \eqref{eq:eta_1}. We first state a preliminary result. For all $\delta < 1$ we can make the estimate that
\begin{align}
    (1-\delta)^{n+2} &= 1 - (n+2)\delta + \sum^{n+2}_{2}  \begin{pmatrix} n+2 \\ 2 \end{pmatrix} (-\delta)^{k} 
    \geq 1 - (n+2)\delta.
    \label{eq:est_bound}
\end{align}
Then, assuming that $\eta(\delta)\leq 1$, $\eta(1-\delta) \leq 1$ and $(1-\delta)^{2n+3} - \delta^{2n+3} \leq 1$ for all $n$, after substituting \eqref{eq:eta_1} into \eqref{eq:U_form_sub} evaluating the integral using \eqref{eq:est_bound} and rearranging we obtain
\begin{align}
    U 
    % \leq&~ \frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2   + \frac{a+1}{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\lVert \eta \rVert_2 + 1 - (1-z)^{n+1} \right)^2 \textrm{d}z \nonumber \\ 
    \leq &\frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2  + \frac{a+1}{4\lVert \eta \rVert_2}\Big((1+ \lVert \eta \rVert_2)^2(1-2\delta)  + \frac{2(1+\lVert \eta \rVert_2) }{(n+2)} (\delta^{n+2} - (1-\delta)^{n+2})  \nonumber \\
    & \hspace{5cm} - \frac{\delta^{2n+3} - (1-\delta)^{2n+3}}{2n+3}  \Big) \nonumber
    \\
    \leq&~ \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2} + \frac{1}{2n+3} \right)  \nonumber
    \\ & \hspace{5cm} -\frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - 1 -\frac{3\delta^{n+1}}{n+2}  \right)\delta  .
\end{align}
A higher order $\delta$ term remains, we let $\delta^{n+1}  \leq m (n+2)$, to obtain
\begin{align}
    U \leq& ~  \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right)  -   \frac{ \delta(a+1)(1+ \lVert \eta \rVert_2)(   2 \lVert \eta \rVert_2 - 1 -3m  )}{6\lVert \eta \rVert_2}  .
\end{align}
For a bound of the form $U\leq U_0(n) - c(n)R^{-\beta}$, we require $  2 \lVert \eta \rVert_2 - 1 -3m \geq0$. 
% At $n=0$ we require $m\leq \frac{-3+2\sqrt{3}}{9}$, while for $n\rightarrow\infty$ the condition is that $m\leq \frac16$. 
Given that $\lVert \eta \rVert_2$ monotonically increases for all $n$ for we take $m =  \frac{1}{21}$, such that the condition holds for all $n$.
The bound that follows holds provided $ \delta^{n+1} \leq      \tfrac{1}{21}(n+2) $.
Finally we have that
\begin{align}
    \label{eq:U_nearly}
    U \leq&~  \underbrace{\frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right) }_{U_0} -  \delta \, \frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - \frac87 \right) .
\end{align}
We determined $\delta$ in \eqref{eq:delta_cond}. If we take $\delta$ as large as possible and substitute into \eqref{eq:U_nearly}, and since $a>0$ then $a+1\geq1$ gives
\begin{align}
    U \leq& U_0  - U_1 \frac{a^{1/4}}{R^{1/4}} , \qquad \text{where}\quad U_1 = \frac{  (1+ \lVert \eta \rVert_2)^{1/2}}{2 \, \lVert \eta \rVert_2^{3/4}} \left(   2 \lVert \eta \rVert_2 - \frac87 \right) .
    \label{eq:U_final_forms}
\end{align}
Minimising \eqref{eq:U_final_forms} with respect to $a$ by solving $\partial_a U =0$ gives
\begin{equation}
    a = \left(\frac{U_1}{4 U_0} \right)^{4/3}    R^{-1/3},
\end{equation}
such that
\begin{align}
\tag{\theequation{\textit{a,b}}}
    \wT \leq U_0 - \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{1/3} R^{-1/3} , \qquad \mean{\delta T} \geq \frac{n+1}{n+2} -  U_0 + \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{1/3} R^{-1/3}\, .
 \end{align}
 %
\begin{figure}
% \hspace{-1cm}
    \centering
    \includegraphics[scale=0.92]{fig/DT_1.eps}
        \begin{tikzpicture}[overlay]
        \node at (-11.3,3.4) {\textit{(a)}};
        \node at (-7.15,3.4) {\textit{(b)}};
        \node at (-3,3.4)
        {\textit{(c)}} ;
    \end{tikzpicture}
    \caption[Lower bounds on dT]{ \textit{(a)} Plots of the lower bounds on $\mean{\delta T}$, with
    heating profiles $H(z)$ given by \eqref{eq:heating_smooth} for $n\in[0,100]$ ({\color{mygrey}\solidrule}) with $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar6}\solidrule}), $n=2$ ({\color{colorbar15}\solidrule}) and $n=\infty$ ({\solidrule}). \textit{(b)} Plots of $R_n$ at which the lower bound on $\mean{\delta T}$ becomes equal to zero for given $n$ and \textit{(c)} plots of $|\sigma|$ as given in \eqref{eq:sig_1} against $n$ for the heating profiles of \eqref{eq:heating_smooth}. }
    \label{fig:bound_dT_1}
\end{figure}
%
The bound on $\mean{\delta T}$ can be rearranged and simplified using \eqref{eq:eta_int_1} to obtain
\begin{align}
    \label{eq:delt_T_main_result}
    \mean{\delta T} \geq& ~ \sigma  +  \frac{ 3 }{16\lVert \eta \rVert_2} \left(\frac{2(1+\lVert \eta\rVert_2)^2(2\lVert \eta \rVert_2 - \tfrac87)^4}{\frac{n+1}{n+2} + \lVert \eta \rVert_2  } \right)^{1/3}
   R^{-1/3}\, .
\end{align}
Observe that if $n=0$, we have the results of \cite{Arslan2021a}
\begin{equation}
\tag{\theequation{\textit{a,b,c}}}
    \wT \leq \frac{3+2\sqrt{3}}{12} - c R^{-1/3} , \quad  \mean{\delta T} \geq \frac{3-2\sqrt{3}}{12} +   cR^{-1/3}\, ,\quad      Nu \leq \left(\frac{3-2\sqrt{3}}{6} + c R^{-1/3}\right)^{-1},
\end{equation}
where instead $c\approx 0.0015$.
As a note the prefactor in the bound is smaller than that demonstrated in \cite{Arslan2021a}, due to the difference between the two choice of the range of $\delta$. The restriction of $m\leq \frac{1}{21}$, restricts the $\delta$ to have to be below $\frac{-6+4\sqrt{3}}{9}$ for $n=0$. Crucially note that for some $R>R_n$ inverse conduction occurs where $\mean{\delta T} < 0$ except for $n = \infty$ when
\begin{equation}
    \wT \leq 1 - c R^{-1/3},  \qquad   \dT \geq c R^{-1/3},  \qquad   Nu \leq c^{-1} R^{1/3},
\end{equation}
and where $c \approx 0.2423$ which once again is smaller than the constant appearing in \cite{Otero2002}.
The novel result of this paper is the intermediate behaviour of $\dT$ as $n$ varies. We find from \eqref{eq:delt_T_main_result} that $\mean{\delta T} \geq \sigma + c R^{-1/3}$ where $|\sigma|\sim \frac{1}{n}$ and $c \sim \mathcal{O}(10^{-1})$. As such for a given heating profile $H(z)$ parameterised by $n$ in \eqref{eq:heating_smooth}, the value of the $R$ above which $\mean{\delta T}\leq 0$, $R_n$, for sufficiently large $n$ scales as $R_n \sim n^3$. 

The other quantity of interest for IHC is $\mean{T}$. Substituting \eqref{eq:eta_1} into \eqref{eq:T_uniform} we have  the following uniform in $R$ bounds
\begin{equation}
    \mean{T} \leq \frac12 \left(1-\frac{2}{(n+2)(n+3)}\right).
\end{equation}
For uniform internal heating $0< \mean{T} \leq\frac13$, while if $n=\infty$ then $\mean{T}\leq \frac12$ which decreases the previously known best upper bound on $\mean{T}$ for Rayleigh-B\'enard convection \cite[Table 1]{Goluskin2016book}. While not demonstrated here, it follows trivially to bound $\mean{T}$ from below for non-uniform heating given by \eqref{eq:heating_smooth}, which would give $\mean{T} \geq c(n) R^{-1/3}$.  




\section{Discussion}

We have demonstrated that for mean one non-uniform IHC the mean conductive heat transport $\dT$ is bounded by $\sigma(\eta) + c(\eta)R^{-1/3}$. Where $\sigma \leq 0$ and as the heating is localised towards the lower boundary, $\sigma \rightarrow 0$, eventually becoming zero when all of the heating happens at $z=0$. In this limit the problem is equivalent to Rayleigh-B\'enard convection with fixed flux boundaries, and both the bounds and linear stability of the problem match. We choose one particular polynomial class of mean one heating profiles \eqref{eq:heating_smooth} parameterised by $n$. For which we can demonstrate that as the heating is localised to the lower boundary, $n$ increases, the $R$ above which inverse conduction ($\dT < 0$) cannot be ruled grows as $n^3$. Additionally with \eqref{eq:heating_smooth}
we can demonstrate a uniform upper bound on $\mean{T}$, which in the limit of $n\rightarrow\infty$ improves on the previously known upper bound for $\mean{T} $ in Rayleigh-B\'enard convection, with fixed flux. 

One weak implication of the results is that Rayleigh-B\'enard convection with fixed flux boundary conditions is a limit of the problem considered here of non-uniform IHC with fixed flux boundaries. The bounds and in \cref{sec:non_uni_egs} match those first shown in \cite{Otero2002} when the heating profiles of \eqref{eq:heating_smooth} are taken to the limit $n\rightarrow\infty$. While the mathematical implication of this statement is an open question, the physical intuition is justified. However, the additional problem to consider is on the definition of the Rayleigh number. The Rayleigh number between boundary and IHC is different and based on scales in the flow, as such for a stronger statement to be made we would want to use a universal Rayleigh number definition that can generalise both flows. 

Finally, the heating profiles considered here are of a one particular type only; mean one heating ($\eta(1)=1$), non-negative and monotonically decreasing in $z$ (excluding $n=0$ where the heating is constant in $z$). The choice is made to highlight the effects of increasingly concentrating the heating region at the lower boundary on inverse conduction. With the final result being that inverse conduction cannot be ruled out for all $R$ even if the internal heating occurs at arbitrarily small $z$. Indicating a limitation of bounding by quadratic auxiliary functionals.  
Alternative choices can be of interest to investigate different features of IHC. For example, in the case of IHC between isothermal boundaries, it may be of interest to consider if there are heating profiles that can improve on the exponential bounds of  \cite{kumar2021ihc}.   




==> v3.tex <==
\section{Introduction}

Convection is ubiquitous in nature. 


\section{Setup}

We consider a layer of fluid between two horizontal plates separated by a distance $d$ and periodic in the horizontal ($x$ and $y$) directions with periods $L_x$ and $L_y$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Gravity acts in the negative vertical direction $z$, and the fluid is heated internally at a volumetric rate $\Tilde{H}$.
The dimensional heating is written as $\Tilde{H}=H_0 H(z)$ with $H_0$ defined as $H_0 = \lVert H \rVert_1 $ and $H(z)$ is an arbitrary function of only $z$. Here and throughout the paper $\lVert f \rVert_p$ is the standard $L^p$ norm of a function $f=f(z)$.

To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2H_0/\kappa \rho c_p$ as the temperature scale \citep{roberts1967convection}. The velocity of the fluid $\boldsymbol{u}=(u,v,w)$ and temeprature $T$ in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ is then governed by the Boussinesq equations
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
The usual non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa}
    \qquad\text{and}\qquad 
    R = \frac{g \alpha H_0 d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are taken to be no-slip and fixed flux:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:T_f}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-\eta(1),
\end{gather}
\end{subequations} 
where we introduce a measure of the vertical energy flux $\eta(z) \in L^2(0,1)$ defined as,
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z)\, \textrm{d}z.
\end{equation}
Then, $\eta(1)$ sets the total energy flux out of the system.
% A statistically stationary state can be achieved when $\eta(1)=1$, corresponding to mean one heating/cooling in the domain \citep{Goluskin2016book,Arslan2021a}. Alternatively, one could take $\eta(1)=0$ (mean zero heating/cooling).
We can obtain an identity of the heat transport of the system by multiplying \eqref{eq:nondim_energy_nonUniform} by $z$ and taking an infinite time and volume average. Then after use of \eqref{eq:eta_general} and a standard application of integration by parts with the boundary conditions \eqref{bc:u_non_u} \& \eqref{bc:T_f} the resulting identity can be written as
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}} &= \volav{\eta(z)}.
\end{align}
The left hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical convective heat flux, $\wT$, and the mean conductive heat flux,
\begin{equation}
\dT = \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}}.
\end{equation}
Inverse conduction occurs if $\dT$ is negative and so to rule this out requires demonstrating that $\dT\geq0$ for all $R$. In \cite{Arslan2021a} the authors consider the case of uniform heating where $\eta = z$, however they are only able to prove that $\dT \geq - \frac{2\sqrt{3} - 3}{12}$.


Finally, to remove the inhomogeneous boundary conditions on $T$ it is convenient to rewrite the temperature field in terms of perturbations from the conductive profile $T_c$,
\begin{equation}
    \label{eq:}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition it follows that $T'_c = - \eta(z)$, where primes denote derivatives with respect to $z$. Then, writing \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ gives
\begin{gather}
    \label{eq:theta_eq}
     \partial_t \theta + \boldsymbol{u} \cdot \nabla \theta = \Delta \theta + w\, \eta(z) ,\\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{gather}

\section{Bounding heat transport}

To investigate inverse conduction while retaining similarities with previous studies of IHC and RBC  \citep{Arslan2021a}, we search for an upper bound on $\wT$ and use \eqref{eq:energy_bal_nu} to bound $\dT$. First, we realise that $\wT = \mean{w\theta}$, since by incompressibilty and the boundary conditions \eqref{bc:u_non_u}, we have the property that
\begin{equation}
    \volav{w f(z)} = \int^{1}_0 \horav{w} f \textrm{d}z = 0.
\end{equation}
In what follows the auxiliary functional method is used to prove an upper bound on $\mean{w\theta}$. 


\subsection{The auxiliary functional method}

Rigorous bounds on the bulk quantities of turbulent flows can be derived using the auxiliary functional method \citep{Chernyshenko2014}. In particular, we consider the following quadratic auxiliary functional
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},\theta\} = \volav{ \frac{a}{2\,Pr\,R} |\boldsymbol{u}|^2 + \frac{b}{2}\left|\theta  - \frac{\phi(z)}{b}\right|^2 },
\end{equation}
where $a$ and $b$ are non-negative scalars and $\phi(z)$ a function to be optimised over. As demonstrated by \cite{Chernyshenko2022} use of quadratic auxiliary functionals makes the method employed equivalent to the background field method where $a$ and $b$ are referred to as balance parameters and $\phi/b$ is the background temperature field. Then, given that $\mathcal{V}\{\boldsymbol{u},\theta\}$ remains bounded in time along solutions of \eqref{eq:mom_eq} \& \eqref{eq:theta_eq} for any given initial $\boldsymbol{u}$ and $\theta$. We can write
\begin{equation}
    \label{eq:AFM_statemen}
    \mean{w\theta} = U - \left( \overline{U - \volav{w\theta} - \frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\} } \right),
\end{equation}
from which we deduce that $\mean{w \theta} \leq U$ if the term in the bracket in \eqref{eq:AFM_statemen} is non-negative. Computations analogous to \cite{Arslan2021a} show that the optimal bound provable is given by
\begin{equation}
    \label{eq:U_bound}
    U = \volav{\frac{\phi'(z)^2}{4b}},
\end{equation}
provided that the following condition, hereby referred to as the \textit{spectral constraint}, is satisfied
\begin{equation}
    \label{eq:sk_non_uni}
    \volav{  \frac{a|w''_{\boldsymbol{k}}(z)|^2}{R\,k^2}  + b k^2|\theta'_{\boldsymbol{k}}(z)|^2 -  \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} (z)\theta^*_{\boldsymbol{k}}(z) \}  } \geq 0. 
\end{equation}
The spectral constraint must hold for all nonzero $\boldsymbol{k}$ where the magnitude of the wavevector $\boldsymbol{k}^2 = k_x^2 + k_y^2$ arises by exploiting the horizontal periodicity in Fourier space. The corresponding boundary conditions become
\begin{gather}
    \label{bc:w_k}
    \hat{w}_{\boldsymbol{k}}(0)= \hat{w}_{\boldsymbol{k}}(1)= \hat{w}_{\boldsymbol{k}}'(0)= \hat{w}_{\boldsymbol{k}}'(1)=0,\\
    \label{bc:T_k}
     \hat{\theta}_{\boldsymbol{k}}'(0) =  \hat{\theta}_{\boldsymbol{k}}'(1) =0.
\end{gather}

% \subsection{Background temperature field}
\subsection{Ans\"atz}

An explicit bound is obtained by evaluating $U$ with three particular choices. These are
\begin{itemize}
    \item a relation between the balance parameters of
\begin{equation}
    \label{eq:b_relation}
    b = \frac{a+1}{\lVert \eta \rVert_2}.
\end{equation}
    \item A choice of background temperature profile of
    \begin{equation}
	 \phi'= (a+1)
        \begin{dcases}
            \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta}, &  0\leq z \leq \delta, \\
           1 + \frac{ \eta(z)}{ \lVert \eta \rVert_2 },  &  \delta \leq z \leq 1-\varepsilon,\\
            \left(1+ \frac{\eta(1-\varepsilon)}{ \lVert \eta \rVert_2 }\right)\frac{(1-z)}{\varepsilon},& 1-\varepsilon \leq z \leq 1,
        \end{dcases}
        \label{eq:phi_prime}
    \end{equation}
    where $\delta$ and $\varepsilon$ are the widths of the boundary layers of $\phi(z)$ at the lower and upper boundaries respectively.
    \item Non-uniform heating functions where
\begin{equation}
    \label{eq:eta_cond}
    \eta(1) = 1.
\end{equation}
\end{itemize}
These three choices come about from three observations. The first is that if $\phi'(z) = a+1+b\eta(z)$, the spectral constraint in \eqref{eq:sk_non_uni} is immediately satisfied. The resultant $U$ can be optimised for $b$ to obtain the relation \eqref{eq:b_relation}. However this choice of $\phi'$ does not give a $R$ dependent bound $U$. Instead if we permit $\phi'$ to have boundary layers of widths $\delta$ and $\varepsilon$, the spectral constraint will yield a $R$ dependent condition. Finally, to allow for a comparison of the results with uniform IHC \citep{Arslan2021a} then we consider only $H$ such that \eqref{eq:eta_cond} holds.

Substituting \eqref{eq:phi_prime} and \eqref{eq:b_relation} into \eqref{eq:U_bound} and given \eqref{eq:eta_cond} and the definition of $\eta(z)$ then $\eta(z) \leq 1$ such that
\begin{multline}
    U = \frac{(a+1)}{12 \lVert \eta \rVert_2}   \left[ \delta\left( \lVert \eta \rVert_2 + \eta(\delta)\right)^2 + \varepsilon \left( \lVert \eta \rVert_2 + \eta(1-\varepsilon) \right)^2 \right] \\ +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\varepsilon}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z\, .
    \label{eq:U_form_sub}
\end{multline}
The strategy to obtain a $R$ dependent bound is to determine, for a particular choice of $\eta$, the variation of $\delta$ and $\varepsilon$ with $R$ that satisfies the spectral constraint in \eqref{eq:sk_non_uni}. Given the choice of $\phi'(z)$ in \eqref{eq:phi_prime} then \eqref{eq:sk_non_uni} can be simplified to 
\begin{equation}
    \label{eq:sk-cond_2}
    \frac{a}{R k^2} \lVert \hat{w}_{\boldsymbol{k}}^2 \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2^2 - \frac{a+1}{\lVert \eta \rVert_2} \left( \int_0^\delta f_1 |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z + \int_{1-\varepsilon}^1 f_2 |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \right)  \geq 0,
\end{equation}
where
\begin{equation}
    f_1 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(\delta))\frac{z}{\delta}, \quad   f_2 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(1-\varepsilon))\frac{1-z}{\varepsilon}.
\end{equation}
The sign-indefinite integrals in \eqref{eq:sk-cond_2} can be further estimated. First, given the boundary conditions on $\hat{w}_{\boldsymbol{k}}$ in \eqref{bc:w_k} use of the fundamental theorem of calculus and Cauchy-Schwarz gives
% \begin{equation}
%     \hat{w}'_{\boldsymbol{k}}(z) = \int^{z}_0 \hat{w}_{\boldsymbol{k}}''(\xi) \textrm{d}\xi \leq \sqrt{z}\, \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2,
% \end{equation}
% therefore 
\begin{equation}
\label{eq:w_estimate}
     \hat{w}_{\boldsymbol{k}}(z) = \int^{z}_0 \int^{\xi}_0 \hat{w}_{\boldsymbol{k}}''(\sigma) \textrm{d}\sigma \textrm{d}\xi \leq \int^{z}_0 \sqrt{\xi} \, \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_{2} \,\textrm{d}\xi  = \frac23 z^\frac32\, \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2.
\end{equation}
Using \eqref{eq:w_estimate} and the Cauchy-Schwarz inequality we can estimate the terms in \eqref{eq:sk-cond_2} to obtain
\begin{subequations}
\begin{gather}
    \int^{\delta}_0 f_1 |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \leq \frac23 \int^{\delta}_0 f_1 \, z^{\frac32} \, \hat{\theta}_{\boldsymbol{k}} \textrm{d}z \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2 \leq \frac23 \left( \int^{\delta}_0 f_1^2 z^3 \textrm{d}z \right)^{\frac12} \lVert \hat{\theta}_{\boldsymbol{k}} \rVert_2 \lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2 ,\\
     \int^{1}_{1-\varepsilon} f_2 |\hat{w}_{\boldsymbol{k}} \hat{\theta}_{\boldsymbol{k}}| \textrm{d}z \leq \frac23 \left( \int^{1}_{1-\varepsilon} f_2^2 z^3 \textrm{d}z \right)^{\frac12} \lVert \hat{\theta}_{\boldsymbol{k}} \rVert_2 \lVert \hat{w}''_{\boldsymbol{k}} \rVert_2 .
 \end{gather}
\end{subequations}
The spectral constraint \eqref{eq:sk-cond_2} can be written as a homogeneous quadratic form in $\lVert \hat{w}_{\boldsymbol{k}}'' \rVert_2$ and $\lVert \hat{\theta}_{\boldsymbol{k}}\rVert_2$, which is non-negative when it has a nonpositive discriminant. This condition can be written as
\begin{equation}
    \label{eq:sk_cond_ineq}
    \left[ \left( \int^{\delta}_0 f_1^2 z^3 \textrm{d}z
    \right)^{\frac12} + \left( \int^{1}_{1-\varepsilon} f_2^2 (1-z)^3 \textrm{d}z \right)^{\frac12} \right]^2 \leq \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) R }.
\end{equation}
An exact relations of the form $\delta = \delta(a,R)$ and $\varepsilon = \varepsilon(a,R)$ can be found after evaluating the integrals for a choice of heating profile $H(z)$.     

\section{Non-uniform heating}

Given that for convection observed in nature the heating and cooling need not be uniform, in the bounding problem as outlined so far the only restriction has been that $\eta$ is in $L^2$. As a first approach to investigate inverse conduction, considered a class of non-uniform heating profile, that can be tuned to concentrate the energy input towards $z=0$. For such a family of profiles we first derive a lower bound on the mean conductive heat transport. Before obtaining an exact relation for the $R=R_c$ above which inverse conduction cannot be ruled out as the heating is varied to concentrate closer to the lower boundary. 
To draw a direct parallel with the results of \cite{Arslan2021a} we consider the class of $H(z)$ where $\eta(1)=1$. 


\subsection{Example: polynomial heating}


A simple choice of smooth heating profile is made with the property $\eta(1)=1$ and where a single parameter can be used to concentrate the heating to the lower boundary. For $n\in [0,\infty)$ we consider the family of smooth functions  
\begin{equation}
    \label{eq:H_1}
    H(n,z) = (n+1)(1-z)^n.
\end{equation}
Then by \eqref{eq:eta_general} we have that
\begin{equation}
\label{eq:eta_1}
    \eta(n,z) = 1 - (1-z)^{n+1}.
\end{equation}
If $n=0$ the profile is equivalent to uniform internal heating, whereas when we let $n\rightarrow\infty$ then the heating profile increasingly approximates a Dirac delta at the lower boundary. The limit of $n=\infty$ is physically equivalent to Rayleigh-B\'enard convection with fixed flux boundary conditions. 
% For the choice \eqref{eq:eta_1}, measures of the available energy in the system are given by $\volav{\eta}$ and $\lVert \eta \rVert_2$ and in terms of $n$ are
% \begin{gather}
%     \volav{\eta} = \frac{n+1}{n+2}\, , \qquad \lVert \eta \rVert_2 = \sqrt{\frac{2(n+1)^2}{(n+2)(2n+3)}}\, .
% \end{gather}
% With the choice of $\eta$ made we can obtain relations for $\delta$ and $\varepsilon$ with $R$ and $n$.

From \eqref{eq:eta_1}, observe that $\eta(n,z)\leq 1$ for all $n$ therefore estimating from above gives
\begin{equation}
    \label{eq:F_simp}
    f_1 = f_2  \leq \lVert \eta \rVert_2 + 1.
\end{equation}
Using \eqref{eq:F_simp} the condition in  \eqref{eq:sk_cond_ineq} becomes
\begin{equation}
    \delta^2 + \varepsilon^2 \leq \sqrt{\frac{36a \lVert \eta \rVert_2 }{(a+1)(1+\lVert \eta \rVert_2)^2 R } } .
\end{equation}
For increasing $n$, the heating profile becomes increasingly asymmetric towards the lower boundary. However, to simplify the algebra initially we let $\delta=\varepsilon$ in the background field, which implies that 
\begin{equation}
    \label{eq:delta_cond}
    \delta \leq \left(\frac{144a \lVert \eta \rVert_2 }{(a+1)(1+\lVert \eta \rVert_2)^2 R } \right)^{\frac14}. 
\end{equation}
Next we turn to evaluating $U$ in \eqref{eq:U_form_sub} with $\eta$ given by \eqref{eq:eta_1}. We first state a preliminary result. For all $\delta < 1$ we can make the estimate
\begin{align}
    (1-\delta)^{n+2} &= 1 - (n+2)\delta + \sum^{n+2}_{2}  \begin{pmatrix} n+2 \\ 2 \end{pmatrix} (-\delta)^{k} 
    \geq 1 - (n+2)\delta.
    \label{eq:est_bound}
\end{align}
Then, since $\eta(\delta)\leq 1$, $\eta(1-\varepsilon) \leq 1$ and $(1-\delta)^{2n+3} - \delta^{2n+3} \leq 1$ for all $n$,  substituting \eqref{eq:eta_1} into \eqref{eq:U_form_sub}, estimating by using \eqref{eq:est_bound} and rearranging gives
\begin{align}
    U 
    % \leq&~ \frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2   + \frac{a+1}{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\lVert \eta \rVert_2 + 1 - (1-z)^{n+1} \right)^2 \textrm{d}z \nonumber \\ 
    \leq &\frac{\delta (a+1)}{6\lVert \eta \rVert_2}   \left(1 + \lVert \eta \rVert_2 \right)^2  + \frac{a+1}{4\lVert \eta \rVert_2}\Big((1+ \lVert \eta \rVert_2)^2(1-2\delta)  + \frac{2(1+\lVert \eta \rVert_2) }{(n+2)} (\delta^{n+2} - (1-\delta)^{n+2})  \nonumber \\
    & \hspace{5cm} - \frac{\delta^{2n+3} - (1-\delta)^{2n+3}}{2n+3}  \Big) \nonumber
    \\
    \leq&~ \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2 (1+\lVert \eta \rVert_2)}{n+2} + \frac{1}{2n+3} \right)  \nonumber
    \\ & \hspace{5cm} -\frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - 1 -\frac{3\delta^{n+1}}{n+2}  \right)\delta  .
    \label{eq:U_exp_2}
\end{align}
A higher order $\delta$ term remains in \eqref{eq:U_exp_2}, so let $\delta^{n+1}  \leq m (n+2)$, to obtain
\begin{align}
    U \leq& ~  \frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right)  -   \frac{ \delta(a+1)(1+ \lVert \eta \rVert_2)(   2 \lVert \eta \rVert_2 - 1 -3m  )}{6\lVert \eta \rVert_2}  .
\end{align}
For a bound of the form $U\leq U_0(n) - c(n)R^{-\beta}$, we require $  2 \lVert \eta \rVert_2 - 1 -3m \geq0$. 
% At $n=0$ we require $m\leq \frac{-3+2\sqrt{3}}{9}$, while for $n\rightarrow\infty$ the condition is that $m\leq \frac16$. 
Given that $\lVert \eta \rVert_2$ monotonically increases for all $n$ for we take $m =  \frac{1}{21}$, such that the condition holds for all $n$.
The bound that follows holds provided $ \delta^{n+1} \leq   \tfrac{1}{21}(n+2) $.
Finally $U$ is bounded from above by
\begin{align}
    \label{eq:U_nearly}
    U \leq&~  \underbrace{\frac{a+1}{4 \lVert \eta \rVert_2 } \left(  (1+\lVert \eta \rVert_2 )^2 - \frac{2(1+\lVert \eta \rVert_2)}{n+2}  + \frac{1}{2n+3} \right) }_{U_0} -  \delta \, \frac{ (a+1)(1+ \lVert \eta \rVert_2)}{6\lVert \eta \rVert_2} \left(   2 \lVert \eta \rVert_2 - \frac87 \right) .
\end{align}
In the condition \eqref{eq:delta_cond} if we take $\delta$ as large as possible and substitute into \eqref{eq:U_nearly} and since $a>0$ then $a+1\geq1$ which gives
\begin{equation}
    U \leq U_0  - U_1 \frac{a^{1/4}}{R^{1/4}} , \qquad \text{where}\quad U_1 = \frac{  (1+ \lVert \eta \rVert_2)^{1/2}}{2 \, \lVert \eta \rVert_2^{3/4}} \left(   2 \lVert \eta \rVert_2 - \frac87 \right) .
    \label{eq:U_final_forms}
\end{equation}
Minimising \eqref{eq:U_final_forms} with respect to $a$ by solving $\partial_a U =0$ gives
\begin{equation}
    a^* = \left(\frac{U_1}{4 U_0} \right)^{4/3}    R^{-1/3}.
\end{equation}
Finally, substituting for $a$ with the optimal $a^*$ gives  
\begin{gather}
    \mean{w\theta} \leq U_0 - \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{1/3} R^{-1/3} .
    % \mean{\delta T} \geq \frac{n+1}{n+2} -  U_0 + \frac34 \left(\frac{U_1^4}{4 U_0} \right)^{1/3} R^{-1/3}\, .
 \end{gather}
The mean conductive heat transport can be obtained after use of the identity \eqref{eq:energy_bal_nu} and rearranging, such that
\begin{align}
    \label{eq:delt_T_main_result}
    \mean{\delta T} \geq& ~  \frac{n+1}{2(n+2)} - \frac{ \lVert \eta \rVert_2 }{2} +  \frac{ 3 }{16\lVert \eta \rVert_2} \left(\frac{2(1+\lVert \eta\rVert_2)^2(2\lVert \eta \rVert_2 - \tfrac87)^4}{\frac{n+1}{n+2} + \lVert \eta \rVert_2  } \right)^{1/3}
   R^{-1/3}\, .
\end{align}
It can be easily verified that in the case of $n=0$ (uniform heating) the bounds are, up to constants, identical to that in \cite{Arslan2021a}. Inverse conduction occurs is defined as $\dT < 0$, such that the critical $R=R_c$ above which inverse conduction cannot be ruled out can be is given by
\begin{equation}
    R_c =  \frac{ 27(1+\lVert \eta\rVert_2)^2(2\lVert \eta \rVert_2 - \tfrac87)^4  } { 256\, \lVert \eta \rVert_2^3(\lVert \eta \rVert_2 - \frac{n+1}{n+2} )^3 ( \lVert \eta \rVert_2 + \frac{n+1}{n+2}  ) }.
\end{equation}
where for sufficiently large $n$, $R_c$ scales as $n^3$. 


\subsection{Interpolating IHC and RBC}

The $H(z)$ in \eqref{eq:H_1} and choice of non-dimensionalisation does not allow us to pass to the limit of $n\rightarrow\infty$. Nevertheless some statements can be made as $n$ increases, and the flow goes from uniform IHC towards, but never equal to, RBC. First off in the limit of $n=\infty$ since $R_c \rightarrow\infty$ inverse conduction can be ruled out. As such, for IHC with non-uniform heating it is not possible to rule out inverse conduction for all $R$ if any heating occurs within the domain. 

The flows of RBC and uniform IHC between fixed flux boundaries have other key differences. One of which is the $R$ at which the system is linearly unstable. Due to the boundary conditions, closed analytic expressions can be obtained for linear instability. Starting with uniform IHC, if instead a non-uniform heating profile, as given by \eqref{eq:H_1} were to be used the using the same procedure as in \cite{Goluskin2015a} gives
\begin{equation}
    \label{eq:RL}
    R_L = \frac{1}{\int^{1}_0 \eta(z) P(z) \textrm{d}z } = \frac{720}{1- 60 \frac{n^2+5n+6}{(n+6)(n+5)(n+4)(n+3)(n+2)}}
\end{equation}
where $P(z)$ is a polynomial more generally dependent on the velocity boundary conditions. Curiously if we take $n=0$ in \eqref{eq:RL} then $R_L = 1440$ as reported in \cite{Goluskin2015a}, while in the limit of $n\rightarrow\infty$, $R_L \rightarrow 720$, which corresponds to the known value fo linear instability for RBC between fixed flux boundaries \citep{Goluskin2016book}. An additional feature for both systems is that the mean temperature, $\mean{T}$, is uniformly bounded from above. As seen in Table 1 of \cite{Goluskin2016book}. Interestingly, when working with non-uniform heating multiplying \eqref{eq:nondim_energy_nonUniform} by $z^2$ and integrating by parts where $H(z)$ is given by \eqref{eq:H_1} gives
\begin{equation}
    \mean{T} \leq \frac12\left(1 - \frac{2}{(n+2)(n+3)} \right). 
\end{equation}
For $n=0$ this matches the known result from \cite{Goluskin2016book} of $\mean{T} \leq \frac13$, whereas in the limit of $n= \infty$ gives that $\mean{T} \leq \frac12$. This would be an improvement to the results known for RBC between fixed flux boundaries. The lower bound on $\mean{T}$ demonstrated for uniform IHC \citep{Goluskin2015a} can be shown to apply, with the same $R$ scaling for all $H(z)$ given by \eqref{eq:H_1}. Parameterised in terms of $n$, and $R$ the bound would be $\mean{T} \geq c(n) R^{-1/3}$, where $0<c(n)<\infty$ for all $n$.  

\subsection{General heating/cooling}

The results in the preceding section correspond to a family of non-uniform heating profiles of which uniform IHC is one member. 


\section{Discussion}

==> v3b.tex <==
\section{Introduction}
\label{sec:intro}


Whether driven by the boundaries, internal heat sources, or a mixture of both, thermal convection is ubiquitous in nature. Convection of a fluid between a hot lower plate and cold upper plate, Rayleigh-B\'enard convection (RBC), has been well studied \citep{chilla2012new, Ahlers2009}. Of interest is an understanding of the effects of turbulent convection, on the bulk quantities of the flow like the mean convective heat transport. 
For flows driven by internal heating, the behaviour of the turbulence is far less constrained. 
In particular, the features of the flow when the nondimensional Rayleigh number $R$, is increased is far less known albeit for a selection of studies \citep{goluskin2012convection, Goluskin2015a,goluskin2016penetrative, Whitehead2011, Lu2004, Lepot2018, Miquel2019, bouillaut2022, Arslan2021, Arslan2023, Arslan2021a, kumar2021ihc}. Here, $R$ is the ratio of the destabilising thermal forcing to stabilising diffusive processes in the fluid. 


This work considers internally heated convection (IHC) between parallel plates with fixed thermal fluxes. Specifically, the lower plate is a thermal insulator, while the upper plate has a fixed flux boundary condition matching the total energy input due to internal heating. In the case of fixed flux RBC, the top plate remains colder than the lower plate for all $R$ and intuition would indicate the same holds for IHC. 
The mean conductive heat flux can be defined precisely as the difference between the mean temperatures of the lower and upper plates, namely
\begin{equation}
\dT := \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}},
\end{equation}
where  $\volav{\cdot}_h$ denotes a horizontal, $\volav{\cdot}$ a volume and overlines an infinite time average. 
While negative temperature gradients could occur locally, downwards conduction, defined as $\dT < 0$, would be unexpected.
However, for uniform IHC in the fixed flux boundary setup, it has been established that $\dT \geq - \frac{2\sqrt{3} - 3}{12} + 1.655 R^{-1/3} \approx - 0.03065 + 1.655 R^{-1/3}$, such that downwards conduction cannot be ruled out for all $R$ \citep{Arslan2021a}.  

Uniform IHC is one case of a wider ensemble of flows driven by non-uniform internal heating. In fact, on geophysical and astrophysical scales, the heating varies in space and time \citep{MantleConvectioninTerrestrialPlanets,tritton1975internally}. Following the results of \cite{Arslan2021a} the natural question becomes, can downwards conduction be eliminated when convection is driven by non-uniform heating profiles?  
As such, in contrast to \cite{Arslan2021a} the internal heating in this work is taken as an arbitrary function of the vertical coordinate.  

We prove rigorous lower bounds for the nondimensional mean conductive heat flux $\dT$. For the problem under consideration 
% the mean convective heat flux, $\wT$ is directly related to $\dT$, this relationship is exploited to 
we prove a bound by use of the \textit{background field method}. The method, introduced by \cite{Doering1994, Doering1996} and \cite{Constantin1995a}, produces bounds on mean quantities through the solution of a convex optimization problem and has demonstrated success in proving bounds for a wide range of flows \citep{Fantuzzi2022} including IHC, albeit with uniform heating  \citep{Lu2004,Whitehead2011,Whitehead2012,Goluskin2015a,Arslan2021a, Arslan2021,Arslan2023,kumar2021ihc}.


The main result of this paper is as follows. For a set of non-uniform heating distributions, we prove that,
\begin{equation}
    \label{eq:main_res}
    \dT \geq \mu + c R^{-1/3} ,
\end{equation}
where $\mu\leq0$ and $c>0$ are both functions of the choice of heating profile. The optimal $\mu$ is determined for a family of polynomial heating profiles, defined by a single parameter that quantifies the concentration of the heating at the lower boundary. This study demonstrates that the threshold of $R$ beyond which downwards conduction cannot be excluded increases, but remains finite, as the concentration of heating in the vicinity of the lower boundary intensifies. In the limit where all the heating occurs at the lower boundary, the problem is expected to be equivalent to RBC between fixed flux boundaries \citep{Otero2002}.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Whether driven by the boundaries, internal heat sources, or a mixture of both, thermal convection is ubiquitous to nature. The case of boundary-driven convection referred to as Rayleigh-B\'enard convection (RBC), has been extensively studied \citep{bodenschatz2000,chilla2012new,Ahlers2009}. 
% An open question in RBC is the ultimate scaling of the heat transport due to turbulent convection as the Rayleigh number, $R$, increases \citep{doering2020turning}. $R$ is a nondimensional number quantifying the ratio of destabilising thermal forcing to stabilising diffusive processes in a fluid. The same open questions exist for the far less studied flow of internally heated convection (IHC), albeit for select studies in the past decade \citep{goluskin2012convection,Goluskin2015a,goluskin2016penetrative,Whitehead2011,Lu2004,Lepot2018,Miquel2019,bouillaut2022,Arslan2021,Arslan2023,Arslan2021a,kumar2021ihc}. Beyond the scaling of heat transport with $R$, another open question is on the existence of `downwards conduction'; downwards conduction here refers to mean conductive heat transport from the top to the bottom. In particular, for uniform IHC between fixed flux boundary conditions, it is not possible to rule out downwards conduction for arbitrarily large $R$, from the governing equations  \citep{Arslan2021a}. 

% For IHC present on geophysical and astrophysical scales, the internal heating can vary in space and time \citep{MantleConvectioninTerrestrialPlanets,tritton1975internally}. 
% An extension of rigorous results for IHC to non-uniform heating distributions is therefore naturally of interest. 
% In contrast to previous studies \citep{Arslan2021a} the internal heating in this work is taken as an arbitrary function of the vertical coordinate. We prove a rigorous lower bounds for the nondimensional mean conductive heat flux $\dT$, where $\volav{\cdot}_h$ denotes a horizontal, $\volav{\cdot}$ a volume and overlines an infinite time average.
% Given a lower bound on $\dT$ the motivating question is if downwards conduction can be ruled out for non-uniform IHC. 
% % While choices of heating can be motivated either by physical processes or open mathematical problems, the results here reflect both.   

% In standard studies of turbulent convection, the emergent properties investigated are the mean convective heat transport $\wT$ and the mean temperature $\mean{T}$. For RBC the two quantities can be related \textit{a priori}, however, this is not possible for IHC \citep{Goluskin2016book}.
% Rigorous scaling bounds for $\mean{T}$ and later $\wT$ in IHC with uniform heating have been derived using the \emph{background method} \citep{Lu2004,Whitehead2011,Whitehead2012,Goluskin2015a,Arslan2021a, Arslan2021,Arslan2023,kumar2021ihc}. The method, popularized by \cite{Doering1994,Doering1996} and \cite{Constantin1995a}, produces bounds on mean quantities that are quadratic in the flow variables through the solution of a convex optimization problem.
% Proving bounds on $\mean{T}$ in IHC is a relatively simple extension from results for RBC, the quantity $\mean{wT}$ is far more difficult to bound. On the other hand, with fixed flux boundary conditions $\wT$ is directly linked to $\dT$.  

% The general result of this paper is as follows. For the set of non-uniform heating distributions that include uniform heating, we prove that,
% \begin{equation}
%     \dT \geq \mu + c R^{-1/3} ,
% \end{equation}
% where $\mu\leq0$ and $c>0$ are both functions of the heating profile. The optimal $\mu$ is determined for a family of polynomial heating profiles, defined by a single parameter that concentrates the heating to the lower boundary. The $R$ above which downwards conduction cannot be ruled out increases, but remains finite, as the heating concentrates to the lower boundary. At the limit where all the heating occurs at the lower boundary, the problem returns to the that of RBC between fixed flux boundaries \citep{Otero2002}.  

 
 


\section{Setup}
\label{sec:setup}

We consider a layer of fluid between two horizontal plates separated by a distance $d$ and periodic in the horizontal ($x$ and $y$) directions with periods $L_x$ and $L_y$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Gravity acts in the negative vertical direction $z$, and the fluid is heated internally at a volumetric rate $\Tilde{H}$.
The dimensional heating is written as $\Tilde{H}=H_0 H(z)$ with $H_0$ defined as $H_0 = \lVert H \rVert_1 $ and $H(z)$ is an arbitrary positive function of only $z$. Here and throughout the paper $\lVert f \rVert_p$ is the standard $L^p$ norm of a function $f=f(z)$.

To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2H_0/\kappa \rho c_p$ as the temperature scale \citep{roberts1967convection}. The velocity of the fluid $\boldsymbol{u}=(u,v,w)$ and temeprature $T$ in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ is then governed by the Boussinesq equations,
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
The non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa},
    \qquad\text{and}\qquad 
    R = \frac{g \alpha H_0 d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are taken to be no-slip and fixed flux:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:nu}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-\eta(1),
\end{gather}
\end{subequations} 
where we introduce a measure of the vertical energy flux $\eta(z) \in L^2(0,1)$ a non-decreasing function defined as,
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z)\, \textrm{d}z.
\end{equation}
Then, $\eta(1)$ sets the total energy flux out of the system. A diagram of the system is shown in \cref{fig:config}\textit{(a)}.



\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \draw[black,thick] (-6,0) -- (-2,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (-6,1.8) -- (-2,1.8) node [anchor = west] {$z=1$};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(2.86,1.8) (3.02,1.62) (3.1,1.5)};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(3.1,0.3) (3.16,0.18) (3.34,0)};
    \draw [dashed ,colorbar10] (2.5,1.8) -- (3.7,0);
    \draw [colorbar10] (3.1,1.5) -- (3.1,0.3);
    \node at (1.25,-0.25) {$ \partial_z T = -1 $};
    \node at (1.25,2.025) {$ \partial_z T = -1 $};
    \node at (-4.75,0.9) { $H(z)$ };
    \draw[->] (-7,0) -- (-7,0.36) node [anchor=east]{$z$};
    \draw[->] (-7,0) -- (-6.6,0) node [anchor=north]{$x$};
    \draw[->] (-7,0) -- (-6.64,0.2) node [anchor=west]{$y$};
    \draw[black,thick] (0,0) -- (4,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (0,1.8) -- (4,1.8) node [anchor = west] {$z=1$};
    \node at (-4.75,-0.25) {$ \partial_z T = 0 $};
    \node at (-4.75,2.025) {$  \partial_z T = -\eta(1) $};
    \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(-3.5,1.8) (-2.8,1.1) (-2.5,0)};
    \draw [colorbar10] plot [smooth,tension=1] coordinates {(-3.5,1.8) (-3.12,1.58) (-3,1.45)}; 
    \draw [colorbar10] (-3,1.45) -- (-3,0);
    \draw[->,colorbar10,thick] (2.5,0) -- (2.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (2.5,0) -- (2.9,0) node [anchor=north]{$T$};
   \draw[->,colorbar10,thick] (-3.5,0) -- (-3.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (-3.5,0) -- (-3.1,0) node [anchor=north]{$T$};
    \node at (-6.4,1.8) {\textit{(a)}};
    \node at (-0.4,1.8) {\textit{(b)}};
    \end{tikzpicture}
    \caption{\textit{(a)} IHC and \textit{(b)}  RBC with fixed flux boundaries, where $H(z)$ is a positive non-uniform heating profile. In both panels ({\color{colorbar10}\dashedrule}) denote the conductive temperature profiles and ({\color{colorbar10}\solidrule}) the mean temperature profiles in the turbulent regime. In panel \textit{(a)} the temperature profiles are for $H(z)=1$. }
    \label{fig:config}
\end{figure}


We can obtain an identity for the heat transport of the system by multiplying \eqref{eq:nondim_energy_nonUniform} by $z$ and taking an infinite time and volume average. Use of \eqref{eq:eta_general} and a standard application of integration by parts with the boundary conditions \eqref{bc:u_non_u} \& \eqref{bc:nu} gives the identity,
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \dT &= \int^{1}_{0}\eta(z)\,\textrm{d}z.
\end{align}
The left hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical convective heat flux, $\wT$, and the mean conductive heat flux.
% \begin{equation}
% \dT = \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}}.
% \end{equation}
Ruling out downwards conduction  equates to demonstrating that $\dT\geq0$ for all $R$.


Finally, to remove the inhomogeneous boundary conditions on $T$ it is convenient to rewrite the temperature field in terms of perturbations from the conductive profile $T_c$,
\begin{equation}
    \label{eq:T}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition it follows that $T'_c(z) = - \eta(z)$, where primes denote derivatives with respect to $z$. Then, \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ becomes,
\begin{gather}
    \label{eq:theta_eq}
     \partial_t \theta + \boldsymbol{u} \cdot \bnabla \theta = \bnabla^2 \theta + w\, \eta(z) ,\\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{gather}

\section{Bounding heat transport}

To investigate downwards conduction while retaining similarities with previous studies of IHC and RBC  \citep{Arslan2021a}, we search for an upper bound on $\wT$ and use \eqref{eq:energy_bal_nu} to bound $\dT$. First, we realise that $\wT = \mean{w\theta}$, since by incompressibilty and the boundary conditions \eqref{bc:u_non_u}, we have the property,
\begin{equation}
    \volav{w f(z)} = \int^{1}_0 \horav{w} f \textrm{d}z = 0,
\end{equation}
for arbitrary $f=f(z)$. In what follows the auxiliary functional method is used to prove an upper bound on $\mean{w\theta}$. 


\subsection{The auxiliary functional method}
\label{sec:afm}

Rigorous bounds on the mean quantities of turbulent flows can be found by using the background field method, formulated within the more general framework of the auxiliary functional method \citep{Chernyshenko2014a,Fantuzzi2022}. In particular, we consider the following quadratic auxiliary functional,
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},\theta\} = \volav{ \frac{a}{2\,Pr\,R} |\boldsymbol{u}|^2 + \frac{b}{2}\left|\theta  - \frac{\phi(z)}{b}\right|^2 },
\end{equation}
where $a$ and $b$ are non-negative scalars and $\phi(z)$ a function to be optimised over. As demonstrated by \cite{Chernyshenko2022} use of quadratic auxiliary functionals makes the method equivalent to the background field method where $a$ and $b$ are referred to as balance parameters and $\phi(z)/b$ is the background temperature field. With a slight abuse of notation we refer to $\phi(z)$ as the background field. Then, given that $\mathcal{V}\{\boldsymbol{u},\theta\}$ remains bounded in time along solutions of \eqref{eq:mom_eq} \& \eqref{eq:theta_eq} for any given initial $\boldsymbol{u}$ and $\theta$, the infinite time average of the time derivative of $\mathcal{V}$ is zero. Using this property we can write,
\begin{equation}
    \label{eq:AFM_statemen}
    \mean{w\theta} = U - \left( \overline{U - \volav{w\theta} - \frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\} } \right),
\end{equation}
from which we deduce that $\mean{w \theta} \leq U$ if the term in the bracket in \eqref{eq:AFM_statemen} is non-negative. For brevity the details are omitted but computations analogous to \cite{Arslan2021a}, show that the optimal bound provable is given by,
\begin{equation}
    \label{eq:U_bound}
    U = \int^{1}_{0}\frac{\phi'(z)^2}{4b}\textrm{d}z,
\end{equation}
provided that the following constraint, referred to as the \textit{spectral constraint}, holds,
\begin{equation}
    \label{eq:sk_non_uni}
     \frac{a}{R\,k^2} \lVert w''_{\boldsymbol{k}}(z) \rVert_2^2  + b k^2\lVert \theta_{\boldsymbol{k}}(z) \rVert_2^2  - \int^{1}_0 \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} (z)\theta^*_{\boldsymbol{k}}(z) \}  \textrm{d}z \geq 0. 
\end{equation}
The spectral constraint must hold for all nonzero $\boldsymbol{k}$ where the magnitude of the wavevector $\boldsymbol{k}^2 = k_x^2 + k_y^2$ arises by exploiting horizontal periodicity in Fourier space. The corresponding boundary conditions become,
\begin{gather}
    \label{bc:w_k}
    w_{\boldsymbol{k}}(0)= w_{\boldsymbol{k}}(1)= w_{\boldsymbol{k}}'(0)= w_{\boldsymbol{k}}'(1)=0,\\
    \label{bc:T_k}
     \theta_{\boldsymbol{k}}'(0) =  \theta_{\boldsymbol{k}}'(1) =0.
\end{gather}

% \subsection{Background temperature field}
\subsection{Ans\"atz}
\label{sec:ansatz}

An explicit bound is obtained by evaluating $U$ with three particular choices. These are
\begin{itemize}
    \item[1.] A relation between the balance parameters of,
\begin{equation}
    \label{eq:b_relation}
    b = \frac{a+1}{\lVert \eta \rVert_2}.
\end{equation}
    \item[2.] A choice of background temperature field of,
    \begin{equation}
	 \phi'= (a+1)
        \begin{dcases}
            \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta}, &  0\leq z \leq \delta, \\
           1 + \frac{ \eta(z)}{ \lVert \eta \rVert_2 },  &  \delta \leq z \leq 1-\delta,\\
            \left(1+ \frac{\eta(1-\delta)}{ \lVert \eta \rVert_2 }\right)\frac{(1-z)}{\delta},& 1-\delta \leq z \leq 1,
        \end{dcases}
        \label{eq:phi_prime}
    \end{equation}
    where $\delta\leq \frac12$ is the width of the boundary layers of $\phi'(z)$.
    \item[3.] Non-uniform heating functions where $\eta(z) \in L^2(0,1)$ is non-decreasing and $\eta(1) = 1$ such that
\begin{equation}
    \label{eq:eta_cond}
    \eta(z) \leq 1.
\end{equation}
\end{itemize}
These three choices come from three observations. The first is that if $\phi'(z) = a+1+b\eta(z)$, the spectral constraint in \eqref{eq:sk_non_uni} is immediately satisfied. The resultant $U$ can be optimised for $b$ to obtain the relation \eqref{eq:b_relation}. In other words, the relation between $a$ and $b$ of \eqref{eq:b_relation} is optimal in the limit of $R\rightarrow\infty$. For all $R<\infty$ we anticipate the deviation to not be of leading order. However, the choice of $\phi'(z) = a+1+b\eta(z)$, does not give a $R$ dependent bound, unless we permit $\phi'(z)$ to have boundary layers of widths $\delta$. The simplest such choice of $\phi'(z)$ being \eqref{eq:phi_prime}. Finally, to allow for a comparison of the results with uniform IHC, $H(z)$ is restricted such that \eqref{eq:eta_cond} holds.


\subsection{ Bound on mean conduction }
\label{sec:bound_dT}
Starting with the spectral constraint \eqref{eq:sk_non_uni},
given the choice \eqref{eq:phi_prime} of $\phi'(z)$, \eqref{eq:sk_non_uni} can be simplified to, 
\begin{equation}
    \label{eq:sk-cond_2}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{a+1}{\lVert \eta \rVert_2} \left( \int_0^\delta f_1 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z + \int_{1-\delta}^1 f_2 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \right)  \geq 0,
\end{equation}
where,
\begin{equation}
    f_1 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(\delta))\frac{z}{\delta}, \quad   f_2 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(1-\delta))\frac{1-z}{\delta}.
\end{equation}
However, since $\eta(z) \leq 1$ and $\delta\leq \tfrac12$ then,
\begin{equation}
    \label{eq:F_simp}
    f_1 \leq \lVert \eta \rVert_2 + 1 \quad \text{and} \quad f_2 \leq \lVert \eta \rVert_2 + 1.
\end{equation}
Next, given the boundary conditions on $w_{\boldsymbol{k}}$ from \eqref{bc:w_k}, use of the fundamental theorem of calculus and the Cauchy-Schwarz inequality gives,
% \begin{equation}
%     w'_{\boldsymbol{k}}(z) = \int^{z}_0 w_{\boldsymbol{k}}''(\xi) \textrm{d}\xi \leq \sqrt{z}\, \lVert w_{\boldsymbol{k}}'' \rVert_2,
% \end{equation}
% therefore 
\begin{equation}
\label{eq:w_estimate}
     w_{\boldsymbol{k}}(z) = \int^{z}_0 \int^{\xi}_0 w_{\boldsymbol{k}}''(\sigma) \textrm{d}\sigma \textrm{d}\xi \leq \int^{z}_0 \sqrt{\xi} \, \lVert w_{\boldsymbol{k}}'' \rVert_{2} \,\textrm{d}\xi  = \frac23 z^\frac32\, \lVert w_{\boldsymbol{k}}'' \rVert_2.
\end{equation}
Using \eqref{eq:w_estimate} and Cauchy-Schwarz we can estimate the sign-indefinite terms in \eqref{eq:sk-cond_2} to obtain
\begin{subequations}
\begin{gather}
    \int^{\delta}_0 f_1 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \leq \frac23 \int^{\delta}_0 f_1 \, z^{\frac32} \, \theta_{\boldsymbol{k}} \textrm{d}z \lVert w_{\boldsymbol{k}}'' \rVert_2 \leq \frac23 \left( \int^{\delta}_0 f_1^2 z^3 \textrm{d}z \right)^{\frac12} \lVert w_{\boldsymbol{k}}'' \rVert_2 \lVert \theta_{\boldsymbol{k}} \rVert_2 . 
     % \int^{1}_{1-\varepsilon} f_2 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \leq \frac23 \left( \int^{1}_{1-\varepsilon} f_2^2 z^3 \textrm{d}z \right)^{\frac12} \lVert \theta_{\boldsymbol{k}} \rVert_2 \lVert w''_{\boldsymbol{k}} \rVert_2 .
 \end{gather}
\end{subequations}
A similar inequality holds for the integral at the upper boundary. 
The spectral constraint \eqref{eq:sk-cond_2} after use of \eqref{eq:F_simp} can be written as a homogeneous quadratic form in $\lVert w_{\boldsymbol{k}}'' \rVert_2$ and $\lVert \theta_{\boldsymbol{k}}\rVert_2$ ,
\begin{equation}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{2(a+1)}{3 \lVert \eta \rVert_2} (1+\lVert \eta \rVert_2 ) \delta^2  \lVert w''_{\boldsymbol{k}} \rVert_2\lVert \theta_{\boldsymbol{k}} \rVert_2    \geq 0,
\end{equation}
which is non-negative when it has a nonpositive discriminant. Therefore the spectral constraint is satisfied if,
\begin{equation}
    \label{eq:sk_cond_ineq}
    \delta^4 \leq \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) (1+\lVert \eta \rVert_2)^2 R }.
\end{equation}
% An exact relations of the form $\delta = \delta(a,R)$ and $\varepsilon = \varepsilon(a,R)$ can be found after evaluating the integrals for a choice of heating profile $H(z)$.    

With the ans\"{a}tz made above, we substitute \eqref{eq:phi_prime} and \eqref{eq:b_relation} into the expression for the bound in \eqref{eq:U_bound}. Given $\eta(z) \leq 1$ the bound can be estimated as
\begin{align}
    U &=
    \frac{\delta(a+1)}{12 \lVert \eta \rVert_2}   \left(  \left( \lVert \eta \rVert_2 + \eta(\delta)\right)^2  + \left( \lVert \eta \rVert_2 + \eta(1-\delta) \right)^2 \right)  +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z\,\nonumber \\
    &  \leq 
    \frac{\delta (a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{6 \lVert \eta \rVert_2}  +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + 1 \right)^2 \textrm{d}z\, \nonumber \\
    &= \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{4 \lVert \eta \rVert_2}   -    \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{3 \lVert \eta \rVert_2}\delta .
    \label{eq:U_form_sub}
\end{align}
% The strategy to obtain a $R$ dependent bound is to determine, for a particular choice of $\eta$, the variation of $\delta$ and $\varepsilon$ with $R$ that satisfies the spectral constraint in \eqref{eq:sk_non_uni}. 
% In both \eqref{eq:U_form_sub} and \eqref{eq:sk_cond_ineq}, there is no benefit to be gained from taking $\delta \neq \varepsilon$, so that we make the simplification $\delta = \varepsilon$. This implies that
% \begin{equation}
%     \delta^4 =  \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) (1+\lVert \eta \rVert_2)^2 R },
%     \label{eq:delta_exac}
% \end{equation}
% is sufficient for the spectral constraint to be satisfied. 
By definition $a\geq0$ such that we can use the estimate that $(a+1)^m\geq1$ for all $m>0$. Then,
taking $\delta$ as large as possible in \eqref{eq:sk_cond_ineq} and substituting into \eqref{eq:U_form_sub} gives that,
\begin{equation}
    U \leq \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{4 \lVert \eta \rVert_2}   -  \frac{\left( \lVert \eta \rVert_2 + 1\right)^{3/2}}{ \sqrt{3} \,\lVert \eta \rVert_2^{3/4}} a^{1/4} R^{-1/4}.
\end{equation}
Solving $\partial_a U =0$ gives the optimising $a$,
\begin{equation}
    a^* = 3^{-2/3} \lVert \eta \rVert_2^{1/3} (\lVert \eta \rVert_2 + 1)^{-2/3} R^{-1/3}.
\end{equation}
Finally, substituting for $a$ and rearranging gives,
\begin{equation}
    \mean{w \theta} \leq \frac{(\lVert \eta \rVert_2 + 1)^2}{4 \lVert \eta \rVert_2} - \frac{3^{1/3}}{4} \frac{(\lVert \eta \rVert_2 + 1)^{4/3}}{\lVert \eta \rVert_2^{2/3}} R^{-1/3},
\end{equation}
such that by \eqref{eq:energy_bal_nu}, 
\begin{equation}
    \label{eq:dT_bound_simple}
    \dT \geq \lVert \eta \rVert_1 - \frac{(\lVert \eta \rVert_2 + 1)^2}{4 \lVert \eta \rVert_2} + \frac{3^{1/3}}{4} \frac{(\lVert \eta \rVert_2 + 1)^{4/3}}{\lVert \eta \rVert_2^{2/3}} R^{-1/3}.
\end{equation}
This completes the proof of \eqref{eq:main_res}. If it were to occur 
downward conduction ($\dT < 0$) is possible for all $R$ above some critical $R_c$. Setting \eqref{eq:dT_bound_simple} to zero and rearranging, we find,
% \begin{equation}
%     R_c = \frac{3(\lVert \eta \rVert_2+1)^4}{64 \lVert \eta \rVert_2^2 \left[\frac{(1+\lVert \eta \rVert_2)^2}{4\lVert \eta \rVert_2} - \volav{\eta}  \right]^3}. 
% \end{equation}
% \begin{equation}
%     R_c \leq \frac{3 \lVert \eta \rVert_2 (\lVert \eta \rVert_2+1)^4}{  (3\lVert \eta \rVert_2+1)^3(1-\lVert \eta \rVert_2)^3}. 
% \end{equation}
\begin{equation}
    R_c = \frac{3\lVert \eta \rVert_2 (\lVert \eta \rVert_2 + 1)^4}{\left((\lVert \eta \rVert_2 + 1)^2 - 4 \lVert \eta \rVert_2 \lVert \eta\rVert_1 \right)^3}\, .
    \label{eq:Rc_g}
\end{equation}
If $R_c=\infty$, the denominator of \eqref{eq:Rc_g} must be zero. For all non-decreasing $\eta(z)$ where $\eta(1)=1$ the estimate $\eta(z)\leq 1$ implies that the denominator is positive and therefore $R_c<\infty$, unless $\eta(z) = 1$. Therefore downwards conduction cannot be ruled out.
It is worth noting that the estimate $\eta(z)\leq 1$, is tighter for heating profiles where the heating is concentrated near the lower boundary. In fact, in the case of uniform heating, where $\eta=z$ the negative asymptote of \eqref{eq:dT_bound_simple} is suboptimal as compared to the result of \cite{Arslan2021a}, however the bound has the benefit of applying to all possible heating profiles where $\eta(1)=1$. 



\section{Example: polynomial heating}
\label{sec:polynom_heating}
For a specific choice of heating profile, a careful handling of the integrals in \eqref{eq:U_form_sub} can give a bound on $\dT$ with an optimal asymptote.
To illustrate an optimal bound on $\dT$ let us consider one family of polynomial heating profiles. For $n \in [0,\infty)$ let,
\begin{equation}   
    \label{eq:H-1}
    H(n,z) = (n+1)(1-z)^n,
\end{equation}
with corresponding internal heating flux,
\begin{equation}
    \label{eq:E-1}
    \eta(n,z) = 1 - (1-z)^{n+1}.
\end{equation}
For $n=0$ the heating is uniform in the domain. As $n$ increases the heating is further concentrated at the lower boundary. As $n\rightarrow\infty$ the heating approximates a Dirac delta at $z=0$. In this limit the flow is expected to be equivalent to RBC with fixed flux boundaries. 

\begin{figure}
    \centering
    \hspace{-1cm}
    \includegraphics[scale=0.9]{fig/non_uni1.eps}
    \caption{Plots of the heating profiles $H(z)$ given by \eqref{eq:H-1} and the corresponding $\eta(z)$ given by \eqref{eq:E-1} for $n=0$ ({\color{colorbar1}\solidrule}), $n=1$ ({\color{colorbar10}\solidrule}), $n=2$ ({\color{colorbar15}\solidrule}) and $n\in[3,100]$ ({\color{mygrey}\solidrule}). }
    \label{fig:enter-label}
\end{figure}

\subsection{Improved bounds}

The results of \cref{sec:bound_dT} apply to 
\eqref{eq:H-1}, however the asymptote of $\dT$ \eqref{eq:dT_bound_simple} for $n=0$ is suboptimal to previous research \citep{Arslan2021a}. An improvement is possible by using \eqref{eq:H-1} and more carefully estimating the expression of $U$ found in \eqref{eq:U_form_sub}.

For the sake of simplicity we will ignore the prefactors and higher order $\delta$ contributions by dropping terms of order $\delta^{n+2}$, indicated by the use of $\lesssim$. These terms do not contribute to $\mu$ but instead would change the value of the constant multiplying $R$ with no change to the scaling.
First we evaluate the integral in \eqref{eq:U_form_sub} from $[\delta,1-\delta]$. Instead of using $\eta(z)\leq 1$ to obtain a trivial integral, substitute \eqref{eq:E-1} and evaluate, to obtain,
\begin{multline}
    \int^{1-\delta}_\delta (\lVert \eta \rVert_2 + \eta(z))^2 \textrm{d}z \lesssim (\lVert \eta \rVert_2 +1)^2(1-2\delta) - \frac{2(\lVert \eta \rVert_2 + 1)}{n+2}(1-\delta)^{n+2} + \frac{1}{2n+3} .  
    \label{eq:int_fine}
\end{multline}
A Taylor expansion of the second term on the right-hand side of \eqref{eq:int_fine} gives a crucial negative contribution that did not appear in the previous section. Given that $\delta\leq 1/2$, then for all $n$,
\begin{align}
    (1-\delta)^{n+2} &= 1 - (n+2)\delta + \sum^{\infty}_{k=2}  \begin{pmatrix} n+2 \\ k \end{pmatrix} (-\delta)^{k} 
    \geq 1 - (n+2)\delta.
    \label{eq:est_bound}
\end{align}
Substituting \eqref{eq:int_fine} and \eqref{eq:est_bound} back into the first line of \eqref{eq:U_form_sub} and rearranging gives,
\begin{equation}
    U \lesssim   \frac{a+1}{4\lVert \eta \rVert_2} \left( (\lVert \eta \rVert_2 + 1)^2 - \frac{2(\lVert \eta \rVert_2+1)}{n+2} + \frac{1}{2n+3} \right) - \frac{\delta(a+1)(\lVert \eta \rVert_2+1)}{6 \lVert \eta \rVert_2 } (2\lVert \eta \rVert_2 - 1).
    \label{eq:u_f}
\end{equation}
It can be easily verified that for all $\eta(z)$ given by \eqref{eq:E-1} it holds that $\lVert \eta \rVert_2 \geq 1/2$, so that \eqref{eq:u_f} gives a bound that approaches a constant from below as $R$ increases.
% , such that a bound of the form $U \lesssim U_0  - U_1 R^{-1/3}$ holds, where $U_0 > 0$ and $U_1>0$. 
Then, the same steps as in \cref{sec:bound_dT} can be followed to obtain a bound on $\mean{w\theta}$ and then $\dT$. More precisely, this involves substituting for $\delta$ and finding the optimising $a$. Without optimising the prefactors of the $R$ scaling, this procedure gives,
\begin{equation}
    \mean{w\theta} \lesssim \frac{U_0}{\lVert \eta\rVert_2} - \frac{(\lVert \eta \rVert_2 + 1)^{2/3}}{U_0^{1/3} \lVert \eta \rVert_2^{2/3}}R^{-1/3} .
\end{equation}
where,
\begin{equation}
    U_0 = \frac{1}{4} \left( (\lVert \eta \rVert_2 + 1)^2 - \frac{2(\lVert \eta \rVert_2+1)}{n+2} + \frac{1}{2n+3} \right).
\end{equation}
By \eqref{eq:energy_bal_nu} our desired result is,
\begin{equation}
    \dT \gtrsim \lVert \eta\rVert_1 - \frac{U_0}{\lVert \eta\rVert_2} + \frac{(\lVert \eta \rVert_2 + 1)^{2/3}}{U_0^{1/3} \lVert \eta \rVert_2^{2/3}}R^{-1/3}.
\end{equation}
Finally, the critical $R$ for the heating profiles given by \eqref{eq:H-1} is,
\begin{equation}
    R_c = \frac{ \lVert \eta \rVert_2 (1+\lVert \eta \rVert_2 )^2 }{U_0 (U_0- \lVert \eta \rVert_2 \lVert \eta \rVert_1  )^3} \, .
    \label{eq:Rc_e1}
\end{equation}
Substituting $\eta(z)$ as given by \eqref{eq:E-1} into \eqref{eq:Rc_e1}, gives that $R_c\sim n^3$, for sufficiently large $n$. Crucially for $n=0$ the asymptote of $\dT$ is equivalent to that from \cite{Arslan2021a}. Furthermore, we anticipate the asymptote remains optimal within our bounding framework for all $n$. As a final point, in the limit of $n\rightarrow\infty$, we have $R_c \rightarrow\infty$, therefore it is not possible to rule out downwards conduction for all $R$, if any heating occurs within the domain. 


\subsection{Interpolating IHC and RBC}

The $H(z)$ in \eqref{eq:H-1} and choice of non-dimensionalisation does not allow us to pass to the limit of $n=\infty$. Nevertheless, as $n$ increases the flow goes from uniform IHC towards RBC with fixed flux boundary conditions (\cref{fig:config}). A proof that for any initial condition solutions of IHC recover that of RBC when $n=\infty$ is not known to us. We can however look at the $R$ at which the flow is linearly unstable as $n$ varies. If a non-uniform heating profile as given by \eqref{eq:H-1} is used, then by the same procedure as outlined in \cite{Goluskin2015a} \textit{mutatis mutandis}, the $R_L$ at which the flow is linearly unstable is,
\begin{equation}
    \label{eq:RL}
    R_L = \frac{1}{\int^{1}_0 \eta(z) P(z) \textrm{d}z } = \frac{720}{1- 60 \frac{n^2+5n+6}{(n+6)(n+5)(n+4)(n+3)(n+2)}} ,
\end{equation}
where $P(z)$ is a polynomial dependent on the velocity boundary conditions (see Appendix A \cite{Goluskin2015a}). In \eqref{eq:RL}, for no-slip boundaries when $n=0$ $R_L = 1440$, while in the limit of $n\rightarrow\infty$ $R_L \rightarrow 720$. Therefore \eqref{eq:RL} recovers the known values for linear instability of uniform IHC and RBC between fixed flux boundaries \citep{Goluskin2016book}.



\section{Discussion}

We proved lower bounds on the mean conductive heat transport $\dT$ for non-uniform IHC between parallel plates with fixed flux and no-slip boundary conditions. The lower bound of $\dT \geq \mu - c R^{-1/3}$, where $c>0$ and $\mu \leq 0$, implies that provided any heating occurs within the domain, the possibility of downwards conduction, defined as a mean negative temperature gradient ($\dT < 0$), cannot be dismissed for arbitrarily large $R$. For a class of polynomial heating profiles parameterised by $n$, measuring how concentrated the heating is to the lower boundary, we find the optimal $\mu$, within the background field method. The bounds agree with previous results for uniform IHC \citep{Arslan2021a}. As $n$ increases, $\mu\rightarrow0^{-}$ and the critical $R$ for linear stability approaches that of fixed flux RBC. 


There are several restrictions in the results presented here,  primarily on the choice of heating profile. We consider $H$ non-uniform only in the vertical direction $z$. In nature, IHC is driven by non-homogeneous heating in space and time. Furthermore, we restrict to positive $H(z)$, yet the results could be extended to heating and cooling profiles if we non-dimensionalise by setting $H_0 = \lVert H \rVert_p$, for any $p\geq2$. Such a relaxation would also alleviate the restriction that $\eta(1)=1$. Additionally, our choice of $H(z)$ contains uniform IHC, however from the constructions in the proof one cannot pass to the case of fixed flux RBC. One reason being the choice of non-dimensionalisation and definition of $R$. Therefore, it would be advantageous to establish a Rayleigh number that can interpolate between convection processes driven by both mechanisms.


The analysis presented here uses the background field method. A route of inquiry to determine the optimality of the result could be with the so-called \textit{optimal wall-to-wall transport} method. 
% approach has been applied to IHC to bound $\mean{T}$, but no results are known for $\wT$. 
An upper and lower bound could help further confirm or rule out the existence of downwards conduction for IHC. If the possibility of downwards conduction cannot be dismissed, it would be of interest to determine the velocity fields that maximize heat transport while exhibiting downwards conduction.


==> v4.tex <==
\section{Introduction}
\label{sec:intro}

Whether driven by the boundaries, internal heat sources, or a mixture of both, thermal convection is ubiquitous in nature. Convection of a fluid between a hot lower plate and cold upper plate, Rayleigh-B\'enard convection (RBC), has been well studied \citep{chilla2012new, Ahlers2009}. Of interest is an understanding of the effects of turbulent convection on the bulk quantities of the flow, such as the mean convective heat transport. For flows driven by internal heating, the behaviour of the turbulence is far less constrained. In particular, the features of the flow when the nondimensional Rayleigh number $R$, is increased is far less known albeit for a selection of studies \citep{goluskin2012convection, Goluskin2015a,goluskin2016penetrative, Whitehead2011, Lu2004, Lepot2018, Miquel2019, bouillaut2022, Arslan2021, Arslan2023, Arslan2021a, kumar2021ihc}. Here, $R$ is the ratio of the destabilising thermal forcing to stabilising diffusive processes in the fluid. 


This work considers internally heated convection (IHC) between parallel plates with fixed thermal fluxes. Specifically, the lower plate is a thermal insulator and the upper plate has a fixed flux boundary condition matching the total heat input due to internal heating. In the case of fixed flux RBC, the top plate remains colder than the lower plate for all $R$ and intuition would indicate the same holds for IHC. 
The nondimensional mean conductive heat flux can be defined as the difference between the mean temperatures of the lower and upper plates, namely
\begin{equation}
\dT := \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1}}},
\end{equation}
where  $\volav{\cdot}_h$ denotes a horizontal, $\volav{\cdot}$ a volume and overlines an infinite time average. While negative temperature gradients could occur locally, downwards conduction, defined as $\dT < 0$, would be unexpected. However, for uniform IHC in the fixed flux boundary setup, it has been established that $\dT \geq - \frac{2\sqrt{3} - 3}{12} + 1.655 R^{-1/3} \approx - 0.03065 + 1.655 R^{-1/3}$, such that downwards conduction has not yet been ruled out for all $R$ \citep{Arslan2021a}.  

Uniform IHC is one case of a wider ensemble of flows driven by non-uniform internal heating. In fact, on geophysical and astrophysical scales, the heating varies in space and time \citep{MantleConvectioninTerrestrialPlanets,tritton1975internally}. Following the results of \cite{Arslan2021a} the question becomes, can downwards conduction be eliminated when the heating is non-uniform? As such, the internal heating, in contrast to \cite{Arslan2021a}, is taken as an arbitrary function of the vertical coordinate.  

We prove rigorous lower bounds for the nondimensional mean conductive heat flux $\dT$. For the problem under consideration, we prove a bound by the use of the \textit{background field method}. The method, introduced by \cite{Doering1994, Doering1996} and \cite{Constantin1995a}, produces bounds on mean quantities through the solution of a convex optimization problem and has demonstrated success in proving bounds for a wide range of flows \citep{Fantuzzi2022} including IHC with uniform heating  \citep{Lu2004,Whitehead2011,Whitehead2012,Goluskin2015a,Arslan2021a, Arslan2021,Arslan2023,kumar2021ihc}.


The main result of this paper is as follows. For a set of non-uniform heating distributions, we prove that,
\begin{equation}
    \label{eq:main_res}
    \dT \geq \mu + c R^{-1/3} ,
\end{equation}
where $\mu\leq0$ and $c>0$ are both functions of the choice of heating profile. The optimal $\mu$ is determined for a family of polynomial heating profiles, defined by a single parameter that quantifies the concentration of the heating at the lower boundary. This study demonstrates that the threshold of $R$ beyond which downward conduction cannot be excluded increases, but remains finite, as the concentration of heating in the vicinity of the lower boundary intensifies. In the limit where all the heating occurs at the lower boundary, the problem is expected to be equivalent to RBC between fixed flux boundaries.  



\section{Setup}
\label{sec:setup}

We consider a layer of fluid between two horizontal plates separated by a distance $d$ and periodic in the horizontal ($x$ and $y$) directions with periods $L_x$ and $L_y$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Gravity acts in the negative vertical direction $z$, and the fluid is heated internally at a volumetric rate $\Tilde{H}$. The dimensional heating is written as $\Tilde{H}=H_0 H(z)$ with $H_0$ defined as $H_0 = \lVert H \rVert_1 $ and $H(z)$ is an arbitrary positive function of only $z$. Here and throughout the paper $\lVert f \rVert_p$ is the standard $L^p$ norm of a function $f=f(z)$.

To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2H_0/\kappa \rho c_p$ as the temperature scale \citep{roberts1967convection}. The velocity of the fluid $\boldsymbol{u}=(u,v,w)$ and temeprature $T$ in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ are then governed by the Boussinesq equations,
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
The non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa},
    \qquad\text{and}\qquad 
    R = \frac{g \alpha H_0 d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are taken to be no-slip and fixed flux:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:nu}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-\eta(1),
\end{gather}
\end{subequations} 
where we introduce a measure of the vertical heat flux $\eta(z) \in L^2(0,1)$ a non-decreasing function defined as,
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z)\, \textrm{d}z.
\end{equation}
Then, $\eta(1)$ sets the total heat flux out of the system. A diagram of the system is shown in \cref{fig:config}\textit{(a)}.



\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \draw[black,thick] (-6,0) -- (-2,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (-6,1.8) -- (-2,1.8) node [anchor = west] {$z=1$};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(2.86,1.8) (3.02,1.62) (3.1,1.5)};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(3.1,0.3) (3.16,0.18) (3.34,0)};
    \draw [dashed ,colorbar10] (2.5,1.8) -- (3.7,0);
    \draw [colorbar10] (3.1,1.5) -- (3.1,0.3);
    \node at (1.25,-0.25) {$ \partial_z T = -1 $};
    \node at (1.25,2.025) {$ \partial_z T = -1 $};
    \node at (-4.75,0.9) { $H(z)$ };
    \draw[->] (-7,0) -- (-7,0.36) node [anchor=east]{$z$};
    \draw[->] (-7,0) -- (-6.6,0) node [anchor=north]{$x$};
    \draw[->] (-7,0) -- (-6.64,0.2) node [anchor=west]{$y$};
    \draw[black,thick] (0,0) -- (4,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (0,1.8) -- (4,1.8) node [anchor = west] {$z=1$};
    \node at (-4.75,-0.25) {$ \partial_z T = 0 $};
    \node at (-4.75,2.025) {$  \partial_z T = -\eta(1) $};
    \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(-3.5,1.8) (-2.8,1.1) (-2.5,0)};
    \draw [colorbar10] plot [smooth,tension=1] coordinates {(-3.5,1.8) (-3.12,1.58) (-3,1.45)}; 
    \draw [colorbar10] (-3,1.45) -- (-3,0);
    \draw[->,colorbar10,thick] (2.5,0) -- (2.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (2.5,0) -- (2.9,0) node [anchor=north]{$T$};
   \draw[->,colorbar10,thick] (-3.5,0) -- (-3.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (-3.5,0) -- (-3.1,0) node [anchor=north]{$T$};
    \node at (-6.4,1.8) {\textit{(a)}};
    \node at (-0.4,1.8) {\textit{(b)}};
    \end{tikzpicture}
    \caption{\textit{(a)} IHC and \textit{(b)}  RBC with fixed flux boundaries, where $H(z)$ is a positive non-uniform heating profile. In both panels ({\color{colorbar10}\dashedrule}) denote the conductive temperature profiles and ({\color{colorbar10}\solidrule}) the mean temperature profiles in the turbulent regime. In panel \textit{(a)} the temperature profiles are for $H(z)=1$. }
    \label{fig:config}
\end{figure}


We can obtain an identity for the heat transport of the system by multiplying \eqref{eq:nondim_energy_nonUniform} by $z$ and taking an infinite time and volume average. Use of \eqref{eq:eta_general} and a standard application of integration by parts with the boundary conditions \eqref{bc:u_non_u} \& \eqref{bc:nu} gives the identity,
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \dT &= \int^{1}_{0}\eta(z)\,\textrm{d}z.
\end{align}
The left hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical convective heat flux, $\wT$, and the mean conductive heat flux. Ruling out downwards conduction  equates to demonstrating that $\dT\geq0$ for all $R$.


Finally, to remove the inhomogeneous boundary conditions on $T$ it is convenient to rewrite the temperature field in terms of perturbations from the conductive profile $T_c$,
\begin{equation}
    \label{eq:T}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition it follows that $T'_c(z) = - \eta(z)$, where primes denote derivatives with respect to $z$. Then, \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ becomes,
\begin{gather}
    \label{eq:theta_eq}
     \partial_t \theta + \boldsymbol{u} \cdot \bnabla \theta = \bnabla^2 \theta + w\, \eta(z) ,\\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{gather}

\section{Bounding heat transport}

To investigate downwards conduction while retaining similarities with previous studies of IHC and RBC  \citep{Arslan2021a}, we search for an upper bound on $\wT$ and use \eqref{eq:energy_bal_nu} to bound $\dT$. First, we realise that $\wT = \mean{w\theta}$, since by incompressibilty and the boundary conditions \eqref{bc:u_non_u} any function $f(z)$ depending only on $z$ satisfies
\begin{equation}
    \volav{w f(z)} = \int^{1}_0 \horav{w} f(z) \textrm{d}z = 0.
\end{equation}
In what follows the auxiliary functional method is used to prove an upper bound on $\mean{w\theta}$. 


\subsection{The auxiliary functional method}
\label{sec:afm}

Rigorous bounds on the mean quantities of turbulent flows can be found by using the background field method, formulated within the more general framework of the auxiliary functional method \citep{Chernyshenko2014a,Fantuzzi2022}. In particular, we consider the following quadratic auxiliary functional,
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},\theta\} = \volav{ \frac{a}{2\,Pr\,R} |\boldsymbol{u}|^2 + \frac{b}{2}\left|\theta  - \frac{\phi(z)}{b}\right|^2 },
\end{equation}
where $a$ and $b$ are non-negative scalars and $\phi(z)$ a function to be optimised over. As demonstrated by \cite{Chernyshenko2022} use of quadratic auxiliary functionals makes the method equivalent to the background field method where $a$ and $b$ are referred to as balance parameters and $\phi(z)/b$ is the background temperature field. With a slight abuse of notation we refer to $\phi(z)$ as the background field. Then, given that $\mathcal{V}\{\boldsymbol{u},\theta\}$ remains bounded in time along solutions of \eqref{eq:mom_eq} \& \eqref{eq:theta_eq} for any given initial $\boldsymbol{u}$ and $\theta$, the infinite time average of the time derivative of $\mathcal{V}$ is zero. Using this property we can write,
\begin{equation}
    \label{eq:AFM_statemen}
    \mean{w\theta} = U - \left( \overline{U - \volav{w\theta} - \frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\} } \right),
\end{equation}
from which we deduce that $\mean{w \theta} \leq U$ if the term in the bracket in \eqref{eq:AFM_statemen} is non-negative. For brevity the details are omitted but computations analogous to \cite{Arslan2021a}, show that the optimal bound provable is given by,
\begin{equation}
    \label{eq:U_bound}
    U = \int^{1}_{0}\frac{\phi'(z)^2}{4b}\textrm{d}z,
\end{equation}
provided that the following constraint, referred to as the \textit{spectral constraint}, holds,
\begin{equation}
    \label{eq:sk_non_uni}
     \frac{a}{R\,k^2} \lVert w''_{\boldsymbol{k}}(z) \rVert_2^2  + b k^2\lVert \theta_{\boldsymbol{k}}(z) \rVert_2^2  - \int^{1}_0 \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} (z)\theta^*_{\boldsymbol{k}}(z) \}  \textrm{d}z \geq 0. 
\end{equation}
The spectral constraint must hold for all nonzero wavevectors $\boldsymbol{k}=(k_x,k_y)$ with magnitude $k^2 = k_x^2 + k_y^2$, which arises by exploiting horizontal periodicity in Fourier space. The corresponding boundary conditions become,
\begin{gather}
    \label{bc:w_k}
    w_{\boldsymbol{k}}(0)= w_{\boldsymbol{k}}(1)= w_{\boldsymbol{k}}'(0)= w_{\boldsymbol{k}}'(1)=0,\\
    \label{bc:T_k}
     \theta_{\boldsymbol{k}}'(0) =  \theta_{\boldsymbol{k}}'(1) =0.
\end{gather}


\subsection{Ansatz}
\label{sec:ansatz}

An explicit bound is obtained by evaluating $U$ with three particular choices. These are
\begin{itemize}
    \item[1.] A relation between the balance parameters of,
\begin{equation}
    \label{eq:b_relation}
    b = \frac{a+1}{\lVert \eta \rVert_2}.
\end{equation}
    \item[2.] A choice of background temperature field of,
    \begin{equation}
	 \phi'= (a+1)
        \begin{dcases}
            \left(1+ \frac{\eta(\delta)}{ \lVert \eta \rVert_2 }\right) \frac{z}{\delta}, &  0\leq z \leq \delta, \\
           1 + \frac{ \eta(z)}{ \lVert \eta \rVert_2 },  &  \delta \leq z \leq 1-\delta,\\
            \left(1+ \frac{\eta(1-\delta)}{ \lVert \eta \rVert_2 }\right)\frac{(1-z)}{\delta},& 1-\delta \leq z \leq 1,
        \end{dcases}
        \label{eq:phi_prime}
    \end{equation}
    where $\delta\leq \frac12$ is the width of the boundary layers of $\phi'(z)$.
    \item[3.] Non-uniform heating functions where $\eta(z) \in L^2(0,1)$ is non-decreasing and $\eta(1) = 1$ such that
\begin{equation}
    \label{eq:eta_cond}
    \eta(z) \leq 1.
\end{equation}
\end{itemize}
These three choices come from three observations. The first is that if $\phi'(z) = a+1+b\eta(z)$, the spectral constraint in \eqref{eq:sk_non_uni} is immediately satisfied. The resultant $U$ can be optimised for $b$ to obtain the relation \eqref{eq:b_relation}. In other words, the relation between $a$ and $b$ of \eqref{eq:b_relation} is optimal in the limit of $R\rightarrow\infty$. For all $R<\infty$ we anticipate the deviation to not be of leading order. However, the choice of $\phi'(z) = a+1+b\eta(z)$, does not give a $R$ dependent bound, unless we permit $\phi'(z)$ to have boundary layers of widths $\delta$. The simplest such choice of $\phi'(z)$ being \eqref{eq:phi_prime}. Finally, to allow for a comparison of the results with uniform IHC, $H(z)$ is restricted such that \eqref{eq:eta_cond} holds.


\subsection{ Bound on mean conduction }
\label{sec:bound_dT}
Starting with the spectral constraint \eqref{eq:sk_non_uni},
given the choice \eqref{eq:phi_prime} of $\phi'(z)$, \eqref{eq:sk_non_uni} can be simplified to, 
\begin{equation}
    \label{eq:sk-cond_2}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{a+1}{\lVert \eta \rVert_2} \left( \int_0^\delta f_1 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z + \int_{1-\delta}^1 f_2 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \right)  \geq 0,
\end{equation}
where,
\begin{equation}
    f_1 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(\delta))\frac{z}{\delta}, \quad   f_2 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(1-\delta))\frac{1-z}{\delta}.
\end{equation}
However, since $\eta(z) \leq 1$ and $\delta\leq \tfrac12$ then,
\begin{equation}
    \label{eq:F_simp}
    f_1 \leq \lVert \eta \rVert_2 + 1, \quad \text{and} \quad f_2 \leq \lVert \eta \rVert_2 + 1.
\end{equation}
Next, given the boundary conditions on $w_{\boldsymbol{k}}$ from \eqref{bc:w_k}, use of the fundamental theorem of calculus and the Cauchy-Schwarz inequality gives,
\begin{equation}
\label{eq:w_estimate}
     w_{\boldsymbol{k}}(z) = \int^{z}_0 \int^{\xi}_0 w_{\boldsymbol{k}}''(\sigma) \textrm{d}\sigma \textrm{d}\xi \leq \int^{z}_0 \sqrt{\xi} \, \lVert w_{\boldsymbol{k}}'' \rVert_{2} \,\textrm{d}\xi  = \frac23 z^\frac32\, \lVert w_{\boldsymbol{k}}'' \rVert_2.
\end{equation}
Using \eqref{eq:w_estimate} and Cauchy-Schwarz we can estimate the sign-indefinite terms in \eqref{eq:sk-cond_2} to obtain
\begin{subequations}
\begin{gather}
    \int^{\delta}_0 f_1 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \leq \frac23 \int^{\delta}_0 f_1 \, z^{\frac32} \, \theta_{\boldsymbol{k}} \textrm{d}z \lVert w_{\boldsymbol{k}}'' \rVert_2 \leq \frac23 \left( \int^{\delta}_0 f_1^2 z^3 \textrm{d}z \right)^{\frac12} \lVert w_{\boldsymbol{k}}'' \rVert_2 \lVert \theta_{\boldsymbol{k}} \rVert_2 . 
 \end{gather}
\end{subequations}
A similar inequality holds for the integral at the upper boundary. 
The spectral constraint \eqref{eq:sk-cond_2} after use of \eqref{eq:F_simp} can be written as a homogeneous quadratic form in $\lVert w_{\boldsymbol{k}}'' \rVert_2$ and $\lVert \theta_{\boldsymbol{k}}\rVert_2$ ,
\begin{equation}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{2(a+1)}{3 \lVert \eta \rVert_2} (1+\lVert \eta \rVert_2 ) \delta^2  \lVert w''_{\boldsymbol{k}} \rVert_2\lVert \theta_{\boldsymbol{k}} \rVert_2    \geq 0,
\end{equation}
which is non-negative when it has a nonpositive discriminant. Therefore the spectral constraint is satisfied if,
\begin{equation}
    \label{eq:sk_cond_ineq}
    \delta^4 \leq \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) (1+\lVert \eta \rVert_2)^2 R }.
\end{equation}
    

\textbf{[Gio's edits]}
With nothing in the boundary layers, the bound becomes
\begin{align}
    U &=
    \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z
    \nonumber \\
    &= \frac{ a+1  }{4 \lVert \eta \rVert_2 } A(\eta)
    - \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int_{(0,\delta) \cup (1-\delta,1)} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z
    \\
    &\leq 
    \frac{ a+1  }{4 \lVert \eta \rVert_2 } A(\eta)
    - \frac{ a+1  }{4 \lVert \eta \rVert_2 }2  \lVert \eta \rVert_2 \delta
\end{align}
where
\begin{equation}
    A(\eta) = \int^{1}_{0} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z
\end{equation}

With the ans\"{a}tz made above, we substitute \eqref{eq:phi_prime} and \eqref{eq:b_relation} into the expression for the bound in \eqref{eq:U_bound}. Given $\eta(z) \leq 1$ the bound can be estimated as
\begin{align}
    U &=
    \frac{\delta(a+1)}{12 \lVert \eta \rVert_2}   \left(  \left( \lVert \eta \rVert_2 + \eta(\delta)\right)^2  + \left( \lVert \eta \rVert_2 + \eta(1-\delta) \right)^2 \right)  +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z\,\nonumber \\
    &  \leq 
    \frac{\delta (a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{6 \lVert \eta \rVert_2}  +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + 1 \right)^2 \textrm{d}z\, \nonumber \\
    &= \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{4 \lVert \eta \rVert_2}   -    \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{3 \lVert \eta \rVert_2}\delta .
    \label{eq:U_form_sub}
\end{align}
By definition $a\geq0$ such that we can use the estimate that $(a+1)^m\geq1$ for all $m>0$. Then,
taking $\delta$ as large as possible in \eqref{eq:sk_cond_ineq} and substituting into \eqref{eq:U_form_sub} gives that,
\begin{equation}
    U \leq \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{4 \lVert \eta \rVert_2}   -  \frac{\left( \lVert \eta \rVert_2 + 1\right)^{3/2}}{ \sqrt{3} \,\lVert \eta \rVert_2^{3/4}} a^{1/4} R^{-1/4}.
\end{equation}
Solving $\partial_a U =0$ gives the optimising $a$,
\begin{equation}
    a^* = 3^{-2/3} \lVert \eta \rVert_2^{1/3} (\lVert \eta \rVert_2 + 1)^{-2/3} R^{-1/3}.
\end{equation}
Finally, substituting for $a$ and rearranging gives,
\begin{equation}
    \mean{w \theta} \leq \frac{(\lVert \eta \rVert_2 + 1)^2}{4 \lVert \eta \rVert_2} - \frac{3^{1/3}}{4} \frac{(\lVert \eta \rVert_2 + 1)^{4/3}}{\lVert \eta \rVert_2^{2/3}} R^{-1/3},
\end{equation}
such that by \eqref{eq:energy_bal_nu}, 
\begin{equation}
    \label{eq:dT_bound_simple}
    \dT \geq \lVert \eta \rVert_1 - \frac{(\lVert \eta \rVert_2 + 1)^2}{4 \lVert \eta \rVert_2} + \frac{3^{1/3}}{4} \frac{(\lVert \eta \rVert_2 + 1)^{4/3}}{\lVert \eta \rVert_2^{2/3}} R^{-1/3}.
\end{equation}
This completes the proof of \eqref{eq:main_res}. If it were to occur 
downward conduction ($\dT < 0$) cannot be ruled out for all $R$ above some critical $R_c$. Setting \eqref{eq:dT_bound_simple} to zero and rearranging, we find,
\begin{equation}
    R_c = \frac{3\lVert \eta \rVert_2 (\lVert \eta \rVert_2 + 1)^4}{\left((\lVert \eta \rVert_2 + 1)^2 - 4 \lVert \eta \rVert_2 \lVert \eta\rVert_1 \right)^3}\, .
    \label{eq:Rc_g}
\end{equation}
If $R_c=\infty$, the denominator of \eqref{eq:Rc_g} must be zero. For all non-decreasing $\eta(z)$ where $\eta(1)=1$ the estimate $\eta(z)\leq 1$ implies that the denominator is positive and therefore $R_c<\infty$, unless $\eta(z) = 1$. Therefore downwards conduction cannot be ruled out. It is worth noting that the estimate $\eta(z)\leq 1$, is tighter for heating profiles where the heating is concentrated near the lower boundary. In fact, in the case of uniform heating, where $\eta=z$ the negative asymptote of \eqref{eq:dT_bound_simple} is suboptimal as compared to the result of \cite{Arslan2021a}, however the bound has the benefit of applying to all possible heating profiles where $\eta(1)=1$. 

\begin{figure}
    \centering
    \hspace{-1cm}
    \includegraphics[scale=0.9]{fig/RC.eps}
    \caption{Contour plot of $R_c$ as given in \eqref{eq:Rc_g}. The white solid line represents the class of polynomial heating profiles \eqref{eq:H-1}. The dashed white line denotes the valid region for $R_c$ due to the Cauchy-Schwarz inequality $\lVert\eta\rVert_1\leq\lVert\eta\rVert_2$. }
    \label{fig:enter-label}
\end{figure}

\section{Example: polynomial heating}
\label{sec:polynom_heating}
For a specific choice of heating profile, a careful handling of the integrals in \eqref{eq:U_form_sub} can give a bound on $\dT$ with an optimal asymptote. To illustrate an optimal bound on $\dT$ let us consider one family of polynomial heating profiles. For $n \in [0,\infty)$ let,
\begin{equation}   
    \label{eq:H-1}
    H(n,z) = (n+1)(1-z)^n,
\end{equation}
with corresponding internal heating flux,
\begin{equation}
    \label{eq:E-1}
    \eta(n,z) = 1 - (1-z)^{n+1}.
\end{equation}
For $n=0$ the heating is uniform in the domain. As $n$ increases the heating is further concentrated at the lower boundary. As $n\rightarrow\infty$ the heating approximates a Dirac delta at $z=0$. In this limit the flow is expected to be equivalent to RBC with fixed flux boundaries. 



\subsection{Improved bounds}

The results of \cref{sec:bound_dT} apply to 
\eqref{eq:H-1}, however the asymptote of $\dT$ \eqref{eq:dT_bound_simple} for $n=0$ is suboptimal to previous research \citep{Arslan2021a}. An improvement is possible by using \eqref{eq:H-1} and more carefully estimating the expression of $U$ found in \eqref{eq:U_form_sub}.

For the sake of simplicity we will ignore the prefactors and higher order $\delta$ contributions by dropping terms of order $\delta^{n+2}$, indicated by the use of $\lesssim$. These terms do not contribute to $\mu$ but instead would change the value of the constant multiplying $R$ with no change to the scaling. First we evaluate the integral in \eqref{eq:U_form_sub} from $[\delta,1-\delta]$. Instead of using $\eta(z)\leq 1$ to obtain a trivial integral, substitute \eqref{eq:E-1} and evaluate, to obtain,
\begin{multline}
    \int^{1-\delta}_\delta (\lVert \eta \rVert_2 + \eta(z))^2 \textrm{d}z \lesssim (\lVert \eta \rVert_2 +1)^2(1-2\delta) - \frac{2(\lVert \eta \rVert_2 + 1)}{n+2}(1-\delta)^{n+2} + \frac{1}{2n+3} .  
    \label{eq:int_fine}
\end{multline}
A Taylor expansion of the second term on the right-hand side of \eqref{eq:int_fine} gives a crucial negative contribution that did not appear in the previous section. Given that $\delta\leq \frac12$, then for all $n$,
\begin{align}
    (1-\delta)^{n+2} &= 1 - (n+2)\delta + \sum^{\infty}_{k=2}  \begin{pmatrix} n+2 \\ k \end{pmatrix} (-\delta)^{k} 
    \geq 1 - (n+2)\delta.
    \label{eq:est_bound}
\end{align}
Substituting \eqref{eq:int_fine} and \eqref{eq:est_bound} back into the first line of \eqref{eq:U_form_sub} and rearranging gives,
\begin{equation}
    U \lesssim   \frac{a+1}{4\lVert \eta \rVert_2} \left( (\lVert \eta \rVert_2 + 1)^2 - \frac{2(\lVert \eta \rVert_2+1)}{n+2} + \frac{1}{2n+3} \right) - \frac{\delta(a+1)(\lVert \eta \rVert_2+1)}{6 \lVert \eta \rVert_2 } (2\lVert \eta \rVert_2 - 1).
    \label{eq:u_f}
\end{equation}
It can be easily verified that for all $\eta(z)$ given by \eqref{eq:E-1} it holds that $\lVert \eta \rVert_2 \geq \frac12$, so that \eqref{eq:u_f} gives a bound that approaches a constant from below as $R$ increases. Then, the same steps as in \cref{sec:bound_dT}, substituting for $\delta$ and finding the optimising $a$, can be followed to obtain a bound on $\mean{w\theta}$ and then $\dT$. Without optimising the prefactors of the $R$ scaling, this procedure gives,
\begin{equation}
    \mean{w\theta} \lesssim \frac{U_0}{\lVert \eta\rVert_2} - \frac{(\lVert \eta \rVert_2 + 1)^{2/3}}{U_0^{1/3} \lVert \eta \rVert_2^{2/3}}R^{-1/3} .
\end{equation}
where,
\begin{equation}
    U_0 = \frac{1}{4} \left( (\lVert \eta \rVert_2 + 1)^2 - \frac{2(\lVert \eta \rVert_2+1)}{n+2} + \frac{1}{2n+3} \right).
\end{equation}
By \eqref{eq:energy_bal_nu} our desired result is,
\begin{equation}
    \dT \gtrsim \lVert \eta\rVert_1 - \frac{U_0}{\lVert \eta\rVert_2} + \frac{(\lVert \eta \rVert_2 + 1)^{2/3}}{U_0^{1/3} \lVert \eta \rVert_2^{2/3}}R^{-1/3}.
\end{equation}
Finally, the critical $R$ for the heating profiles given by \eqref{eq:H-1} becomes,
\begin{equation}
    R_c = f(n) \sim \frac{ \lVert \eta \rVert_2 (1+\lVert \eta \rVert_2 )^2 }{U_0 (U_0- \lVert \eta \rVert_2 \lVert \eta \rVert_1  )^3} \sim n^3 \, .
    \label{eq:Rc_e1}
\end{equation}
Where $\sim$ is used since the constants of the $R$ scaling were not optimised and where the final relation holds for sufficiently large $n$. Crucially for $n=0$ the asymptote of $\dT$ is equivalent to that from \cite{Arslan2021a}. Furthermore, we anticipate the asymptote remains optimal within our bounding framework for all $n$. As a final point, in the limit of $n\rightarrow\infty$, we have $R_c \rightarrow\infty$, therefore it is not possible to rule out downwards conduction for all $R$, if any heating occurs within the domain. 


\subsection{Interpolating IHC and RBC}

The $H(z)$ in \eqref{eq:H-1} and choice of non-dimensionalisation does not allow us to pass to the limit of $n=\infty$. Nevertheless, as $n$ increases the flow goes from uniform IHC towards RBC with fixed flux boundary conditions (\cref{fig:config}). A proof that for any initial condition solutions of IHC recover that of RBC when $n=\infty$ is not known to us. We can however look at the $R$ at which the flow is linearly unstable as $n$ varies. If a non-uniform heating profile as given by \eqref{eq:H-1} is used, then by the same procedure as outlined in \cite{Goluskin2015a} \textit{mutatis mutandis}, the $R_L$ at which the flow is linearly unstable is,
\begin{equation}
    \label{eq:RL}
    R_L = \frac{1}{\int^{1}_0 \eta(z) P(z) \textrm{d}z } = \frac{720}{1- 60 \frac{n^2+5n+6}{(n+6)(n+5)(n+4)(n+3)(n+2)}} ,
\end{equation}
where $P(z)$ is a polynomial dependent on the velocity boundary conditions (see Appendix A \cite{Goluskin2015a}). In \eqref{eq:RL}, for no-slip boundaries when $n=0$ $R_L = 1440$, while in the limit of $n\rightarrow\infty$ $R_L \rightarrow 720$. Therefore \eqref{eq:RL} recovers the known values for linear instability of uniform IHC and RBC between fixed flux boundaries \citep{Goluskin2016book}.



\section{Discussion}

We proved lower bounds on the mean conductive heat transport $\dT$ for non-uniform IHC between parallel plates with fixed flux and no-slip boundary conditions. The lower bound of $\dT \geq \mu - c R^{-1/3}$, where $c>0$ and $\mu \leq 0$, implies that provided any heating occurs within the domain, the possibility of downwards conduction, defined as a mean negative temperature gradient ($\dT < 0$), cannot be dismissed for arbitrarily large $R$. For a class of polynomial heating profiles parameterised by $n$, measuring how concentrated the heating is to the lower boundary, we find the optimal $\mu$ within the background field method. The bounds agree with previous results for uniform IHC \citep{Arslan2021a}. As $n$ increases, $\mu\rightarrow0^{-}$ and the critical $R$ for linear stability approaches that of fixed flux RBC. 


There are several restrictions in the results presented here,  primarily on the choice of heating profile. We consider $H$ non-uniform only in the vertical direction $z$. In nature, IHC is non-homogeneous in space and time. Furthermore, we restrict to positive $H(z)$, yet the results could be extended to positive and negative $H(z)$ if we non-dimensionalise by fixing $H_0 = \lVert H \rVert_p$, for any $p\geq2$. Such a relaxation would also alleviate the condition that $\eta(1)=1$. Additionally, our choice of $H(z)$ contains uniform IHC, however, from the constructions in the proof, one cannot pass to the case of fixed flux RBC. One reason is the choice and definition of $R$. Therefore, it would be advantageous to establish a Rayleigh number that can interpolate between convection processes driven by both mechanisms.


The analysis presented here uses the background field method. A route of inquiry to determine the optimality of the result could be with the so-called \textit{optimal wall-to-wall transport} method. An upper and lower bound could help further confirm or rule out the existence of downward conduction for IHC. If downwards conduction cannot be dismissed it would be insightful to determine the velocity fields that maximise heat transport while exhibiting this behaviour.


==> v5.tex <==
\section{Introduction}
\label{sec:intro}


This work considers internally heated convection (IHC) between parallel plates with fixed thermal fluxes. We assume that the lower plate is a thermal insulator while the upper plate has a fixed flux boundary condition matching the total heat input due to internal heating. Beyond a given Rayleigh number, $R$, the flow is expected to be unstable. For example, if heating is applied uniformly in the domain, instability occurs whenever $R > 1440$ \citep{Goluskin2015a}. In the unsteady regime, a key physical property of the flow is the mean temperature drop $\dT$ between the upper and lower plates. For the case of fixed-flux boundary conditions considered in this work, and in contrast to classical Rayleigh-B\'enard convection, $\dT$ is an emergent statistic of the unsteady flow \citep{Goluskin2016book}. We denote a volume average as $\volav{\cdot}$, subscript $h$ represents a horizontal average, and overlines are for infinite time averages.



The purpose of this paper is to understand the dependence of the temperature drop $\dT$ on both the Rayleigh number $R$ of the flow and on the geometric location of the internal heating. More specifically, we aim to provide rigorous scaling laws of the form,
\begin{equation}
    \label{eq:main_res}
    \dT := \overline{\horav{T|_{z=0}}} - \overline{\horav{T|_{z=1} }} \geq \mu + c R^{-\sigma}, 
\end{equation}
which hold for any solution to the governing equations, where $c$ and $\mu$ are constants depending only on the nature of the internal heating, and $\sigma$ is a scaling rate to be identified. In light of the relative lack of experimental and numerical data regarding internally heated flows, obtaining such rigorous scaling laws is important to future research.

Perhaps the most closely related flow for which a rigorous characterisation of the temperature drop is known is for the case of fixed-flux Rayleigh-B\'enard convection, shown schematically in \cref{fig:config}\textit{(b)}. Here, symmetric heating and cooling rates are prescribed at upper and lower boundaries, as opposed to internally, and the temperature drop satisfies the rigorous bound $\dT \geq cR^{-1/3}$ \citep{Otero2002}. The physical interpretation of this result is that the upper plate, where heat is extracted, must, on average, remain cooler than the lower one and that the provable gap between these two values decreases at a rate of $R^{-1/3}$, with an increasingly turbulent and homogenised flow as $R \rightarrow \infty$. Noting that the $R$ is a flux based Rayleigh number the provable decay rate of the lower bound on $\dT$, agrees with that predicted by some phenomenological theories, namely the so-called ultimate regime \citep{spiegel1963generalization,kraichnan1962}. The final state of turbulent Rayleigh-B\'enard continues to be studied numerically and in experiments \citep{Ahlers2009,chilla2012new,doering2020turning}, where the ultimate regime has somewhat controversially been observed at sufficiently high Rayleigh numbers \citep{doering2019b,ahlers2022prl}.


Much less is known for internally heated flows with fixed flux boundary conditions. The only rigorous result proven to date is for uniformly applied internal heating, and in this case, $\dT \geq -0.030605 + 1.655R^{-1/3}$ \citep{Arslan2021a}. While the asymptotic decay rate of this bound agrees with that observed for Rayleigh-B\'enard convection with fixed flux boundary conditions, the appearance of the negative constant -0.030605 is significant. It implies that for a sufficiently high Rayleigh number, one cannot rigorously rule out the case that $ \overline{\horav{T|_{z=1}}} > \overline{\horav{T|_{z=0}}} $. That is, although all heat is extracted from the upper boundary, the time-averaged, internally-heated flow could behave as an “inverse conductor” with the top plate hotter than the bottom one. It is surprising that one cannot rigorously predict the behaviour of such a simple physical property of internally heated flows, especially given that the associated result for Rayleigh-B\'enard convection is well-aligned with existing phenomenological theories.


In this paper, we address this gap in the literature by identifying a class of internally heated flow for which time-averaged inverse conduction (i.e., $ \overline{\horav{T|_{z=1}}} > \overline{\horav{T|_{z=0}}} $) can be definitively ruled out. To do this, we extend the mathematical approach of \cite{Arslan2021a} for uniformly heated flows to apply to the case in which heating is prescribed in an arbitrary vertical distribution. Naively, one would expect that an inverse conductor is less likely to occur and thus should be easier to rigorously prove if the internal heating is applied close to the lower boundary. Our investigations open the door to the study of the dynamics of turbulent convection for spatially varying heating or cooling. However, only the former appears in this work.   
The main result of our paper is to show that, for any Rayleigh number, there exists a class of internally heated flows for which, if heating is applied sufficiently close to the bottom boundary, time-averaged mean inverse conduction can be rigorously ruled out. 



\section{Setup}
\label{sec:setup}

We consider a layer of fluid between two horizontal plates separated by a distance $d$ and periodic in the horizontal ($x$ and $y$) directions with periods $L_x$ and $L_y$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Gravity acts in the negative vertical direction $z$, and the fluid is heated internally at a volumetric rate $\Tilde{H}$. The dimensional heating is written as $\Tilde{H}=H_0 H(z)$ with $H_0$ defined as $H_0 = \frac{1}{L_x L_y d}\int^{L_x}_0\int^{L_y}_0\int^{d}_0 |\Tilde{H}| \textrm{d}x \textrm{d}y\textrm{d}z$ and $ H(z)$ is a positive function such that $\lVert H(z) \rVert_1 = 1$. Here and throughout the paper $\lVert f \rVert_p$ is the standard $L^p$ norm of a function $f=f(z)$ where $z\in[0,1]$.

To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2H_0/\kappa \rho c_p$ as the temperature scale \citep{roberts1967convection}. The velocity of the fluid $\boldsymbol{u}=(u,v,w)$ and temeprature $T$ in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ are then governed by the Boussinesq equations,
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
The non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa},
    \qquad\text{and}\qquad 
    R = \frac{g \alpha H_0 d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are taken to be no-slip and fixed flux:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:nu}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-\eta(1),
\end{gather}
\end{subequations} 
where we introduce a measure of the vertical heat flux $\eta(z) \in L^2(0,1)$, a positive non-decreasing function defined as
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z)\, \textrm{d}z.
\end{equation}
Then, $\eta(1)$ sets the total heat flux out of the system. A diagram of the system is shown in \cref{fig:config}\textit{(a)}.



\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \draw[black,thick] (-6,0) -- (-2,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (-6,1.8) -- (-2,1.8) node [anchor = west] {$z=1$};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(2.86,1.8) (3.02,1.62) (3.1,1.5)};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(3.1,0.3) (3.16,0.18) (3.34,0)};
    \draw [dashed ,colorbar10] (2.5,1.8) -- (3.7,0);
    \draw [colorbar10] (3.1,1.5) -- (3.1,0.3);
    \node at (1.25,-0.25) {$ \partial_z T = -1 $};
    \node at (1.25,2.025) {$ \partial_z T = -1 $};
    \node at (-4.75,0.9) { $H(z)$ };
    \draw[->] (-7,0) -- (-7,0.36) node [anchor=east]{$z$};
    \draw[->] (-7,0) -- (-6.6,0) node [anchor=north]{$x$};
    \draw[->] (-7,0) -- (-6.64,0.2) node [anchor=west]{$y$};
    \draw[black,thick] (0,0) -- (4,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (0,1.8) -- (4,1.8) node [anchor = west] {$z=1$};
    \node at (-4.75,-0.25) {$ \partial_z T = 0 $};
    \node at (-4.75,2.025) {$  \partial_z T = -\eta(1) $};
    \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(-3.5,1.8) (-2.8,1.1) (-2.5,0)};
    \draw [colorbar10] plot [smooth,tension=1] coordinates {(-3.5,1.8) (-3.12,1.58) (-3,1.45)}; 
    \draw [colorbar10] (-3,1.45) -- (-3,0);
    \draw[->,colorbar10,thick] (2.5,0) -- (2.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (2.5,0) -- (2.9,0) node [anchor=north]{$T$};
   \draw[->,colorbar10,thick] (-3.5,0) -- (-3.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (-3.5,0) -- (-3.1,0) node [anchor=north]{$T$};
    \node at (-6.4,1.8) {\textit{(a)}};
    \node at (-0.4,1.8) {\textit{(b)}};
    \end{tikzpicture}
    \caption{\textit{(a)} IHC and \textit{(b)}  Rayleigh-B\'enard convection with fixed flux boundaries, where $H(z)$ is a positive non-uniform heating profile. In both panels ({\color{colorbar10}\dashedrule}) denote the conductive temperature profiles and ({\color{colorbar10}\solidrule}) the mean temperature profiles in the turbulent regime. In panel \textit{(a)} the temperature profiles are for $H(z)=1$. }
    \label{fig:config}
\end{figure}


We can obtain an identity for the mean vertical heat transport of the system by multiplying \eqref{eq:nondim_energy_nonUniform} by $z$ and taking an infinite-time and volume average. Use of \eqref{eq:eta_general} and a standard application of integration by parts with the boundary conditions \eqref{bc:u_non_u} \& \eqref{bc:nu} gives the identity,
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \dT &= \int^{1}_{0}\eta(z)\,\textrm{d}z.
\end{align}
The left hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical convective heat flux, $\wT$, and the mean conductive heat flux. Ruling out inverse conduction  equates to demonstrating that $\dT\geq0$ for all $R$.


Finally, to remove the inhomogeneous boundary conditions on $T$ it is convenient to rewrite the temperature field in terms of perturbations from the conductive profile $T_c$,
\begin{equation}
    \label{eq:T}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition it follows that $T'_c(z) = - \eta(z)$, where primes denote derivatives with respect to $z$. Then, \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ becomes,
\begin{gather}
    \label{eq:theta_eq}
     \partial_t \theta + \boldsymbol{u} \cdot \bnabla \theta = \bnabla^2 \theta + w\, \eta(z) ,\\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{gather}

\section{Bounding heat transport}

To investigate inverse conduction while retaining similarities with previous studies of IHC and Rayleigh-B\'enard convection  \citep{Arslan2021a}, we search for an upper bound on $\wT$ and use \eqref{eq:energy_bal_nu} to bound $\dT$. First, we realise that $\wT = \mean{w\theta}$, since by incompressibilty and the boundary conditions \eqref{bc:u_non_u} any function $f(z)$ satisfies
\begin{equation}
    \volav{w f(z)} = \int^{1}_0 \horav{w} f(z) \textrm{d}z = 0.
\end{equation}
In what follows the auxiliary functional method is used to prove an upper bound on $\mean{w\theta}$. 


\subsection{The auxiliary functional method}
\label{sec:afm}

Rigorous bounds on the mean quantities of turbulent flows can be found by using the background field method \citep{Doering1994, Doering1996,Constantin1995a}, formulated within the more general framework of the auxiliary functional method \citep{Chernyshenko2014a,Fantuzzi2022}. In particular, we consider the following quadratic auxiliary functional,
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},\theta\} = \volav{ \frac{a}{2\,Pr\,R} |\boldsymbol{u}|^2 + \frac{b}{2}\left|\theta  - \frac{\phi(z)}{b}\right|^2 },
\end{equation}
where $a$ and $b$ are non-negative scalars and $\phi(z)$ a function to be optimised over. As demonstrated by \cite{Chernyshenko2022} use of quadratic auxiliary functionals makes the method equivalent to the background field method where $a$ and $b$ are referred to as balance parameters and $\phi(z)/b$ is the background temperature field. With a slight abuse of notation we refer to $\phi(z)$ as the background field. Then, given that $\mathcal{V}\{\boldsymbol{u},\theta\}$ remains bounded in time along solutions of \eqref{eq:mom_eq} \& \eqref{eq:theta_eq} for any given initial $\boldsymbol{u}$ and $\theta$ where $\nabla\cdot \boldsymbol{u}=0$, the infinite-time average of the time derivative of $\mathcal{V}$ is zero. Using this property we can write,
\begin{equation}
    \label{eq:AFM_statemen}
    \mean{w\theta} = U - \left( \overline{U - \volav{w\theta} - \frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\} } \right),
\end{equation}
from which we deduce that $\mean{w \theta} \leq U$ if the functional $U - \volav{w\theta}-\frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\}\geq 0$ in \eqref{eq:AFM_statemen} is pointwise non-negative. See \cite{Arslan2023t} for a detailed discussion of the background field method as applied to IHC. For brevity the details are omitted but computations analogous to \cite{Arslan2021a} show that the optimal bound provable is given by,
\begin{equation}
    \label{eq:U_bound}
    U = \int^{1}_{0}\frac{\phi'(z)^2}{4b}\textrm{d}z,
\end{equation}
provided that the following constraint, referred to as the \textit{spectral constraint}, holds,
\begin{multline}
    \label{eq:sk_non_uni}
     \frac{a}{R\,k^2} \lVert w''_{\boldsymbol{k}}(z) \rVert_2^2 + \frac{2a}{R} \lVert w'_{\boldsymbol{k}}(z) \rVert_2^2 + \frac{ak^2}{R}\lVert w_{\boldsymbol{k}}(z) \rVert_2^2 + b \lVert \theta'_{\boldsymbol{k}}(z) \rVert_2^2  + b k^2\lVert \theta_{\boldsymbol{k}}(z) \rVert_2^2  \\ - \int^{1}_0 \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} (z)\theta^*_{\boldsymbol{k}}(z) \}  \textrm{d}z \geq 0. 
\end{multline}
The spectral constraint must hold for all nonzero wavevectors $\boldsymbol{k}=(k_x,k_y)$ with magnitude $k^2 = k_x^2 + k_y^2$, which arises by exploiting horizontal periodicity in Fourier space. The corresponding boundary conditions become,
\begin{subequations} 
\begin{gather}
    \label{bc:w_k}
    w_{\boldsymbol{k}}(0)= w_{\boldsymbol{k}}(1)= w_{\boldsymbol{k}}'(0)= w_{\boldsymbol{k}}'(1)=0,\\
    \label{bc:T_k}
     \theta_{\boldsymbol{k}}'(0) =  \theta_{\boldsymbol{k}}'(1) =0.
\end{gather}
\end{subequations}


\subsection{Ansatz}
\label{sec:ansatz}

An explicit bound is obtained by evaluating $U$ with two particular choices. These are
\begin{itemize}
    \item[1.] A relation between the balance parameters of,
\begin{equation}
    \label{eq:b_relation}
    b = \frac{a+1}{\lVert \eta \rVert_2}.
\end{equation}
    \item[2.] A choice of background temperature field of,
    \begin{equation}
	 \phi'(z) = \frac{(a+1)}{\lVert \eta \rVert_2}
        \begin{dcases}
            0, &  0\leq z \leq \delta, \\
            \eta(z) + \lVert \eta \rVert_2,  &  \delta \leq z \leq 1-\delta,\\
            0,& 1-\delta \leq z \leq 1,
        \end{dcases}
        \label{eq:phi_prime}
    \end{equation}
    where $\delta \leq \frac12$ is the width of the boundary layers of $\phi'(z)$.
    % \item[3.] Non-uniform heating functions where $\eta(z) \in L^2(0,1)$ is non-decreasing and $\eta(1) = 1$ such that
% \begin{equation}
%     \label{eq:eta_cond}
%     \eta(z) \leq 1.
% \end{equation}
\end{itemize}
These two choices come from two observations. The first is that if $\phi'(z) = a+1+b\eta(z)$, the spectral constraint in \eqref{eq:sk_non_uni} is immediately satisfied. The resultant $U$ can be optimised for $b$ to obtain the relation \eqref{eq:b_relation}. In other words, the relation between $a$ and $b$ of \eqref{eq:b_relation} is optimal in the limit of $R\rightarrow\infty$. For all $R<\infty$ we anticipate the deviation to not be of leading order. However, the choice of $\phi'(z) = a+1+b\eta(z)$, does not give a $R$ dependent bound, unless we permit $\phi'(z)$ to have boundary layers of widths $\delta$. The simplest such choice of $\phi'(z)$ being \eqref{eq:phi_prime}.
% Finally, to allow for a comparison of the results with uniform IHC, $H(z)$ is restricted such that \eqref{eq:eta_cond} holds.


\subsection{ Bound on mean conduction }
\label{sec:bound_dT}
Starting with \eqref{eq:sk_non_uni}, we drop the positive terms in $w'_{\boldsymbol{k}}$, $w_{\boldsymbol{k}}$ and $\theta'_{\boldsymbol{k}}$ to give a simplified condition for the spectral constraint to hold. Then, given the choice \eqref{eq:b_relation} and \eqref{eq:phi_prime}  for $b$ and $\phi'(z)$ respectively, \eqref{eq:sk_non_uni} is replaced with, 
\begin{equation}
    \label{eq:sk-cond_2}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{a+1}{\lVert \eta \rVert_2}  \int_{(0,\delta)\cup(1-\delta,1)} (\eta(z)+\lVert \eta \rVert_2) |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \geq 0.
\end{equation}
% where,
% \begin{equation}
%     f_1 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(\delta))\frac{z}{\delta}, \quad   f_2 = \lVert \eta \rVert_2 + \eta(z) - ( \lVert \eta \rVert_2 + \eta(1-\delta))\frac{1-z}{\delta}.
% \end{equation}
Since $\eta(z) \leq 1$ by the choice of normalisation and $\delta\leq \tfrac12$ then,
\begin{equation}
    \label{eq:F_simp}
   \eta(z)+\lVert \eta \rVert_2 \leq  1+\lVert \eta \rVert_2 .
\end{equation}
Next, given the boundary conditions on $w_{\boldsymbol{k}}$ from \eqref{bc:w_k}, use of the fundamental theorem of calculus and the Cauchy-Schwarz inequality gives,
\begin{equation}
\label{eq:w_estimate}
     w_{\boldsymbol{k}}(z) = \int^{z}_0 \int^{\xi}_0 w_{\boldsymbol{k}}''(\sigma) \textrm{d}\sigma \textrm{d}\xi \leq \int^{z}_0 \sqrt{\xi} \, \lVert w_{\boldsymbol{k}}'' \rVert_{2} \,\textrm{d}\xi  = \frac23 z^\frac32\, \lVert w_{\boldsymbol{k}}'' \rVert_2.
\end{equation}
Using \eqref{eq:w_estimate} and Cauchy-Schwarz we can estimate the sign-indefinite terms in \eqref{eq:sk-cond_2} to obtain
\begin{align}
     \int_{(0,\delta)\cup(1-\delta,1)} (1+\lVert \eta \rVert_2) |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \nonumber &= 2\int^{\delta}_0 (1+\lVert \eta \rVert_2) |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \nonumber \\ &\leq \frac43 \int^{\delta}_0 (1+\lVert \eta \rVert_2) \, z^{\frac32} \, \theta_{\boldsymbol{k}} \textrm{d}z  \lVert w_{\boldsymbol{k}}'' \rVert_2  \nonumber \\
    &\leq \frac43 \left( \int^{\delta}_0 (1+\lVert \eta \rVert_2)^2 z^3 \textrm{d}z \right)^{\frac12} \lVert w_{\boldsymbol{k}}'' \rVert_2 \lVert \theta_{\boldsymbol{k}} \rVert_2\nonumber\\ &=\frac23 (1+\lVert \eta \rVert_2)\delta^2 \lVert w_{\boldsymbol{k}}'' \rVert_2 \lVert \theta_{\boldsymbol{k}} \rVert_2  . 
    \label{eq:wt_est}
 \end{align}
The simplified spectral constraint \eqref{eq:sk-cond_2} after use of \eqref{eq:F_simp} and \eqref{eq:wt_est} can be written as a homogeneous quadratic form in $\lVert w_{\boldsymbol{k}}'' \rVert_2$ and $\lVert \theta_{\boldsymbol{k}}\rVert_2$,
\begin{equation}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{2(a+1)}{3 \lVert \eta \rVert_2} (1+\lVert \eta \rVert_2 ) \delta^2  \lVert w''_{\boldsymbol{k}} \rVert_2\lVert \theta_{\boldsymbol{k}} \rVert_2    \geq 0,
\end{equation}
which is non-negative when it has a nonpositive discriminant. Therefore the spectral constraint is satisfied if,
\begin{equation}
    \label{eq:sk_cond_ineq}
    \delta^4 \leq \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) (1+\lVert \eta \rVert_2)^2 R }.
\end{equation}
    

With the ans\"{a}tze made above, we substitute \eqref{eq:b_relation} and \eqref{eq:phi_prime} into the expression for the bound in \eqref{eq:U_bound}. Making use of the fact that $\eta(z)$ is positive gives after rearranging,  
\begin{align}
    U &=
    \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z
    \nonumber \\
    &= \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1}_{0}\left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z 
    - \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int_{(0,\delta) \cup (1-\delta,1)} \left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z
    \nonumber \\
    &\leq 
   \frac12 (a+1)  \left( \lVert \eta \rVert_2 + \lVert \eta \rVert_1 -  \lVert \eta \rVert_2 \delta \right).
     \label{eq:U_form_sub}
\end{align}
% where
% \begin{equation}
%     A(\eta) = \int^{1}_{0} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z = 2\lVert \eta \rVert_2(\lVert \eta \rVert_2 +\lVert\eta\rVert_1)
% \end{equation}
% With the ans\"{a}tze made above, we substitute \eqref{eq:phi_prime} and \eqref{eq:b_relation} into the expression for the bound in \eqref{eq:U_bound}. Given $\eta(z) \leq 1$ the bound can be estimated as
% \begin{align}
%     U &=
%     \frac{\delta(a+1)}{12 \lVert \eta \rVert_2}   \left(  \left( \lVert \eta \rVert_2 + \eta(\delta)\right)^2  + \left( \lVert \eta \rVert_2 + \eta(1-\delta) \right)^2 \right)  +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + \eta(z) \right)^2 \textrm{d}z\,\nonumber \\
%     &  \leq 
%     \frac{\delta (a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{6 \lVert \eta \rVert_2}  +  \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left( \lVert \eta \rVert_2 + 1 \right)^2 \textrm{d}z\, \nonumber \\
%     &= \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{4 \lVert \eta \rVert_2}   -    \frac{(a+1)\left( \lVert \eta \rVert_2 + 1\right)^2}{3 \lVert \eta \rVert_2}\delta .
%     \label{eq:U_form_sub}
% \end{align}
By definition $a\geq0$ such that we can use the estimate that $(a+1)^m\geq1$ for all $m>0$. Then,
taking $\delta$ as large as possible in \eqref{eq:sk_cond_ineq} and substituting into \eqref{eq:U_form_sub} gives that,
\begin{align}
    U &\leq   \frac12 (a+1)  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1) 
    - \frac{\sqrt{3}}{2} \frac{\lVert\eta\rVert_2^{5/4}}{(1+\lVert\eta\rVert_2)^{1/2}}(a+1)^{3/4} a^{1/4} R^{-1/4}  \nonumber\\
    &\leq   \frac12 (a+1)  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1) 
    - \frac{\sqrt{3}}{2} \frac{\lVert\eta\rVert_2^{5/4}}{(1+\lVert\eta\rVert_2)^{1/2}} a^{1/4} R^{-1/4} .
    \label{eq:U_delt_sub}
\end{align}
After $U$ is taken as large as possible in \cref{eq:U_delt_sub}, the $a$ optimising the resulting expression can be found by solving $\partial_a U =0$, which gives,
\begin{equation}
    a^* =  \frac{a_0 \lVert \eta \rVert_2^{5/3}}{ (\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{4/3} (1+\lVert \eta \rVert_2 )^{2/3}} R^{-1/3},
\end{equation}
where $a_0 = \left(9/256\right)^{1/3}$.
Finally, substituting for $a$ and rearranging gives,
\begin{equation}
    \mean{w \theta} \leq  \frac12  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1)  -  \frac{a_1 \lVert \eta \rVert_2^{5/3}}{(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{1/3}(1+\lVert \eta \rVert_2)^{2/3} } R^{-1/3},
\end{equation}
where $a_1 = \tfrac12 a_0^{1/4}(\sqrt{3}-a_0^{3/4}) $,
then by \eqref{eq:energy_bal_nu}, 
\begin{equation}
    \label{eq:dT_bound_simple}
    \dT \geq   \frac12  ( \lVert \eta \rVert_1 - \lVert \eta \rVert_2)  +  \frac{a_1 \lVert \eta \rVert_2^{5/3}}{(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{1/3}(1+\lVert \eta \rVert_2)^{2/3} } R^{-1/3}.
\end{equation}
This completes the proof of \eqref{eq:main_res}. If it were to occur 
downward conduction ($\dT < 0$) cannot be ruled out for all $R$ above some critical $R_c$. Setting \eqref{eq:dT_bound_simple} to zero and rearranging, we find,
\begin{equation}
    R_c = \frac{8a_1^3 \lVert \eta \rVert_2^5 }{(1+\lVert \eta \rVert_2)^2(\lVert \eta \rVert_2 - \lVert \eta \rVert_1)^2(\lVert \eta \rVert_2^2 - \lVert \eta \rVert_1^2)}\, .
    \label{eq:Rc_g}
\end{equation}
If $R_c=\infty$, the denominator of \eqref{eq:Rc_g} must be zero. For all $\eta(z)$, by construction, we have $0\leq\eta(z)\leq 1$ such that
\begin{equation}
    \lVert \eta \rVert_2^2 = \lVert \eta^2 \rVert_1 \leq \lVert \eta \rVert_1, 
\end{equation}
which gives an upper bound on $\lVert \eta \rVert_2$. Along with the Cauchy-Schwarz inequality we have that
\begin{equation}
    \lVert \eta \rVert_1 \leq \lVert \eta \rVert_2 \leq \lVert \eta\rVert_1^{1/2}.
    \label{eq:eta_L2_bounds}
\end{equation}
A consequence of the bounds in \eqref{eq:eta_L2_bounds} is that the denominator in \eqref{eq:Rc_g} remains positive and therefore $R_c<\infty$, unless $\lVert \eta\rVert_1 = \lVert \eta \rVert_2$. This implies that inverse conduction cannot be ruled out for all heating profiles and only for those for which $\lVert \eta \rVert_1 =\lVert \eta\rVert_2$, an example of which would be if all the heating were localised to a single point, like the lower boundary, in which case the flow would be analogous to Rayleigh-B\'enard convection between fixed flux boundaries. 

\subsection{Example heating profiles}

To validate the main results from the previous subsection we can consider the case of uniform heating. For uniform heating $H(z)=1$ and by \eqref{eq:eta_general} $\eta=z$ such that \eqref{eq:dT_bound_simple} gives $\dT \geq -0.030605 + 0.1850 R^{-1/3}$. The results matches the scaling and asymptote of \cite{Arslan2021a}. The difference in the constant multiplying the $R$ scaling is due to the difference in choice of background profile $\phi'(z)$. The numerical optimisation carried out in \cite{Arslan2021a} demonstrated that the optimal bound, for uniform heating, was obtained with background fields that are linear in $z$ within the boundary layers. 

The results \eqref{eq:dT_bound_simple} and \eqref{eq:Rc_g} apply to all heating profiles that fit the definition of $\eta(z)$ and choice of non-dimensionalisation. To illustrate the results a selection of non-uniform heating profiles are plotted in \cref{fig:main_res} where the heating is near the bottom boundary \textit{(d)}, the heating is near the upper boundary \textit{(e)} and where the heating is sinusoidal \textit{(f)}, with the corresponding $R_c$ highlighted in \cref{fig:main_res} \textit{(a)}. The contour plot of \cref{fig:main_res} \textit{(a)} also highlights the bounds on $\lVert \eta\rVert_2$  shown in \eqref{eq:eta_L2_bounds}.  

\begin{figure}
    \centering
    \hspace{-1cm}
    \includegraphics[scale=1]{fig/myVectorFile.eps}
     \begin{tikzpicture}[overlay]
        \node at (-12,8.4) {\textit{(a)}};
       \node at (-4.5,6.7) {\textit{(b)}};
        \node at (-12,2.7) {\textit{(c)}};
        \node at (-8.8,2.7) {\textit{(d)}};
       \node at (-5.9,2.7) {\textit{(e)}};
       \node at (-3,2.7) {\textit{(f)}};
    \end{tikzpicture}
    \caption{\textit{(a)} Contour plot of $R_c$ as given in \eqref{eq:Rc_g} with the inset \textit{(b)} highlighting a region where $\lVert \eta\rVert_1 \sim \lVert \eta \rVert_2$, for no special reason the region chosen is $[0.925,1]\times[0.95,1]$. In panel \textit{(a)} the green cross (\mycross{matlabgreen}) highlights uniform heating, drawn in \textit{(c)}, the blue cross (\mycross{matlabblue}) highlights heating near the lower boundary drawn in \textit{(d)}, the yellow cross (\mycross{matlabyellow}) highlights heating near the upper boundary \textit{(e)} and the black cross (\mycross{black}) highlights sinusoidal heating, panel \textit{(f)}. }
    \label{fig:main_res}
\end{figure}

% \section{Example: polynomial heating}
% \label{sec:polynom_heating}
% For a specific choice of heating profile, a careful handling of the integrals in \eqref{eq:U_form_sub} can give a bound on $\dT$ with an optimal asymptote. To illustrate an optimal bound on $\dT$ let us consider one family of polynomial heating profiles. For $n \in [0,\infty)$ let,
% \begin{equation}   
%     \label{eq:H-1}
%     H(n,z) = (n+1)(1-z)^n,
% \end{equation}
% with corresponding internal heating flux,
% \begin{equation}
%     \label{eq:E-1}
%     \eta(n,z) = 1 - (1-z)^{n+1}.
% \end{equation}
% For $n=0$ the heating is uniform in the domain. As $n$ increases the heating is further concentrated at the lower boundary. As $n\rightarrow\infty$ the heating approximates a Dirac delta at $z=0$. In this limit the flow is expected to be equivalent to RBC with fixed flux boundaries. 



% \subsection{Improved bounds}

% The results of \cref{sec:bound_dT} apply to 
% \eqref{eq:H-1}, however the asymptote of $\dT$ \eqref{eq:dT_bound_simple} for $n=0$ is suboptimal to previous research \citep{Arslan2021a}. An improvement is possible by using \eqref{eq:H-1} and more carefully estimating the expression of $U$ found in \eqref{eq:U_form_sub}.

% For the sake of simplicity we will ignore the prefactors and higher order $\delta$ contributions by dropping terms of order $\delta^{n+2}$, indicated by the use of $\lesssim$. These terms do not contribute to $\mu$ but instead would change the value of the constant multiplying $R$ with no change to the scaling. First we evaluate the integral in \eqref{eq:U_form_sub} from $[\delta,1-\delta]$. Instead of using $\eta(z)\leq 1$ to obtain a trivial integral, substitute \eqref{eq:E-1} and evaluate, to obtain,
% \begin{multline}
%     \int^{1-\delta}_\delta (\lVert \eta \rVert_2 + \eta(z))^2 \textrm{d}z \lesssim (\lVert \eta \rVert_2 +1)^2(1-2\delta) - \frac{2(\lVert \eta \rVert_2 + 1)}{n+2}(1-\delta)^{n+2} + \frac{1}{2n+3} .  
%     \label{eq:int_fine}
% \end{multline}
% A Taylor expansion of the second term on the right-hand side of \eqref{eq:int_fine} gives a crucial negative contribution that did not appear in the previous section. Given that $\delta\leq \frac12$, then for all $n$,
% \begin{align}
%     (1-\delta)^{n+2} &= 1 - (n+2)\delta + \sum^{\infty}_{k=2}  \begin{pmatrix} n+2 \\ k \end{pmatrix} (-\delta)^{k} 
%     \geq 1 - (n+2)\delta.
%     \label{eq:est_bound}
% \end{align}
% Substituting \eqref{eq:int_fine} and \eqref{eq:est_bound} back into the first line of \eqref{eq:U_form_sub} and rearranging gives,
% \begin{equation}
%     U \lesssim   \frac{a+1}{4\lVert \eta \rVert_2} \left( (\lVert \eta \rVert_2 + 1)^2 - \frac{2(\lVert \eta \rVert_2+1)}{n+2} + \frac{1}{2n+3} \right) - \frac{\delta(a+1)(\lVert \eta \rVert_2+1)}{6 \lVert \eta \rVert_2 } (2\lVert \eta \rVert_2 - 1).
%     \label{eq:u_f}
% \end{equation}
% It can be easily verified that for all $\eta(z)$ given by \eqref{eq:E-1} it holds that $\lVert \eta \rVert_2 \geq \frac12$, so that \eqref{eq:u_f} gives a bound that approaches a constant from below as $R$ increases. Then, the same steps as in \cref{sec:bound_dT}, substituting for $\delta$ and finding the optimising $a$, can be followed to obtain a bound on $\mean{w\theta}$ and then $\dT$. Without optimising the prefactors of the $R$ scaling, this procedure gives,
% \begin{equation}
%     \mean{w\theta} \lesssim \frac{U_0}{\lVert \eta\rVert_2} - \frac{(\lVert \eta \rVert_2 + 1)^{2/3}}{U_0^{1/3} \lVert \eta \rVert_2^{2/3}}R^{-1/3} .
% \end{equation}
% where,
% \begin{equation}
%     U_0 = \frac{1}{4} \left( (\lVert \eta \rVert_2 + 1)^2 - \frac{2(\lVert \eta \rVert_2+1)}{n+2} + \frac{1}{2n+3} \right).
% \end{equation}
% By \eqref{eq:energy_bal_nu} our desired result is,
% \begin{equation}
%     \dT \gtrsim \lVert \eta\rVert_1 - \frac{U_0}{\lVert \eta\rVert_2} + \frac{(\lVert \eta \rVert_2 + 1)^{2/3}}{U_0^{1/3} \lVert \eta \rVert_2^{2/3}}R^{-1/3}.
% \end{equation}
% Finally, the critical $R$ for the heating profiles given by \eqref{eq:H-1} becomes,
% \begin{equation}
%     R_c = f(n) \sim \frac{ \lVert \eta \rVert_2 (1+\lVert \eta \rVert_2 )^2 }{U_0 (U_0- \lVert \eta \rVert_2 \lVert \eta \rVert_1  )^3} \sim n^3 \, .
%     \label{eq:Rc_e1}
% \end{equation}
% Where $\sim$ is used since the constants of the $R$ scaling were not optimised and where the final relation holds for sufficiently large $n$. Crucially for $n=0$ the asymptote of $\dT$ is equivalent to that from \cite{Arslan2021a}. Furthermore, we anticipate the asymptote remains optimal within our bounding framework for all $n$. As a final point, in the limit of $n\rightarrow\infty$, we have $R_c \rightarrow\infty$, therefore it is not possible to rule out downwards conduction for all $R$, if any heating occurs within the domain. 


% \subsection{Interpolating IHC and RBC}

% The $H(z)$ in \eqref{eq:H-1} and choice of non-dimensionalisation does not allow us to pass to the limit of $n=\infty$. Nevertheless, as $n$ increases the flow goes from uniform IHC towards RBC with fixed flux boundary conditions (\cref{fig:config}). A proof that for any initial condition solutions of IHC recover that of RBC when $n=\infty$ is not known to us. We can however look at the $R$ at which the flow is linearly unstable as $n$ varies. If a non-uniform heating profile as given by \eqref{eq:H-1} is used, then by the same procedure as outlined in \cite{Goluskin2015a} \textit{mutatis mutandis}, the $R_L$ at which the flow is linearly unstable is,
% \begin{equation}
%     \label{eq:RL}
%     R_L = \frac{1}{\int^{1}_0 \eta(z) P(z) \textrm{d}z } = \frac{720}{1- 60 \frac{n^2+5n+6}{(n+6)(n+5)(n+4)(n+3)(n+2)}} ,
% \end{equation}
% where $P(z)$ is a polynomial dependent on the velocity boundary conditions (see Appendix A \cite{Goluskin2015a}). In \eqref{eq:RL}, for no-slip boundaries when $n=0$ $R_L = 1440$, while in the limit of $n\rightarrow\infty$ $R_L \rightarrow 720$. Therefore \eqref{eq:RL} recovers the known values for linear instability of uniform IHC and RBC between fixed flux boundaries \citep{Goluskin2016book}.






\section{Discussion}

We prove lower bounds on the mean conductive heat transport $\dT$ for non-uniform IHC between parallel plates with fixed flux and no-slip boundary conditions. Our results are characterised by the vertical heat flux $\eta(z)$. The lower bound of $\dT \geq \mu - c R^{-1/3}$, where $c>0$ and $\mu \leq 0$, implies the possibility of inverse conduction, defined as a mean negative temperature gradient ($\dT < 0$), can be ruled out for all $R$ only if $\lVert \eta \rVert_2 = \lVert \eta \rVert_1$. Furthermore, we obtain an exact relation for the critical Rayleigh number $R_c$ in terms of $\eta$, below which inverse conduction is ruled out.  
Our results match previous studies \citep{Arslan2021a}, such that within the background field method $\mu$ and the $R$ scaling is optimal for the case of uniform internal heating, where $\eta = z$.


There are several restrictions in the results presented here,  primarily on the choice of heating profile. We consider heating non-uniform only in the vertical direction $z$. For flows in nature to which the model applies, the internal heating is generally non-homogeneous in space and time. Furthermore, we restrict to positive $H(z)$, yet the results could be extended to positive and negative $H(z)$ if we non-dimensionalise by fixing $H_0 = \lVert H \rVert_p$, for any $p>1$. Such a modification would also adjust the condition that $\eta(1)=1$ to ensure that the heat leaving the system matches the net input by heating or cooling. Such an alteration would provide analogies of the results obtained here with other recent work on non-uniformly heated convection \cite{Song2022,kazemi2022,bouillaut2022}. 
It is important to note that while the choice of $H(z)$ contains uniform IHC, from the constructions in this work one cannot pass to the case of fixed flux Rayleigh-B\'enard convection. The limitation arises from the choice and definition of $R$. A future line of inquiry to remove this restriction would be establishing a Rayleigh number that can interpolate between convection processes driven by boundary or body forcing.   


The analysis presented here uses the background field method, an alternative route of inquiry to determine the optimality of the result with the so-called method of \textit{optimal wall-to-wall transport}. An upper and lower bound could help further confirm or rule out the existence of inverse conduction for IHC. If inverse conduction cannot be dismissed it would be insightful to determine the velocity fields that maximise heat transport while exhibiting this behaviour.  



==> v6.tex <==
\section{Introduction}
\label{sec:intro}


Convection driven by spatially varying heating is attracting attention as a generalisation of internally heated convection (IHC) due to its relevance in studying different regimes of heat transport by turbulence. Recent work demonstrates that varying the heating location can enhance heat transport in bounded domains \citep{kazemi2022,bouillaut2022, Lepot2018} and that bounds on the heat transport depend on the supply of potential energy due to variable heating \citep{Song2022}. 
Such studies of non-uniformly heated convection have implications for geophysical fluid dynamics, from mixing in lakes, where solar radiation acts as a spatially varying heat source, to convection of the Earth's mantle and liquid outer core driven by energy released irregularly by radioactive isotopes and secular cooling. Non-uniformly heated convection controls wildlife in lakes, tectonic activity and planetary magnetism \citep{schubert2015treatise}. Furthermore, non-uniform heating is theoretically significant because it induces a much larger class of flows than those by boundary-forced examples such as Rayleigh-B\'enard convection (RBC). 

This work considers non-uniform IHC between parallel plates with fixed thermal fluxes. We assume that the lower plate is a thermal insulator and the upper plate is a poor conductor. The heat flux through the upper plate is assumed to be fixed and to match the total heat input due to internal heating (\cref{fig:config}\textit{(a)}). Beyond a given Rayleigh number, $R$, the purely conductive state is expected to be unstable, where $R$ quantifies the destabilising effect of heating to the stabilising effect of diffusion. For example, if heating is applied uniformly in the domain, instability occurs for $R > 1440$ \citep{Goluskin2015a}. In the ensuing unsteady regime, one physical property of the flow is the mean temperature difference $\dT$ between the lower and upper plates (we use $\volav{\cdot}$ to represent an infinite time and volume average, with subscript $h$ denoting a horizontal average). For the case of the fixed-flux boundary conditions considered in this work, and in contrast to RBC, $\dT$ is an emergent statistic of the unsteady flow \citep{Goluskin2016book}.

\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \draw[black,thick] (-6,0) -- (-2,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (-6,1.8) -- (-2,1.8) node [anchor = west] {$z=1$};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(2.86,1.8) (3.02,1.62) (3.1,1.5)};
    \draw [colorbar10] plot [smooth, tension = 1] coordinates {(3.1,0.3) (3.16,0.18) (3.34,0)};
    \draw [dashed ,colorbar10] (2.5,1.8) -- (3.7,0);
    \draw [colorbar10] (3.1,1.5) -- (3.1,0.3);
    \node at (1.25,-0.25) {$ \partial_z T = -1 $};
    \node at (1.25,2.025) {$ \partial_z T = -1 $};
    \node at (-4.75,0.9) { $H(z)$ };
    \draw[->] (-7,0) -- (-7,0.36) node [anchor=east]{$z$};
    \draw[->] (-7,0) -- (-6.6,0) node [anchor=north]{$x$};
    \draw[->] (-7,0) -- (-6.64,0.2) node [anchor=west]{$y$};
    \draw[black,thick] (0,0) -- (4,0) node [anchor=west] {$z=0$};
    \draw[black,thick] (0,1.8) -- (4,1.8) node [anchor = west] {$z=1$};
    \node at (-4.75,-0.25) {$ \partial_z T = 0 $};
    \node at (-4.75,2.025) {$  \partial_z T = - 1 $};
    \draw [dashed,colorbar10] plot [smooth, tension = 1] coordinates {(-3.5,1.8) (-2.8,1.1) (-2.5,0)};
    \draw [colorbar10] plot [smooth,tension=1] coordinates {(-3.5,1.8) (-3.12,1.58) (-3,1.45)}; 
    \draw [colorbar10] (-3,1.45) -- (-3,0);
    \draw[->,colorbar10,thick] (2.5,0) -- (2.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (2.5,0) -- (2.9,0) node [anchor=north]{$T$};
   \draw[->,colorbar10,thick] (-3.5,0) -- (-3.5,0.4) node [anchor=south]{$z$};
    \draw[->,colorbar10,thick] (-3.5,0) -- (-3.1,0) node [anchor=north]{$T$};
    \node at (-6.4,1.8) {\textit{(a)}};
    \node at (-0.4,1.8) {\textit{(b)}};
    \end{tikzpicture}
    \caption{\textit{(a)} Internally heated and \textit{(b)}  Rayleigh-B\'enard convection with fixed flux boundaries, where $H(z)$ is a positive non-uniform heating profile. In both panels, ({\color{colorbar10}\dashedrule}) denotes the conductive temperature profiles and ({\color{colorbar10}\solidrule}) the mean temperature profiles in the turbulent regime. In panel \textit{(a)}, the temperature profiles are for $H(z)=1$. }
    \label{fig:config}
\end{figure}

This paper communicates bounds on $\dT$ that depend on the Rayleigh number $R$ of the flow and the spatial distribution of the heat sources. More specifically, we prove that, for any solution of the governing Boussinesq equations,
\begin{equation}
    \label{eq:main_res}
    \dT := \horav{T|_{z=0}} - \horav{T|_{z=1} } \geq \sigma R^{-\gamma}-\mu, 
\end{equation}
where $\sigma,\mu>0$ are constants depending only on the nature of the internal heating, and $\gamma$ is a scaling rate. Given the relative lack of experimental and numerical data regarding internally heated flows, obtaining rigorous bounds can provide valuable insight into turbulence induced by bulk heating.

Perhaps the most closely related flow for which a rigorous characterisation of $\dT$ is known is the case of fixed-flux RBC, shown schematically in \cref{fig:config}\textit{(b)}. There, symmetric heating and cooling rates are prescribed at upper and lower boundaries (as opposed to internally), and the temperature drop satisfies the rigorous bound $\dT \geq cR^{-1/3}$ for a constant $c>0$ \citep{Otero2002}. The physical interpretation of this result is that the upper plate, through which heat leaves the domain, must, on average, remain colder than the lower one. In particular, the difference in temperature between the plates cannot decrease at a rate faster than $R^{-1/3}$, with an increasingly turbulent and homogenised flow as $R \rightarrow \infty$. Noting that $R$ is a flux-based Rayleigh number, the provable decay rate of the lower bound on $\dT$ agrees with that predicted by some phenomenological theories, namely the so-called ultimate regime \citep{kraichnan1962,spiegel1963generalization}
(see \cite{  doering2020turning} and \cite{lohse2023} for recent reviews on the ultimate regime in RBC). 



Much less is known about $\dT$ for internally heated flows with fixed flux boundary conditions. The only rigorous result proven to date is for uniformly applied internal heating, where $\dT \geq -0.030605 + 1.655R^{-1/3}$ \citep{Arslan2021a}. While the asymptotic decay rate of this bound agrees with that observed for RBC with fixed flux boundary conditions, the appearance of the negative constant -0.030605 is significant. It implies that for a sufficiently high Rayleigh number, one cannot rigorously rule out the possibility that $ \horav{T|_{z=1}} > \horav{T|_{z=0}} $ (i.e. that $\dT<0$), which means that although all heat leaves the domain from the upper boundary, on average conduction transfers heat downwards for sufficiently turbulent flows. Naturally, this raises the question of the extent to which this might be true of domains that are heated non-uniformly. For example, one might expect negative mean conductive heat fluxes as being more likely to occur if heating were concentrated near the upper boundary, as shown in \cref{fig:config2}\textit{(a)}, than if it concentrates at the bottom boundary (\cref{fig:config2}\textit{(b)}). More precisely, one considers the set of Rayleigh numbers for which it might be possible to guarantee non-negative $\dT$ and whether there are any distributions of internal heating for which, like fixed-flux RBC, negative $\dT$ can disqualified for all $R$.  



\begin{figure}
    \centering
    \hspace{-1cm}
    \begin{tikzpicture}[every node/.style={scale=0.95}]
    \fill [colorbar14] (-7,1.8) rectangle (-3.5,1.2);
    \fill [colorbar14] (-3,0) rectangle (0.5,0.6);
    \shade [top color = colorbar6, bottom color = colorbar13] (1,0.9) rectangle (4.5,0.45);
    \draw [colorbar13] (1,0.45) -- (4.5,0.45);
    \shade [top color = colorbar13, bottom color = colorbar6] (1,0.45) rectangle (4.5,0);
    \draw [colorbar6] (1,0.9) -- (4.5,0.9);
    \shade [top color = colorbar6, bottom color = colorbar1] (1,1.8) rectangle (4.5,1.35);
    \draw [colorbar1] (1,1.35) -- (4.5,1.35);
    \shade [top color = colorbar1, bottom color = colorbar6] (1,1.35) rectangle (4.5,0.9);
    \draw[black,line width=0.35mm] (-7,0) -- (-3.5,0) ;
    \draw[black,line width=0.35mm] (-7,1.8) -- (-3.5,1.8) ;
    \draw[black,line width=0.35mm] (-3,0) -- (0.5,0) ;
    \draw[black,line width=0.35mm] (-3,1.8) -- (0.5,1.8) ;
    \draw[black,line width=0.35mm] (1,0) -- (4.5,0) node [anchor=west] {$z=0$};
    \draw[black,line width=0.35mm] (1,1.8) -- (4.5,1.8) node [anchor = west] {$z=1$};
    \draw plot [smooth, tension = 1] coordinates {(-4.8,1.8) (-4.2,1.5) (-4,1.2)};
    \draw (-4,1.2) -- (-4,0);
    \draw plot [smooth, tension = 1] coordinates {(0,0) (-0.12,0.3) (-0.5,0.6)};
    \draw (-0.5,0.6) -- (-0.8,1.8);
    \draw plot [smooth, tension = 1] coordinates {(3.2,1.8) (3.8,0.8) (4,0)};
    \node at (-7.2,1.8) {\textit{(a)}};
    \node at (-3.2,1.8) {\textit{(b)}};
    \node at (0.8,1.8) {\textit{(c)}};
    \end{tikzpicture}
    \caption{ Examples of non-uniform heating profiles with illustrative sketches of the conductive temperature profiles (\solidrule) for fixed flux boundary conditions. In \textit{(a)}, the heating is localised near the upper boundary and in \textit{(b)} near the lower boundary while being zero elsewhere, shown with red ({\color{colorbar14}\solidrule}) and white spaces respectively. For \textit{(c)} the heating is sinusoidal with a maximum at $z=0.25$ ({\color{colorbar13}\solidrule}) and a minimum of zero at $z=0.75$ ({\color{colorbar1}\solidrule}).   }
    \label{fig:config2}
\end{figure}


We address these questions for a large class of heating profiles by obtaining a lower bound on $\dT$ that depends on $R$ and several geometric properties of the heating profile. In particular, we find an expression for the critical value of $R$ below which $\dT \geq 0$ for solutions of the governing equations. To do this, we develop the mathematical approach of \cite{Arslan2021a} for flows driven by arbitrary (non-uniform) heating. The paper is structured as follows: \S\ref{sec:setup} describes the setup, in \S\ref{sec:Bounds} we prove the lower bound \eqref{eq:main_res}, \S\ref{sec:Imp_bound} highlights implications of the bound and \S\ref{sec:conclusion} provides concluding remarks with perspectives for future work.      



\section{Setup}
\label{sec:setup}

We consider a layer of fluid between two horizontal plates separated by a distance $d$ and periodic in the horizontal ($x$ and $y$) directions with periods $L_x d$ and $L_y d$. The fluid has kinematic viscosity $\nu$, thermal diffusivity $\kappa$, density $\rho$, specific heat capacity $c_p$ and thermal expansion coefficient $\alpha$. Gravity acts in the negative vertical direction, and the fluid is heated internally at a position-dependent non-negative volumetric rate $\Tilde{H}\geq 0$. We assume that $\Tilde{H}$ is a non-negative integrable function on the domain that depends only on the vertical coordinate and satisfies   $\langle \tilde{H}\rangle>0$ strictly, and define a dimensionless heating as $H(z):=\tilde{H}/\langle \tilde{H}\rangle$. Note that $\langle H\rangle=\|H\|_{1}=1$ because $H(z)\geq 0$. Here and throughout the paper, $\lVert f \rVert_p$ is the standard $L^p$ norm of a function $f:[0,1]\rightarrow\mathbb{R}$.


To non-dimensionalise the problem, we use $d$ as the characteristic length scale, $d^2/\kappa$ as the time scale and $d^2\langle \tilde{H}\rangle/\kappa \rho c_p$ as the temperature scale. The velocity of the fluid $\boldsymbol{u}(\boldsymbol{x},t)=(u(\boldsymbol{x},t),v(\boldsymbol{x},t),w(\boldsymbol{x},t))$ and temperature $T(\boldsymbol{x},t)$ in the non-dimensional domain $\Omega = [0,L_x]\times[0,L_y]\times[0,1]$ are then governed by the Boussinesq equations,
\begin{subequations}
\label{eq:gov_eqs}
\begin{align}   
    \label{eq:continuit}
    \bnabla \cdot \boldsymbol{u} &= 0,\\
    \label{eq:mom_eq}
    \partial_t \boldsymbol{u} + \boldsymbol{u} \cdot \bnabla \boldsymbol{u} + \bnabla p &= Pr\, \bnabla^2 \boldsymbol{u} + Pr\, R\, T \vec{e}_3 ,   \\
    \label{eq:nondim_energy_nonUniform}
    \partial_t T + \boldsymbol{u}\cdot \bnabla T &= \bnabla^2 T + H(z).
\end{align}
\end{subequations}
The non-dimensional numbers are the Prandtl and Rayleigh numbers, defined as 
\begin{equation}
    Pr = \frac{\nu}{\kappa},
    \qquad\text{and}\qquad 
    R = \frac{g \alpha \langle \tilde{H}\rangle d^5 }{\rho c_p \nu \kappa^2 }.
\end{equation}
The boundary conditions are no-slip for the velocity and fixed flux for the temperature:
\begin{subequations}
\label{bc:non_uni}
\begin{gather}
    \label{bc:u_non_u}
    \boldsymbol{u}|_{z=\{0,1\}} = 0, \\
    \label{bc:nu}
    \partial_z T|_{z=0} = 0, \quad \partial_z T|_{z=1}=-1.
\end{gather}
\end{subequations} 
 A diagram of the system is shown in \cref{fig:config}\textit{(a)}.

It proves useful to define a function $\eta \in L^2(0,1)$ such that $\eta(z)$ measures the total (dimensionless) heat  added to those parts of the domain below a height $z$:
\begin{equation}
    \label{eq:eta_general}
    \eta(z):= \int^{z}_0 H(z)\, \textrm{d}z.
\end{equation}
Our assumptions on $H(z)$ imply that $0\leq \eta(z)\leq 1$. The value $\eta(1)=1$ corresponds to the total heat added to the domain and, therefore, to the negative heat flux applied at the top boundary in \eqref{bc:nu}.
We can obtain an identity for the mean vertical heat transport of the system by multiplying \eqref{eq:nondim_energy_nonUniform} by $z$ and taking an infinite-time and volume average. Use of \eqref{eq:eta_general} and a standard application of integration by parts with the boundary conditions \eqref{bc:u_non_u} \& \eqref{bc:nu} gives the identity,
\begin{align}   
\label{eq:energy_bal_nu}
    \wT + \dT &= -\int^{1}_{0}(z-1)H\,\textrm{d}z=\int^{1}_{0}\eta(z)\,\textrm{d}z.
\end{align}
The left-hand side of \eqref{eq:energy_bal_nu} is the sum of the mean vertical convective heat flux, $\wT$, and the mean conductive heat flux, $\dT$, and balances the potential energy added to the system. To see why, note that $-zH$ is the pointwise supply of (dimensionless) potential energy (the negative sign is there because potential energy is created by positive heating from below or negative heating from above). The middle term in \eqref{eq:energy_bal_nu} therefore accounts for the potential energy created by internal heating and cooling from the top boundary (alternatively, the shifted coordinate $z\mapsto z-1$, centred on the top boundary, can be seen as a means of removing the cooling at the top boundary from the calculation).

To remove the inhomogeneous boundary conditions on $T$ it is convenient to rewrite the temperature field in terms of perturbations $\theta$ from the conductive profile $T_c$,
\begin{equation}
    \label{eq:T}
    T(\boldsymbol{x},t) = \theta(\boldsymbol{x},t)  + T_c(z).
\end{equation}
The steady conductive temperature profile can be found after taking $\boldsymbol{u}=0$ and $T(\boldsymbol{x},t)=T(\boldsymbol{x})$ in \eqref{eq:nondim_energy_nonUniform}. Given the insulating lower boundary condition, $T'_c(z) = - \eta(z)$, where primes denote derivatives with respect to $z$. Then, \eqref{eq:nondim_energy_nonUniform} in terms of $\theta$ becomes
\begin{gather}
    \label{eq:theta_eq}
     \partial_t \theta + \boldsymbol{u} \cdot \bnabla \theta = \bnabla^2 \theta + w\, \eta(z) ,\\
    \label{bc:theta_non_u}
    \partial_z \theta|_{z=\{0,1\}} = 0 \, .
\end{gather}

\section{Bounding heat transport}
\label{sec:Bounds}

To bound $\dT$ using methods that have been successfully applied to uniform IHC \citep{Arslan2021a}, we search for an upper bound on $\wT$ and use \eqref{eq:energy_bal_nu} to bound $\dT$. We will prove upper bounds on  $\mean{w\theta}$, which is equal to $\wT$ because the incompressibility of the velocity field and the boundary conditions \eqref{bc:u_non_u} imply that any function $f:[0,1]\rightarrow\mathbb{C}$ satisfies $\volav{w f} = \int^{1}_0 \horav{w} f(z) \textrm{d}z = 0$. The derivation in  \cref{sec:afm} is analogous to that in \cite{Arslan2021a}, we only outline the main ideas in this paper.


\subsection{The auxiliary functional method}
\label{sec:afm}

Rigorous bounds on the mean quantities of turbulent flows can be found with the background method \citep{Doering1994, Doering1996,Constantin1995a}, formulated within the more general framework of the auxiliary functional method \citep{Chernyshenko2014a,Fantuzzi2022}. We consider the quadratic auxiliary functional
\begin{equation}
    \mathcal{V}\{\boldsymbol{u},\theta\} =  \fint_\Omega  \frac{a}{2\,Pr\,R} |\boldsymbol{u}|^2 + \frac{b}{2}\left|\theta  - \frac{\phi(z)}{b}\right|^2 \textrm{d}\boldsymbol{x} ,
\end{equation}
where $a$ and $b$ are non-negative scalars and $\phi(z)$ a function to be optimised. As demonstrated by \cite{Chernyshenko2022}, the use of quadratic auxiliary functionals is equivalent to the background method, where $a$ and $b$ are referred to as balance parameters and $\phi(z)/b$ is the background temperature field. With a slight abuse of terminology, we refer to $\phi(z)$ as the background field. 

Given that $\mathcal{V}\{\boldsymbol{u},\theta\}$ remains bounded in time along solutions of \eqref{eq:continuit}, \eqref{eq:mom_eq} \& \eqref{eq:theta_eq} for any given initial $\boldsymbol{u}$ and $\theta$, the infinite-time average of the time derivative of $\mathcal{V}$ is zero. Using this property, we can write,
\begin{equation}
    \label{eq:AFM_statemen}
    \mean{w\theta} = U - \left( U - \volav{w\theta} - \limsup_{\tau\rightarrow\infty} \frac{1}{\tau}\int^{\tau}_0\frac{\textrm{d}}{\textrm{d}t} \mathcal{V}\{\boldsymbol{u},\theta\} \textrm{d}t  \right),
\end{equation}
and deduce that $\mean{w \theta} \leq U$ if the functional in the brackets in \eqref{eq:AFM_statemen} is pointwise in time non-negative. 
Computations analogous to \cite{Arslan2021a} show that the optimal bound provable is given by,
\begin{equation}
    \label{eq:U_bound}
    U = \int^{1}_{0}\frac{\phi'(z)^2}{4b}\textrm{d}z,
\end{equation}
provided that the following constraint, referred to as the \textit{spectral constraint}, holds,
\begin{multline}
    \label{eq:sk_non_uni}
     \frac{a}{R\,k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{2a}{R} \lVert w'_{\boldsymbol{k}} \rVert_2^2 + \frac{ak^2}{R}\lVert w_{\boldsymbol{k}} \rVert_2^2 + b \lVert \theta'_{\boldsymbol{k}}\rVert_2^2  + b k^2\lVert \theta_{\boldsymbol{k}} \rVert_2^2  \\ - \int^{1}_0 \left(a + 1 + b  \eta(z) - \phi'(z) \right)\textrm{Re}\{w_{\boldsymbol{k}} \theta^*_{\boldsymbol{k}} \}  \textrm{d}z \geq 0, 
\end{multline}
where $w_{\boldsymbol{k}}(z)$ and $\theta_{\boldsymbol{k}}(z)$ are the amplitudes of the Fourier modes introduced by exploiting horizontal periodicity.
The spectral constraint must hold for all nonzero wavevectors $\boldsymbol{k}=(k_x,k_y)$ with magnitude $k^2 = k_x^2 + k_y^2$ and all $w_{\boldsymbol{k}}(z)$ and $\theta_{\boldsymbol{k}}(z)$ satisfying the boundary conditions
\begin{subequations} 
\begin{gather}
    \label{bc:w_k}
    w_{\boldsymbol{k}}(0)= w_{\boldsymbol{k}}(1)= w_{\boldsymbol{k}}'(0)= w_{\boldsymbol{k}}'(1)=0,\\
    \label{bc:T_k}
     \theta_{\boldsymbol{k}}'(0) =  \theta_{\boldsymbol{k}}'(1) =0.
\end{gather}
\end{subequations}


\subsection{Enforcing the spectral constraint}
\label{sec:spectral}

To obtain an explicit bound $U$, we choose to set
\begin{equation}
    \label{eq:b_relation}
    b = \frac{a+1}{\lVert \eta \rVert_2},
\end{equation}
and use the background field
    \begin{equation}
	 \phi'(z) = \frac{(a+1)}{\lVert \eta \rVert_2}
        \begin{dcases}
            0, &  0\leq z \leq \delta, \\
            \eta(z) + \lVert \eta \rVert_2,  &  \delta \leq z \leq 1-\delta,\\
            0,& 1-\delta \leq z \leq 1,
        \end{dcases}
    \label{eq:phi_prime}
    \end{equation}
    where $\delta \leq \frac12$ is the width of the boundary layers of $\phi'(z)$.
Both choices are motivated by results obtained in the case of uniform IHC \citep{Arslan2021a}. We expect that corrections to the bound obtained from further optimisation of $b$ and $\phi'(z)$ do not change the qualitative behaviour of the results in this work. Fine-tuning \eqref{eq:phi_prime} could involve using boundary layers of different widths and non-constant functions near the boundaries. We expect that this will change the values, but not signs, of the constants $\mu$ and $\sigma$ in \eqref{eq:main_res}.
% To motivate these choices, note that if $\phi'(z) = a+1+b\eta(z)$, then the spectral constraint in \eqref{eq:sk_non_uni} is immediately satisfied. The resulting bound $U$, which is conservative because it is uniform in $R$, can be optimised for $b$ to obtain the relation \eqref{eq:b_relation}. By definition $U$ is non-negative and since we seek an upper bound of the form $U\leq U_0 - \sigma R^{-\gamma}$, the uniform bound is exact only in the limit $R\rightarrow\infty$ but remains conservative for all finite $R$.
% We thus conjecture that the relation between $a$ and $b$ in \eqref{eq:b_relation} is optimal to leading order for all $R\gg 1$. 
% However, the choice $\phi'(z) = a+1+b\eta(z)$ does not give a $R$-dependent bound, unless $\phi'(z)$ has boundary layers of widths $\delta$, as found in the simple example \eqref{eq:phi_prime}. The simplest modification to $\phi'(z)$ such that it has boundary layers of equal widths $\delta$ is the choice \eqref{eq:phi_prime}.


We begin by formulating a simpler sufficient condition for the spectral constraint \eqref{eq:sk_non_uni} to hold. First, we drop the positive terms in $w_{\boldsymbol{k}}'(z)$, $w_{\boldsymbol{k}}(z)$ and $\theta'_{\boldsymbol{k}}(z)$. Then, we plug in our choices \eqref{eq:b_relation} for $b$ and \eqref{eq:phi_prime}  for $\phi'(z)$, and use the inequality $\eta(z)\leq 1$ to conclude that \eqref{eq:sk_non_uni} holds if 
\begin{equation}
    \label{eq:sk-cond_2}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{a+1}{\lVert \eta \rVert_2} (1+\lVert \eta \rVert_2)  \int_{(0,\delta)\cup(1-\delta,1)} |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \geq 0.
\end{equation}
Note that the boundary layers $(0,\delta)$ and $(1-\delta,1)$ are disjoint because $\delta\leq \tfrac12$ by assumption.

Next, given the boundary conditions on $w_{\boldsymbol{k}}(z)$ from \eqref{bc:w_k}, the use of the fundamental theorem of calculus and the Cauchy-Schwarz inequality gives,
\begin{equation}
\label{eq:w_estimate}
     w_{\boldsymbol{k}}(z) = \int^{z}_0 \int^{\xi}_0 w_{\boldsymbol{k}}''(\sigma) \textrm{d}\sigma \textrm{d}\xi \leq \int^{z}_0 \sqrt{\xi} \, \lVert w_{\boldsymbol{k}}'' \rVert_{2} \,\textrm{d}\xi  = \frac23 z^\frac32\, \lVert w_{\boldsymbol{k}}'' \rVert_2.
\end{equation}
Using \eqref{eq:w_estimate} and the Cauchy-Schwarz inequality, we can estimate
\begin{align}
     \int_0^\delta |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z \leq  \int_0^\delta |w_{\boldsymbol{k}}| |\theta_{\boldsymbol{k}}| \textrm{d}z
     \leq \frac23 \lVert w_{\boldsymbol{k}}'' \rVert_2\int_0^\delta
     z^{\frac32} \, |\theta_{\boldsymbol{k}}| \textrm{d}z 
     &\leq \frac23 \lVert w_{\boldsymbol{k}}'' \rVert_2 \lVert \theta_{\boldsymbol{k}} \rVert_2\left( \int^{\delta}_0 z^3 \textrm{d}z \right)^{\frac12} \nonumber \\
     &=\frac{\delta^2}{3}  \lVert w_{\boldsymbol{k}}'' \rVert_2 \lVert \theta_{\boldsymbol{k}} \rVert_2 . 
 \end{align}
 The same estimate applies to $\int_{1-\delta}^1 |w_{\boldsymbol{k}} \theta_{\boldsymbol{k}}| \textrm{d}z$, so we conclude that \cref{eq:sk-cond_2} holds if
\begin{equation}
    \frac{a}{R k^2} \lVert w''_{\boldsymbol{k}} \rVert_2^2 + \frac{a+1}{\lVert \eta \rVert_2} k^2  \lVert \theta_{\boldsymbol{k}}\rVert_2^2 - \frac{2(a+1)}{3 \lVert \eta \rVert_2} (1+\lVert \eta \rVert_2 ) \delta^2  \lVert w''_{\boldsymbol{k}} \rVert_2\lVert \theta_{\boldsymbol{k}} \rVert_2    \geq 0.
\end{equation}
The left-hand side of this inequality is a homogeneous quadratic form in $\lVert w_{\boldsymbol{k}}'' \rVert_2$ and $\lVert \theta_{\boldsymbol{k}}\rVert_2$, and it is non-negative if it has a nonpositive discriminant. Therefore, the spectral constraint is satisfied if,
\begin{equation}
    \label{eq:sk_cond_ineq}
    \delta^4 \leq \frac{ 9 a  \lVert \eta \rVert_2}{ (a+1) (1+\lVert \eta \rVert_2)^2 R }.
\end{equation}

\subsection{Evaluating the bound}
\label{sec:eval_b}

Next, we estimate the bound $U$ in \eqref{eq:U_bound} given our ans\"{a}tze \eqref{eq:b_relation} and \eqref{eq:phi_prime}. Making use of the fact that $\eta(z)\geq 0$ gives, after rearranging,  
\begin{align}
    U &=
    \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1-\delta}_{\delta} \left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z
    \nonumber \\
    &= \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int^{1}_{0}\left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z 
    - \frac{ a+1  }{4 \lVert \eta \rVert_2 } \int_{(0,\delta) \cup (1-\delta,1)} \left(\eta(z) +  \lVert \eta \rVert_2\right)^2 \textrm{d}z
    \nonumber \\
    &\leq 
   \frac12 (a+1)  \left( \lVert \eta \rVert_2 + \lVert \eta \rVert_1 -  \lVert \eta \rVert_2 \delta \right).
     \label{eq:U_form_sub}
\end{align}
By definition, $a$ is real and positive, which means that $(a+1)^m\geq1$ for all $m>0$. Therefore,
taking $\delta$ as large as possible in \eqref{eq:sk_cond_ineq} and substituting into \eqref{eq:U_form_sub} gives,
\begin{align}
    U &\leq   \frac12 (a+1)  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1) 
    - \frac{\sqrt{3}}{2} \frac{\lVert\eta\rVert_2^{5/4}}{(1+\lVert\eta\rVert_2)^{1/2}}(a+1)^{3/4} a^{1/4} R^{-1/4}  \nonumber\\
    &\leq   \frac12 (a+1)  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1) 
    - \frac{\sqrt{3}}{2} \frac{\lVert\eta\rVert_2^{5/4}}{(1+\lVert\eta\rVert_2)^{1/2}} a^{1/4} R^{-1/4} .
    \label{eq:U_delt_sub}
\end{align}
We now minimise the last expression in \eqref{eq:U_delt_sub} over $a$ to obtain the best possible estimate on $U$. The optimal choice of $a$ is,
\begin{equation}
    a^* =  \frac{a_0 \lVert \eta \rVert_2^{5/3}}{ (\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{4/3} (1+\lVert \eta \rVert_2 )^{2/3}} R^{-1/3},
\end{equation}
where $a_0 = (\frac{9}{256})^{1/3}$. Finally, substituting for $a$ in \eqref{eq:U_delt_sub}, rearranging and since  $\mean{w\theta} \leq U$, we get,
\begin{equation}
    \mean{w \theta} \leq  \frac12  ( \lVert \eta \rVert_2 + \lVert \eta \rVert_1)  -  \frac{a_1 \lVert \eta \rVert_2^{5/3}}{(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{1/3}(1+\lVert \eta \rVert_2)^{2/3} } R^{-1/3},
\end{equation}
where $a_1 = \frac{3\sqrt{3}}{8} a_0^{1/4} $.
Then, by \eqref{eq:energy_bal_nu}, 
\begin{equation}
    \label{eq:dT_bound_simple}
    \dT \geq   \frac12  ( \lVert \eta \rVert_1 - \lVert \eta \rVert_2)  +  \frac{a_1 \lVert \eta \rVert_2^{5/3}}{(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)^{1/3}(1+\lVert \eta \rVert_2)^{2/3} } R^{-1/3},
\end{equation}
completing the proof of \eqref{eq:main_res}. 


\section{Implications of the bound}
\label{sec:Imp_bound}
Equation \eqref{eq:dT_bound_simple} states that $\dT < 0$ is only possible when $R>R_o$, where 
\begin{equation}
    R_o = \frac{8a_1^3 \lVert \eta \rVert_2^5 }{(1+\lVert \eta \rVert_2)^2(\lVert \eta \rVert_2 + \lVert \eta \rVert_1)(\lVert \eta \rVert_2 - \lVert \eta \rVert_1)^3}\, .
    \label{eq:Rc_g}
\end{equation}
According to \eqref{eq:dT_bound_simple}, only for heating profiles for which $\|\eta\|_{1}=\|\eta\|_{2}$ is it possible to guarantee that $\dT>0$ for all $R$. However, noting that $\eta(z)$ increases monotonically with respect to $z$, $\eta(0)=0$ and $\eta(1)=1$ then,
\begin{equation}
    \lVert \eta \rVert_2^2 = \lVert \eta^2 \rVert_1 < \lVert \eta \rVert_1. 
    \label{eq:eta_L2_bounds}
\end{equation}
Within the class of heating profiles, we have considered, \eqref{eq:eta_L2_bounds} gives an upper bound on $\lVert \eta \rVert_2$ and rules out the possibility that there is a heating profile for which $\dT>0\ \forall R$. Taking $H$ as a distribution rather than a function, then $\|\eta\|_{1}=\|\eta\|_{2}$ would correspond to the set of distributions consisting of two (not necessarily equal) finite amounts of heat, represented as Dirac measures at $z=0$ and $z=1$. 

\begin{figure}
    \centering
    \hspace{-1cm}
    \includegraphics[scale=1]{fig/myVectorFile.eps}
     \begin{tikzpicture}[overlay]
        \node at (-12,8.4) {\textit{(a)}};
       \node at (-4.5,6.7) {\textit{(b)}};
        \node at (-12,2.7) {\textit{(c)}};
        \node at (-8.8,2.7) {\textit{(d)}};
       \node at (-5.9,2.7) {\textit{(e)}};
       \node at (-3,2.7) {\textit{(f)}};
    \end{tikzpicture}
    \caption{\textit{(a)} Contour plot of $R_o$ as given in \eqref{eq:Rc_g} with the inset \textit{(b)} highlighting a region ($[0.925,1]\times[0.95,1]$) where $\lVert \eta\rVert_1 \sim \lVert \eta \rVert_2$. In panel \textit{(a)} the green cross (\mycross{matlabgreen}) highlights uniform heating, drawn in \textit{(c)}, the blue cross (\mycross{matlabblue}) highlights heating near the lower boundary drawn in \textit{(d)}, the yellow cross (\mycross{matlabyellow}) highlights heating near the upper boundary \textit{(e)} and the black cross (\mycross{black}) highlights sinusoidal heating, panel \textit{(f)}. }
    \label{fig:main_res}
\end{figure}



A further restriction on the possible values of $\|\eta\|_{1}$ and $\|\eta\|_{2}$ comes from the Cauchy-Schwarz inequality $\|\eta\|_{1}\leq\|\eta\|_{2}$, which would be saturated by distributions consisting of a single Dirac measure of unit heat at some height $z\in[0,1]$. For the differentiable $\eta$ considered in this work, the inequality is strict,
\begin{equation}
    \lVert \eta \rVert_1 < \lVert \eta \rVert_2.
    \label{eq:eta_L1_bounds}
\end{equation}
The open set of functions satisfying \eqref{eq:eta_L2_bounds} and \eqref{eq:eta_L1_bounds} is illustrated in figure \ref{fig:main_res}\textit{(a)}.

In \cref{sec:Bounds}, the additional requirement that $\delta\leq \frac12$ in the choice of $\phi'(z)$ gives a minimum $R=R_m$ above which the final bound \eqref{eq:dT_bound_simple} holds. Taking $\delta$ as large as possible in \eqref{eq:sk_cond_ineq} gives that $\delta \leq \frac12$ for all
\begin{equation}
    R \geq R_m = \frac{18 \lVert \eta \rVert_2^{2} }{(\lVert \eta \rVert_1 + \lVert \eta \rVert_2)(1+ \lVert \eta \rVert_2)^2}.
\end{equation}



To validate the main results from \cref{sec:Bounds} we can consider the case of uniform heating, $H(z)=1$. In this case one has $\eta(z)=z$ and obtains from  \eqref{eq:dT_bound_simple} the lower bound $\dT \geq -0.030605 + 0.1850 R^{-1/3}$, valid for all $R\geq R_m =2.2384$ which is far below the critical Rayleigh number for linear instability of 1440. The bound matches the scaling and asymptote of \cite{Arslan2021a}. The difference in the constant multiplying the $O(R^{-1/3})$ term is due to the choice of taking $\phi'(z)$ linear (rather than constant) in $z$ within the boundary layers.


The results \eqref{eq:dT_bound_simple} and \eqref{eq:Rc_g} apply to all heating profiles that can be specified as a function of $z$ and integrate to unity. \cref{fig:main_res} \textit{(a)}  is a contour plot of the critical $R_o$ over the open region satisfying the inequalities \eqref{eq:eta_L2_bounds} and \eqref{eq:eta_L1_bounds}. Example non-uniform heating profiles from \cref{fig:config2} are plotted in \cref{fig:main_res}, for cases in which the heating is \textit{(d)} near the bottom boundary, \textit{(e)} near the upper boundary and \textit{(f)} sinusoidal, with the corresponding $R_o$ highlighted with crosses in \cref{fig:main_res} \textit{(a)}. 



\section{Conclusion}
\label{sec:conclusion}

We have obtained lower bounds on the mean vertical conductive heat transport, $\dT$, for non-uniform internally heated convection between parallel plates with fixed flux thermal boundary conditions. The bounds can be expressed in terms of a Rayleigh number and the mean vertical heat flux $\eta(z)$, which corresponds to the prescribed internal heating $H(z)$ integrated upwards from the bottom boundary to a height $z$. In particular, we prove with the auxiliary functional method that $\dT \geq -\mu + \sigma R^{-1/3}$ in \eqref{eq:dT_bound_simple}, where $\mu, \sigma>0$. We were, therefore, able to obtain an explicit Rayleigh number $R_o$, in terms of $\eta(z)$, below which it is possible to guarantee that $\dT\geq 0$. The results are consistent with those obtained from the particular case of uniform internal heating ($\eta=z$) \citep{Arslan2021a}.


Only in the limit of heat being concentrated entirely at the bottom is it possible to guarantee that $\dT \geq 0$ for all $R$ ($\mu=0$ in the previous paragraph). However, in a mathematical sense, such heating profiles are distributions rather than functions of $z$, lying beyond the scope of the internal heating profiles considered in this work and constitute the boundary, or closure, of the open set of pairs $(\|\eta\|_{1}, \|\eta\|_{2})$ that determine $\mu$ and $\sigma$ and are shown in figure \ref{fig:main_res}. In this regard, there is an intriguing connection with Rayleigh-B\'{e}nard convection, for which $\dT \geq 0$ for all $R$ \citep{Otero2002}.


While the use of the auxiliary functional method provides a rigorous bound on $\dT$, it does not guarantee the existence of flows that saturate the bound or provide insight into the predominant physical processes that are responsible for extremising $\dT$. In other words, the question of whether there are solutions to the Boussinesq equations that produce negative mean vertical conductive heat transport ($\dT<0$) when $R>R_o$ remains an open and interesting problem to investigate in the future. A possible avenue for exploring this question is the method of optimal wall-to-wall transport \citep[see e.g.][]{Tobasco2017}, which would yield a velocity field that minimises $\dT$ subject to a prescribed set of constraints, along with upper bounds on $\dT$. 

Caution should be applied in interpreting the Rayleigh number that is used to study non-uniform IHC. Our Rayleigh number follows convention by defining temperature and length scales using the volume averaged internal heating and domain height, respectively. However, in cases with heating concentrated towards the top of the domain, the physical interpretation of the Rayleigh number as quantifying the size of destabilising forces relative to the stabilising effects of diffusion is questionable. Although the choice of Rayleigh number is somewhat superficial, an appropriate choice might shed light on the dependence of the bounds on $R$ in terms of the underlying physics. Heating and cooling that is applied non-uniformly over the horizontal as well as vertical directions \citep[see e.g.][]{Song2022} poses further challenges in this regard and an opportunity to extend the results reported
in this work.



